PhD Dissertation: Generalized Independent Components Analysis Over Finite Alphabets

Independent component analysis (ICA) is a statistical method for transforming an observable multi-dimensional random vector into components that are as statistically independent as possible from each other. Usually the ICA framework assumes a model according to which the observations are generated (such as a linear transformation with additive noise). ICA over finite fields is a special case of ICA in which both the observations and the independent components are over a finite alphabet. In this thesis we consider a formulation of the finite-field case in which an observation vector is decomposed to its independent components (as much as possible) with no prior assumption on the way it was generated. This generalization is also known as Barlow's minimal redundancy representation and is considered an open problem. We propose several theorems and show that this hard problem can be accurately solved with a branch and bound search tree algorithm, or tightly approximated with a series of linear problems. Moreover, we show that there exists a simple transformation (namely, order permutation) which provides a greedy yet very effective approximation of the optimal solution. We further show that while not every random vector can be efficiently decomposed into independent components, the vast majority of vectors do decompose very well (that is, within a small constant cost), as the dimension increases. In addition, we show that we may practically achieve this favorable constant cost with a complexity that is asymptotically linear in the alphabet size. Our contribution provides the first efficient set of solutions to Barlow's problem with theoretical and computational guarantees. Finally, we demonstrate our suggested framework in multiple source coding applications.

==> Chapters/Combined_GP.tex <==
\section{Introduction}
\begin{comment}
The use of computerized simulation as an experimental tool has
expanded over the years to many fields of science and engineering.
Exploring the evolution of fire \cite[chapter~1]{santner}, measuring
oil pressure at wells \citep{Kennedy+O'Hagan} and designing computer
hardware \citep{IBM} are just some of the applications where
computer experiments now frequently replace physical experiments. It
is often useful to fit a surrogate, statistical model that relates
the output of the simulator to the levels of input factors. For
example, a surrogate can facilitate much more extensive exploration
of the factor space when the underlying mathematical model coded
into the simulation is a rather complex one, resulting in
substantial run times. The surrogate model can also be helpful in
enhancing understanding of the input-output relationships.
\cite{Sacks} suggested that the observed values of the response
variable could be modeled as realizations of a Gaussian process.
This approach - often referred to as \textit{Kriging} - is described
in Section \ref{Kriging}.  Amongst other benefits, the Gaussian
process model provides us with a basis for statistical inference in
addition to point estimates.\\
\end{comment}

\noindent Gaussian process models require specification of both model
parameters and structural features. It is convenient to assume a
priori that - apart from an optional linear trend - the underlying process is stationary (having identical
marginal distributions throughout the input space), but this
property could prove undesirable if the true response changes
significantly across different regions. \cite{Taddy} counter the
problem by fitting seperate models to subdivisions of the input
space, while \cite{nonstationary} avoid it by fitting a
nonstationary process instead. In Section \ref{Combined} we propose
a model that leaves room for more than one active process in
modeling the data. We formulate a Bayesian
model and use methods for efficient implementation.
Univariate and bivariate simulation results
presented in Section \ref{Simulations} suggest that this approach
has benefits for rapidly changing functions.
We examine two applications in Section \ref{sec:app}. In the first example, a
simulator is used to study ground motion caused by an earthquake.
This application includes 9 different input factors reflecting
the strength and frequency content of the seismic signal and
the lithology of the affected site. The second example, which simulates a heat exchanger,
was first described by \cite{Qian}.\\


\begin{comment}
\noindent Although deterministic computer experiments differ from physical experiments
in many aspects (blocking, randomization and replication are redundant,
to name some), the often time-consuming performance of each run makes
experimental design a major issue. Many popular designs relate to the
notion of uniform spread, making no a priori assumptions on the outcomes,
whereas other designs focus on optimizing various statistical criteria.
\cite{Sigal}, \cite{jones+johnson}, \cite{Kleijnen} and
\citet[chapter~5]{santner} provide extensive reviews of many of these
ideas.
\end{comment}
\noindent In Section
\ref{Batch_Sequential} we exploit the Bayesian framework established
earlier to generate Maximum Entropy designs  \citep{Shewry} for our model
in two different ways.  We examine their effect on the prediction and
Bayesian inference for a bivariate function. This is followed by final
comments and discussion in Section \ref{Discussion}.




\begin{comment}
\section{The Gaussian Process Model}\label{Kriging}
Gaussian process models are commonly used in relating a vector $\boldsymbol{x}$ of inputs and a real (sometimes vector) valued response $Y(\boldsymbol{x})$. The general model is
\begin{align}\label{GRF}
y(\boldsymbol{x}) = \boldsymbol{f}^\top(\boldsymbol{x})\boldsymbol{\beta} + Z(\boldsymbol{x}) + \varepsilon(\boldsymbol{x})\hspace{0.3em},
\end{align}
where $\boldsymbol{f}$ is a vector of fixed regression functions,
$\boldsymbol{\beta}$ is a vector of unknown regression parameters,
$\varepsilon(\boldsymbol{x})$ is the (random) measurement error and
$Z(\boldsymbol{x})$ is a zero mean Gaussian process, often
stationary with variance $\sigma^2$ and correlation function
$R\left(\boldsymbol{x}_1,\boldsymbol{x}_2\right)$. In this work,
$y\ofx$ is the output of a deterministic simulator,
therefore the error term can be omitted. In addition, as in
\cite{Welch92}, we reduce $\boldsymbol{f}$ to an unknown intercept
only, $\beta_0$, preferring to model dependence on $\boldsymbol{x}$
via the correlation function. Partial justification for this choice
is given by \cite{Dizza}, who argue that low order polynomial terms
are approximately accounted for by the leading eigenfunctions of
$R\left(\boldsymbol{x}_1,\boldsymbol{x}_2\right)$ for popular
classes of correlation functions.\\




\noindent Consider the problem of estimating the value of the output $y$ at a point
$\boldsymbol{x}_0$ in the factor space on the basis of $n$ runs of the
simulator, which result in data $$\boldsymbol{y} =
\left[y\left(\boldsymbol{x}_1\right),\ldots,y\left(\boldsymbol{x}_n\right)\right]^{\mathsf{T}}\spc.$$
It can be shown (see \citealt[chapter~4]{santner}, for detailed
derivation) that if
$$\boldsymbol{R} =
\left\{R\left(\boldsymbol{x}_i,\boldsymbol{x}_j\right)\right\}\spc,\spc1\leq i,j\leq n$$ is the correlation matrix at the design sites,
$$\boldsymbol{r}(\boldsymbol{x}) =
\left[R\left(\boldsymbol{x}_0,\boldsymbol{x}_1\right),\ldots,R\left(\boldsymbol{x}_0,\boldsymbol{x}_n\right)\right]^{\mathsf{T}}$$
and in addition we assign an improper prior to $\beta_0$, $\pi(\beta_0)\propto 1$, then
$$y(\boldsymbol{x}_0)\big|\boldsymbol{y}\sim\mathcal{N}\left\{\widehat{y}(\boldsymbol{x}_0)\hspace{0.1em},\hspace{0.1em}\sigma_0^2(\boldsymbol{x}_0)\right\}$$
where
\begin{align}\label{eq:prediction}
\widehat{y}(\boldsymbol{x}_0) =
\mathbb{E}\left[y(\boldsymbol{x}_0)\big|{\boldsymbol{y}}\right] =
\widehat{\beta}_0 +
\boldsymbol{r}^{\mathsf{T}}(\boldsymbol{x}_0)\boldsymbol{R}^{^{-1}}\left(
\boldsymbol{y} - \widehat{\beta}_0\boldsymbol{1}_n\right)\hspace{0.3em},
\end{align}
$$\widehat{\beta}_0 = \left(\boldsymbol{
1}_n^{\mathsf{T}}\boldsymbol{R}^{^{-1}}\boldsymbol{1}_n\right)^{-1}\boldsymbol{
1}_n^{\mathsf{T}}\boldsymbol{R}^{^{-1}}{\boldsymbol{y}}$$
and
\begin{align}\label{eq:post_var_1}
\sigma_0^2(\boldsymbol{x}_0) =
\var\left[y(\boldsymbol{x}_0)\big|{\boldsymbol{y}}\right] =
\sigma^2\left[1-\boldsymbol{r}(\boldsymbol{x}_0)^{\mathsf{T}}\boldsymbol{R}^{^{-1}}\boldsymbol{r}(\boldsymbol{x}_0)
+ \dfrac{\left\{1-\boldsymbol{
1}_n^{\mathsf{T}}\boldsymbol{R}^{^{-1}}\boldsymbol{r}(\boldsymbol{x}_0)\right\}^2}{\boldsymbol{
1}_n^{\mathsf{T}}\boldsymbol{R}^{^{-1}}\boldsymbol{1}_n}\right]\hspace{0.3em}.
\end{align}
Note that (\ref{eq:prediction}) is the usual choice for an estimator of
$y(\boldsymbol{x}_0)$ as the minimizer of the mean squared prediction
error. It is also the BLUP of $y(\boldsymbol{x}_0)$ and interpolates the
original data with zero posterior variance. Expression
(\ref{eq:post_var_1}) is the mean squared prediction error itself. If
$\sigma^2$ is assumed unknown then the predictor
$\widehat{y}(\boldsymbol{x}_0)$ remains unchanged, but
$$\dfrac{y(\boldsymbol{x}_0)-\widehat{y}(\boldsymbol{x}_0)}{s(\boldsymbol{x}_0)}\Bigg|\boldsymbol{y}\sim t_{n-1}\spc,$$
where $s^2(\boldsymbol{x}_0)$ is the result of replacing $\sigma^2$ in (\ref{eq:post_var_1}) by $$\left(n-1\right)^{-1}{\boldsymbol{y}}^{\mathsf{T}}\left[\boldsymbol{R}^{^{-1}}
- \dfrac{\boldsymbol{R}^{^{-1}}\boldsymbol{1}_n\boldsymbol{
1}_n^{\mathsf{T}}\boldsymbol{R}^{^{-1}}}{\boldsymbol{
1}_n^{\mathsf{T}}\boldsymbol{R}^{^{-1}}\boldsymbol{1}_n}\right]{\boldsymbol{y}}\spc.$$
\end{comment}





\section{Convex Combination of Gaussian Processes}\label{Combined}


Suppose now that
$y\left(\boldsymbol{x}_1\right),\ldots,y\left(\boldsymbol{x}_n\right)$
are realized observations from not one but a mixture of two independent
stationary Gaussian processes having the same marginal variance, namely
$$y(\boldsymbol{x}) = \beta + Z(\boldsymbol{x})$$
where
\begin{align}\label{eq:mixture}
Z(\boldsymbol{x}) = pZ_1(\boldsymbol{x}) + (1-p)Z_2(\boldsymbol{x})\hspace{0.5em},\hspace{0.5em} 0\leq p\leq1
\end{align}
and
\begin{align}\label{eq:corrs}
Z_1\ofx = \mathrm{GP}\left(0, \sigma^2R_1\left(\boldsymbol{h};\boldsymbol{\theta}_1\right)\right)\hspace{1em};\hspace{1em} Z_2\ofx =
\mathrm{GP}\left(0, \sigma^2R_2\left(\boldsymbol{h};\boldsymbol{\theta}_2\right)\right).
\end{align}
The mixture parameter $p$ can serve one of two purposes: if $R_1(\boldsymbol{h};\boldsymbol{\theta}_1)$ and $R_2(\boldsymbol{h};\boldsymbol{\theta}_2)$ belong to different families of
correlation functions then $p$ reflects our uncertainty regarding the
structure of the correlation between different observations; if both
belong to the same family but differ in scale (i.e. the correlation
parameters $\boldsymbol{\theta}$), then our model could be thought of as combining a
`tame' process and a second, `volatile' process.  This is done by
using two quite different values of $\boldsymbol{\theta}$ in the correlation function.
This kind of construction was inspired by smooth functions whose behavior
changes across different areas of the input space.\\



\noindent Combining (\ref{eq:mixture}) and (\ref{eq:corrs}) we know that
\begin{align*}
Z(\boldsymbol{x}) = \mathrm{GP}\left(0\hspace{0.2em},\hspace{0.2em}\widetilde{\sigma}^2_{p}\cdot\widetilde{R}_{p,\boldsymbol{\theta}_1,\boldsymbol{\theta}_2}\left(\boldsymbol{h}\right)\right)
\end{align*}
is merely another stationary process, with
\begin{align}\label{eq:var_combined}
\widetilde{\sigma}^2_{p} = \left[p^2 + (1-p)^2\right]\sigma^2
\end{align}
and
\begin{align}\label{eq:corr_combined}
\widetilde{R}_{p,\boldsymbol{\theta}_1,\boldsymbol{\theta}_2}\left(\boldsymbol{h}\right) = \dfrac{p^2R_1\left(\boldsymbol{h};\boldsymbol{\theta}_1\right) +\left(1-p\right)^2R_2(\boldsymbol{h};\boldsymbol{\theta}_2)}{p^2 + (1-p)^2}\hspace{0.5em}.
\end{align}

\noindent \cite{booker} proposed a nearly identical framework for the purpose of improving
numerical stability when a Kriging metamodel is used to optimize a computer
code. He fitted a model consisting of two indpendent Gaussian processes with different
correlation structures, using maximum likelihood to estimate the variance and
correlation parameters.
Modeling spatial variation by a sum of independent processes has also been explored in the kriging literature, where it is known as \textit{regionalization} (see \citealt[chapter~14]{regionalization}).\\

\noindent In this work, we favor the Bayesian approach to fit our model, partly because we wish
to derive prediction intervals along with our predictions, and they are immediately
available from the posterior predictive
distribution.
Although optimization is not the focal point of this work,
improved numerical stability is a welcome byproduct of our approach, as we
argue in Section \ref{Discussion}.\\


\noindent Recently, \cite{CGP} proposed a Composite Gaussian
Process (CGP) model, which also involves a linear combination of
`local' and `global' processes.  Thus CGP is similar in structure to
our model.  One important difference between the models is that
we give constant weights to the two processes whereas CGP
allows the weights to vary across the input space, making their
composite process nonstationary.  We compare its performance to our combined GP
model, using the \texttt{CGP} R package (see \citealt{CGP_Pack}).


%*****************************************************************************
%*****************************************************************************

\subsection{Isotropic Processes}
We focus here on the case where $\boldsymbol{\theta}_1=\theta_1\boldsymbol{1}_d$ and $\boldsymbol{\theta}_2=\theta_2\boldsymbol{1}_d$, and assign a prior distribution
$\left(p,\theta_1,\theta_2\right)\sim
\pi\left(p,\theta_1,\theta_2\right)$. Then we apply a change of variables
so that all the parameters are supported by the entire real axis,
\begin{align}\label{change_of_vars}
\psi = \log\dfrac{p}{1-p}\spc,\spc \varphi_1 =
\log\theta_1\spc,\spc\varphi_2 = \log\theta_2\spc.
\end{align}
For the rest of this work, we will omit the subscripts in (\ref{eq:var_combined}) and the correlation matrix based on (\ref{eq:corr_combined}) and simply write $\widetilde{\sigma}^2$ and $\widetilde{\boldsymbol{R}}$, respectively, with
$$\widehat{\beta}=\widehat{\beta}_{p,\theta_1,\theta_2} = \left(\boldsymbol{1}_n^{\mathsf{T}}\widetilde{\boldsymbol{R}}^{-1}\boldsymbol{1}_n\right)^{-1}\boldsymbol{1}_n^{\mathsf{T}}\widetilde{\boldsymbol{R}}^{-1}\boldsymbol{y}\spc.$$
The log-posterior can then be expressed as
\begin{align}\label{eq:logpost}
\log \hspace{0.1em}&\pi\left\{\psi,\varphi_1,\varphi_2\big|\boldsymbol{y}\right\} =\nonumber\\[1em]  &\log\pi\left\{p(\psi),\theta_1(\varphi_1),\theta_2(\varphi_2)\right\}\nonumber\\[1em]
&- \frac{1}{2}\left[n\log\widetilde{\sigma}^2 + \log\left|\widetilde{\boldsymbol{R}}\right| + \frac{\left(\boldsymbol{y}-\widehat{\beta}\boldsymbol{1}_n\right)^{\mathsf{T}}\widetilde{\boldsymbol{R}}^{^{-1}}\left(\boldsymbol{y}-\widehat{\beta}\boldsymbol{1}_n\right)}{\widetilde{\sigma}^2}\right]  \nonumber\\[1em]
& + \varphi_1 + \varphi_2 - \psi - 2\log\left(1 + \expo{-\psi}\right) + \mathrm{const}
\end{align}
(where the last line is the logarithm of the Jacobian of (\ref{change_of_vars})) and we may thus use the Metropolis-Hastings scheme (see \citealt[chapter~7]{casella}, for example) to draw a random sample from the posterior distribution $\pi\left(p,\theta_1,\theta_2\big|\boldsymbol{y}\right)$\spc.\\






\noindent The sample from the posterior distribution provides a basis for
statistical inference about values of the underlying function at any new
site $\boldsymbol{x}_0$. Recall that
\begin{align*}
y\left(\boldsymbol{x}_0\right)\big|\boldsymbol{y},p,\theta_1,\theta_2\sim\mathcal{N}\big\{\mu_{p,\theta_1,\theta_2}\left(\boldsymbol{x}_0\big|\boldsymbol{y}\right),\sigma^2_{p,\theta_1,\theta_2}\left(\boldsymbol{x}_0\big|\boldsymbol{y}\right)\big\}
\end{align*}
with
\begin{align}\label{eq:post_mean}
\mu_{p,\theta_1,\theta_2}\left(\boldsymbol{x}_0\big|\boldsymbol{y}\right) = \widehat{\beta} + \boldsymbol{r}^{\mathsf{T}}\left(\boldsymbol{x}_0\right)\widetilde{\boldsymbol{R}}^{^{-1}}\left(\boldsymbol{y}-\widehat{\beta}\boldsymbol{1}_n\right)
\end{align}
and
\begin{align}\label{eq:post_var}
\sigma^2_{p,\theta_1,\theta_2}\left(\boldsymbol{x}_0\big|\boldsymbol{y}\right)
=
\widetilde{\sigma}^2\left[1-\boldsymbol{r}^{\mathsf{T}}\left(\boldsymbol{x}_0\right)\widetilde{\boldsymbol{R}}^{^{-1}}\boldsymbol{r}\left(\boldsymbol{x}_0\right)
+ \frac{\left\{1-\boldsymbol{1}_n^{\mathsf{T}}\widetilde{\boldsymbol{R}}^{^{-1}}\boldsymbol{r}\left(\boldsymbol{x}_0\right)\right\}^2}{\boldsymbol{1}_n^{\mathsf{T}}\widetilde{\boldsymbol{R}}^{^{-1}}\boldsymbol{1}_n}\right]\spc,
\end{align}
where again $\boldsymbol{r}\left(\boldsymbol{x}_0\right) = \boldsymbol{r}_{p,\theta_1,\theta_2}\left(\boldsymbol{x}_0\right) =
\left[\widetilde{R}\left(\boldsymbol{x}_0,\boldsymbol{x}_1\right),\ldots,\widetilde{R}\left(\boldsymbol{x}_0,\boldsymbol{x}_n\right)\right]^{\mathsf{T}}$.\\
So a random sample from the posterior predictive distribution
$\pi\left(y\left(\boldsymbol{x}_0\right)\big|\boldsymbol{y}\right)$ can be
drawn by translating each pair from the sample
$\left\{\big(\mu_{p,\theta_1,\theta_2}\left(\boldsymbol{x}_0\big|\boldsymbol{y}\right),\sigma^2_{p,\theta_1,\theta_2}\left(\boldsymbol{x}_0\big|\boldsymbol{y}\right)\big)\right\}$
(where each pair corresponds to a single triplet from
$\pi\left(p,\theta_1,\theta_2\big|\boldsymbol{y}\right)$ drawn as
described earlier) to a single draw from the posterior predictive distribution via a random normal generator.
A natural predictor would then be
\begin{align*}
\widehat{y}\left(\boldsymbol{x}_0\right) =
\mathbb{E}\left[y\left(\boldsymbol{x}_0\right)\big|\boldsymbol{y}\right] =
\mathbb{E}\left\{\mathbb{E}\left[y\left(\boldsymbol{x}_0\right)\big|\boldsymbol{y},p,\theta_1,\theta_2\right]\right\}
=
\mathbb{E}\left[\mu_{p,\theta_1,\theta_2}\left(\boldsymbol{x}_0\big|\boldsymbol{y}\right)\right]\spc
\end{align*}
and could be estimated by the sample average; in addition,
$100(1-\alpha)\%$ prediction intervals may be constructed using
the empirical $\alpha/2$ and $1-\alpha/2$ quantiles.
\begin{comment}
An example is given in Figure \ref{fig:post_pred} which plots a histogram of the posterior predictive distribution at a single site for one of the test functions discussed in Section \ref{Simulations}.
\end{comment}

\noindent For computational efficiency, note that (\ref{eq:logpost}) (evaluated in each M-H iteration) involves matrix inversions and matrix-vector products which are later used in (\ref{eq:post_mean}) and (\ref{eq:post_var}). Retaining those expressions on the fly is therefore essential for reasonable machine time. Also, in our implementation we performed the Geweke test (see \citealt{Geweke}) for convergence of the Markov chain every $50$ iterations (after a predetermined size - $1000$ in our case - had been obtained) to automatically halt the MCMC process.


\subsection{Anisotropic Processes}
When $d>1$ we can extend our approach to anisotropic processes by setting $\boldsymbol{\theta}_2 = (1 + \lambda)\boldsymbol{\theta}_1$ for $\lambda > 0$ (here $\boldsymbol{\theta}_1 = \left[\theta_1,\ldots,\theta_d\right]^{\mathsf{T}}$). A possible change of variables would now be
\begin{align*}
\psi = \log\dfrac{p}{1-p}\spc,\spc \varphi_i =
\log\theta_i\spc(1\leq i\leq d)\spc\text{and}\spc\eta = \log\lambda\spc,
\end{align*}
followed by the same steps as in the isotropic combined model, with the assigned joint prior now being $\pi\left(p,\boldsymbol{\theta},\lambda\right)$. Unlike the isotropic model (where the number of unknown parameters, $p$, $\theta_1$ and $\theta_2$, remains constant for all dimensions), here the number of parameters grows linearly in the number of dimensions.

\section{Simulation Results}\label{Simulations}
Here we consider four univariate and five bivariate
functions and compare the performance of the combined process model
suggested in Section \ref{Combined} to the ordinary Kriging method
described in Section \ref{GP} and the CGP method of \cite{CGP}
in terms of the mean squared prediction error and interval length,
under certain specifications of correlation structures and prior distributions.\\


\begin{example}\label{ex:univariate} (One Dimensional Examples)

\fontfamily{phv}\selectfont{
%**************************************************************************
%************* Some changes and re-ordering have been done ****************
\noindent Starting with the univariate case, we examine the
following functions:\\
$f_1(x)=\left(\sin10x+\cos15x\right)\Big/2$\spc,\spc
$f_2(x)=\sin\left(10x\right)$\spc,\spc\\
$f_3(x)=\sin\left(18x-9\right)\Big/\left(18x-9\right)$\spc
 and \spc
$f_4(x)=\mathrm{e}^{3x}\cos\left(5x-10\right)$\spc.\\

\noindent The correlation function in use for both processes in the Combined GP model
was Mat\'{e}rn with smoothness parameter $\nu=5$,
\begin{align}\label{matern}
R\left(h;\theta\right) = \frac{1}{16\Gamma\left(|h|\right)}\left(\frac{2\sqrt{5}|h|}{\theta}\right)^{5}K_{5}\left(\frac{2\sqrt{5}|h|}{\theta}\right)\spc,
\end{align}
where $K_{\nu}(\cdot)$ is the modified Bessel function of order $\nu$ and $h = x_1-x_2$.\\

\noindent We also examined the success of our model when combining Gaussian processes
with different correlation structures (as in \citealt{booker}). For that, we combined processes based on the Mat\'{e}rn correlation function (\ref{matern}) and the Nonnegative Cubic Spline correlation function
\begin{align*}
R\left(h;\theta\right) =
\begin{cases}
\begin{array}{ccc}
1 - 6\left(\dfrac{h}{\theta}\right)^2 + 6\left(\dfrac{|h|}{\theta}\right)^3 & &|h| \leq \dfrac{\theta}{2}\\[1em]
2\left(1 - \dfrac{|h|}{\theta}\right)^3 & &\dfrac{\theta}{2} < |h| \leq \theta\\[1em]
0 & & |h| > \theta
\end{array}
\end{cases}
\spc.
\end{align*}
The results for this model are listed in Table \ref{tab:summary} under `Two Families'.\\

\noindent In all examples
independent $\mathrm{U}(0,1)$, $\text{Inv-}\Gamma(3,2)$ and
$\text{Inv-}\Gamma(5,16)$ priors were assigned to $p$, $\theta_1$
and $\theta_2$, respectively, so that $\theta_1$ is the large-scale
parameter with $\mathbb{E}(\theta_1)=1$ and $\theta_2$ is the
small-scale parameter with $\mathbb{E}(\theta_2)=4$.
Good mixing of the resulting Markov chain is implied from \ref{MCMC_Diagnostics_Figures},
through both the autocorrelation plots and the trace plots.\\

\begin{figure}
  \centering
  \subfloat{\label{fig:MCMC1}\includegraphics[width=1\textwidth]{MCMC_Diagnostics1.pdf}}\\
  \subfloat{\label{fig:MCMC2}\includegraphics[width=1\textwidth]{MCMC_Diagnostics2.pdf}}
  \caption{Diagnostic plots for the MCMC sample drawn in the fitting process of $f_1(x)$.}
  \label{MCMC_Diagnostics_Figures}
\end{figure}



\noindent Each of the
above functions was approximated using all four methods (ordinary
Kriging, Combined GP, Two Families and CGP) $100$ times, based on random Latin
hypercube training designs consisting of $8$ points each in the
$[0,1]$ interval.  The empirical root
mean squared prediction error (RMSPE) was calculated on a fixed and
independent test set consisting of $50$ (uniformly spread) points and was averaged over $100$ trials.
Predictions and prediction intervals were based on $1000$ draws from
the posterior. Table \ref{tab:summary} presents RMSPE and interval coverage, with standard errors.
}
%**************************************************************************
%**************************************************************************




\begin{table}[ht!]
{\footnotesize
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 &Model &$f_1(x)$ &$f_2(x)$ &$f_3(x)$ &$f_4(x)$\\[0.5em]
\hline
\multirow{4}{*}{$\begin{array}{c}\text{Empirical}\\ \text{RMSPE}\end{array}$}
&Single GP &$.200\qq(.006)$ &$.067\qq(.006)$  &$.078\qq(.002)$ &$\textbf{.305\qq(.011)}$ \\
&Combined GP &$.114\qq(.004)$ &$\textbf{.047\qq(.002)}$  &$.077\qq(.002)$ &$.327\qq(.011)$ \\
&Two Families &$\textbf{.099\qq(.004)}$ &$.069\qq(.001)$  &$.151\qq(.002)$ &$1.217\qq(.009)$ \\
&CGP &$.258\qq(.005)$ &$.156\qq(.007)$  &$\textbf{.049\qq(.006)}$ &$.401\qq(.016)$ \\
\hline
\multirow{4}{*}{$\begin{array}{c}\text{$95\%$ PI}\\ \text{Coverage}\end{array}$}
&Single GP &$99.9\%\qq(.04)$ &$99.5\%\qq(.23)$  &$100\%$ &$86.3\%\qq(.25)$ \\
&Combined GP &$95.3\%\qq(.49)$ &$99.6\%\qq(.22)$  &$100\%$ &$87.8\%\qq(.23)$ \\
&Two Families &$99.1\%\qq(.34)$ &$100\%$  &$100\%$ &$100\%$ \\
&CGP &$93.9\%\qq(.63)$ &$98.6\%\qq(.40)$  &$100\%$ &$89.6\%\qq(.43)$ \\
\hline
\multirow{2}{*}{$\begin{array}{c}\text{Average}\\ \text{Quantile}\end{array}$} &Combined GP &$.498$ &$.491$ &$.489$ &$.492$\\
&Two Families &$.492$ &$.493$ &$.515$ &$.514$\\
\hline
$\begin{array}{c}\text{Relative}\\ \text{Improvement}\end{array}$ &Combined vs. Single &$42.9\%$ &$28.9\%$ &$1.6\%$ &$-7.2\%$\\
\hline
$\overline{\kappa}$ &$\overline{\hspace{2em}}$ &$9.77$ &$9.54$ &$5.97$ &$3.98$\\
\hline
\end{tabular}
\caption{Model comparison for the 1D simulation. Numbers in parentheses denote standard errors.}
\label{tab:summary}
}
\end{table}

\fontfamily{phv}\selectfont{
\noindent The relative improvement in RMSPE indicated in the table has an interesting relationship with
the average line curvature of the approximated function, denoted by
\begin{align}
\overline{\kappa} = \int_0^1\frac{\left|f''(x)\right|^2}{\left(1+f'(x)^{2}\right)^{3/2}}\hspace{0.1em}\di x\spc,
\end{align}
as it appears to be monotonically increasing with the latter,
hinting that the combined process becomes more effective as the
underlying function becomes more ``complex'' (i.e. with large values of $\overline{\kappa}$).
The combined process was clearly more successful in approximating $f_1(x)$ and $f_2(x)$,
but ordinary Kriging did better in predicting $f_4(x)$ values; the
two methods were about equally accurate for $f_3(x)$ (where the CGP model
was the outright winner).
Figure \ref{fig:predict_univariate} shows how the combined process model
manages to keep track of the changes in the behavior of $f_1(x)$.
The Two Families model displayed a more extreme behavior of the same
type, as it quite convincingly outperformed the others for the most volatile
function, $f_1(x)$, but became erratic (e.g. large prediction intervals, frequent
change of roles between the two components etc.) with the simpler underlying
functions. It is interesting to note that even in the most successful
simulations of $f_1(x)$ for the two families model, no authentic combination
of the two components was indicated.  Instead, there was
a single dominant component (i.e. $\pi\left(p|\boldsymbol{y}\right)$ was strongly
concentrated about either $0$ or $1$), suggesting the main benefit here was robustness with
respect to the choice of the correlation structure.
}

\begin{figure}[ht!]
\centering
\includegraphics[width=0.9\textwidth]{Func_1_plot.pdf}
\caption{Function $f_1(x)$ reconstruction from $8$ points. Shaded area: combined
process $95\%$ prediction intervals.}
  \label{fig:predict_univariate}
\end{figure}

\begin{comment}
\begin{figure}[ht!]
\centering
\includegraphics[width=.6\linewidth]{Post_Pred_Hist.png}
\caption{Histogram of a sample
from the posterior predictive distribution at a single site for the
function $f_1(x)$, along with the true and predicted values and the
$95\%$ prediction interval (from LL to UL).}
\label{fig:post_pred}
\end{figure}
\end{comment}

\end{example}


\noindent The row referring to interval coverage compares the proportion of
test points whose values were covered by the $95\%$ prediction
intervals (one may think of this as the proportion of test values
not situated in the extreme tails of the posterior predictive
distribution) produced by all models. For the first function, only the combined method had the desired level of coverage; its average interval length was also the shortest. All methods yielded over-coverage on the second and third functions; the combined method had the shortest interval lengths.  The fourth example led to under-coverage, except for the two families model, which had very wide intervals.  Another row in the table contains the average (empirical) quantile of the true values within the posterior predictive distribution of the combined process models. As desired, all were rather close to the median.

\begin{example}\label{examp:2d} (Two Dimensional Examples)
\fontfamily{phv}\selectfont{
\noindent We also used five bivariate functions to compare the performance of our
mixture model to standard kriging with a single Gaussian process and to CGP,
\begin{align*}
f_5\left(x_1,x_2\right)=\mathrm{e}^{-1.4x_1}\cos\left(\frac{7\pi x_1x_2}{2}\right)+\log\left(x_1+x_2+0.1\right)\spc,
\end{align*}
\begin{align*}
f_6\left(x_1,x_2\right)=\left[\left(x_1-0.2\right)^2 - \left(x_2-0.7\right)^2\right]\mathrm{e}^{-5\left[\left(x_1-0.8\right)^2+\left(x_2-0.1\right)^2\right]}\cos\big[\left(10x_1-5\right)x_2\big]\spc,
\end{align*}
\begin{align*}
f_7(\left(x_1,x_2\right)=\left[\left(x_1-0.5\right)^2 + 4\left(x_2-0.8\right)^2\right]\cdot\left[\cos\pi\left(x_1-0.1\right) + \cos\pi\left(x_2-0.5\right)\right]\spc,
\end{align*}
\begin{align*}
f_8\left(x_1,x_2\right)=\left[\sin(2x_1)+\cos(4x_1)\right]\cdot\left[\sin(8x_2)+\cos(4x_2)\right]
\end{align*}
and
\begin{align*}
f_9\left(x_1,x_2\right)=\frac{\sin\left(9x_1-4.5\right)\sin\left(12x_2-6\right)}{\left(9x_1-4.5\right)\left(12x_2-6\right)}\spc.
\end{align*}
Here Gaussian correlation functions of the form
\begin{align*}
R\left(\boldsymbol{u},\boldsymbol{v}\right) = \exp\left\{-\theta_1\left(u_1-v_1\right)^2-\theta_2\left(u_2-v_2\right)^2\right\}
\end{align*}
were used for all processes (ordinary Kriging, isotropic and anisotropic Combined GP).
Two isotropic processes, i.e.
\begin{align*}
R_i\left(\boldsymbol{u},\boldsymbol{v}\right) = \exp\left\{-\theta_i\left|\left|\boldsymbol{u}-\boldsymbol{v}\right|\right|^2\right\}\spc;\spc i=1,2\spc,
\end{align*}
were taken for the combined GP model with the same priors assigned to all parameters as in the univariate case.
The anisotropic combined process was based on two independent $\text{Inv-}\Gamma(3,2)$ priors for $\boldsymbol{\theta} = \left(\theta_1,\theta_2\right)$ and $\text{Inv-}\Gamma(3,4)$ prior for $\lambda$.\\

\noindent We used the \texttt{lhs} R package to generate $100$ size $14$ optimum Latin hypercube
designs (maximizing the average distance between any two design points) in $[0,1]^2$ and fit $100$ instances per model for all
functions. In addition, ordinary Kriging models were fit using the \texttt{mlegp} R package.
Root mean squared prediction error was then evaluated on a $25\times25$ lattice in the same region.\\

\noindent Figure \ref{2D_Reconstruction}
shows the prediction surface of $f_7\left(x_1,x_2\right)$ next to the real surface
and Figure \ref{2D_figure} plots $f_5\left(x_1,x_2\right)$ and $f_8\left(x_1,x_2\right)$ along
with predictions and prediction intervals constructed by the fitted
combined GP model.
}

\begin{figure}[ht!]
\centering
\includegraphics[width=0.9\textwidth]{Func4_3D_Reconstruction.png}
\caption{Reconstruction of the function $f_7\left(x_1,x_2\right)$ from a $14$ point
design using the combined process. The true surface appears in the left
panel, the estimate in the right panel.}
  \label{2D_Reconstruction}
\end{figure}


\begin{figure}
  \centering
  \subfloat[][]{\label{Func_1_3D}\includegraphics[width=0.37\textwidth]{Func_1_3D.png}}
  \subfloat[][]{\label{Func_5_3D}\includegraphics[width=0.52\textwidth]{Func_5_3D.png}}
  \caption{Left panel: $f_5\left(x_1,x_2\right)$ surface along with predictions (solid points) and $95\%$ prediction intervals obtained by fitting the combined process. Right panel: $f_8\left(x_1,x_2\right)$}
  \label{2D_figure}
\end{figure}

\noindent Table \ref{tab:2D_summary} summarizes the results of our simulations.
In four out of five cases the isotropic combined process improved the average prediction
error - while maintaining a
satisfactory level of coverage - compared to the standard Kriging
method. The case of $f_7\left(x_1,x_2\right)$ resembles that of $f_4(x)$ from
Example \ref{ex:univariate}, where the combined process model was
outperformed by standard Kriging in terms of mean squared prediction
error, but had the upper hand in terms of achieving nominal coverage
rates. Figure \ref{2D_Reconstruction} suggests that the graph of $f_7\left(x_1,x_2\right)$
is nearly planar.  This simple structure could perhaps explain why a single process would
suffice here, as with $f_4(x)$ in Example \ref{ex:univariate}. The case of $f_8\left(x_1,x_2\right)$ is an interesting one, as the
different frequencies along the axes somewhat resemble the notion of
anisotropy. It is thus not surprising that the anisotropic combined
process gave the best results for that function. In these examples
the CGP model was comparable to the others in terms of coverage,
but lagged behind as far as accurate prediction was concerned.





\begin{table}[ht!]
{\footnotesize
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 &Model &$f_5\left(x_1,x_2\right)$ &$f_6\left(x_1,x_2\right)$ &$f_7\left(x_1,x_2\right)$ &$f_8\left(x_1,x_2\right)$ &$f_9\left(x_1,x_2\right)$\\[0.5em]
\hline
\multirow{4}{*}{$\begin{array}{c}\text{Empirical}\\ \text{RMSPE}\end{array}$}
&$\begin{array}{c}\text{Single}\\[-.5em] \text{GP}\end{array}$ &$.240\qq(.007)$ &$.051\qq(.001)$  &$\textbf{.144\qq(.005)}$ &$.176\qq(.005)$ &$.114\qq(.006)$\\
\cline{2-7}
&$\begin{array}{c}\text{Comb.}\\[-.5em] \text{Iso.}\end{array}$ &$\textbf{.207\qq(.003)}$ &$\textbf{.038\qq(.001)}$ &$.186\qq(.006)$ &$.178\qq(.005)$ &$\textbf{.091\qq(.002)}$\\
\cline{2-7}
&$\begin{array}{c}\text{Comb.}\\[-.5em] \text{Aniso.}\end{array}$ &$.215\qq(.003)$ &$.043\qq(.001)$ &$.172\qq(.006)$ &$\textbf{.162\qq(.005)}$ &$.095\qq(.003)$\\
\cline{2-7}
&CGP &$.254\qq(.003)$ &$.045\qq(.001)$ &$.228\qq(.011)$ &$.309\qq(.009)$ &$.136\qq(.003)$\\
\hline
\multirow{4}{*}{$\begin{array}{c}\text{$95\%$ PI}\\ \text{Coverage}\end{array}$}
&$\begin{array}{c}\text{Single}\\[-.5em] \text{GP}\end{array}$ &$85.2\%\qq(1.8)$ &$83.0\%\qq(1.3)$ &$78.4\%\qq(1.6)$ &$90.1\%\qq(1.7)$ &$94.3\%\qq(1.1)$\\
\cline{2-7}
&$\begin{array}{c}\text{Comb.}\\[-.5em] \text{Iso.}\end{array}$ &$90.4\%\qq(0.8)$ &$88.9\%\qq(0.7)$ &$91.8\%\qq(0.5)$ &$98.2\%\qq(0.5)$ &$95.7\%\qq(0.6)$\\
\cline{2-7}
&$\begin{array}{c}\text{Comb.}\\[-.5em] \text{Aniso.}\end{array}$ &$92.4\%\qq(0.8)$ &$89.8\%\qq(0.7)$ &$92.1\%\qq(0.7)$ &$99.0\%\qq(0.4)$ &$97.3\%\qq(0.4)$\\
\cline{2-7}
&CGP &$89.7\%\qq(0.9)$ &$90.6\%\qq(0.6)$ &$92.4\%\qq(0.6)$ &$91.6\%\qq(1.4)$ &$96.3\%\qq(0.4)$\\
\hline
\end{tabular}
\caption{Model comparison for the 2D simulation.}
\label{tab:2D_summary}
}
\end{table}
\end{example}




\section{Tuning of the Hyperparameters}\label{hyperpars}
In the previous section we assigned nonnegative prior distributions to the correlation parameters, whose
purpose was to differentiate between the two processes. We considered using noninformative priors; however, these
attempts were unsuccessful, with failure of the MCMC routine. Care is
needed with such priors.  It has been demonstrated by \cite{berger} (and
further echoed by \citealt[chapter~3]{santner}) that improper priors (chosen for the
correlation parameters) may lead to improper posteriors. From similar considerations, it seemed
reasonable to require that the prior distributions have (at least) first and second moments, and that the correlation
parameter of the `volatile' process be centered at a value that is three or four times greater than
that of the `tame' process. In Example \ref{examp:2d}, for instance, the choice of
$\theta_1\sim\text{Inv-}\Gamma(3,2)$ and $\theta_2\sim\text{Inv-}\Gamma(5,16)$
ticked all the right boxes, since $\mathbb{E}\left[\theta_1\right] = 1$, $\mathbb{E}\left[\theta_2\right] = 4$ and
$\var\left[\theta_1\right] = 1$ is the largest possible variance for an inverse-gamma distribution about $1$
with integer hyperparameters, leaving enough room for variability. If, however, one is interested in
a more general (possibly automated) solution for choosing the hyperparameters for $\theta_1\sim\text{Inv-}\Gamma(\alpha_1,\beta_1)$
and $\theta_2\sim\text{Inv-}\Gamma(\alpha_2,\beta_2)$ (with the understanding that, for lack of
better a priori information, the prior distribution of $p$ remains uniform), one appealing option is an Empirical Bayes approach,
by choosing the quadruplet $\boldsymbol{\zeta}=(\alpha_1,\beta_1,\alpha_2,\beta_2)$ which maximizes the marginalized likelihood
\begin{align}\label{marg_like}
p\left(\boldsymbol{y};\boldsymbol{\zeta}\right) = \int p\left(\boldsymbol{y}\big|p,\boldsymbol{\theta};\boldsymbol{\zeta}\right)\pi\left(p,\boldsymbol{\theta};\boldsymbol{\zeta}\right)\di \left(p,\boldsymbol{\theta}\right)\spc.
\end{align}
Recall that $\boldsymbol{y}\big|\beta,p,\boldsymbol{\theta}\sim\mathcal{N}_n\left(\beta\boldsymbol{1}_n\hspace{.1em},\hspace{.1em}\widetilde{\sigma}^2\widetilde{\boldsymbol{R}}\right)$. Then, by assigning $\beta\sim\mathcal{N}\left(0,\tau^2\right)$ , it is easy to verify that $\boldsymbol{y}\big|p,\boldsymbol{\theta}\sim\mathcal{N}_n\Big(\boldsymbol{0}_n\hspace{.1em},\hspace{.1em}\widetilde{\sigma}^2\widetilde{\boldsymbol{R}} + \tau^2\boldsymbol{1}_n\boldsymbol{1}_n^{\mathsf{T}}\Big)$ , hence the integrand in (\ref{marg_like}) is the multivariate normal density with said parameters. It is thus obvious that letting $\tau\to\infty$ to have $\pi(\beta)\propto1$ would result in an improper marginal distribution. We therefore recommend setting $\tau$ to a large (yet finite) value.\\

\noindent For a given quadruplet of hyperparameters, $\boldsymbol{\zeta}$, evaluation of (\ref{marg_like}) can be carried out by importance
sampling, where sampling from $\pi\left(\boldsymbol{\theta};\boldsymbol{\zeta}\right)$ is particularly easy for independent priors
like the ones we use. However, the maximization of (\ref{marg_like}) with respect to $\boldsymbol{\zeta}$ is quite involved, and we
advise restricting attention to a finite, predefined set of `reasonable' quadruplets, over which the marginalized
likelihood is to be maximized.\\

\noindent To demonstrate these ideas, let us consider again the test functions of Example \ref{examp:2d}, and restrict ourselves to the set $\mathcal{A}$ of
$60$ quadruplets $(\alpha_1,\beta_1,\alpha_2,\beta_2)$ formed by
\begin{align*}
\begin{cases}
\alpha_1\in\left\{3,4,5,6,7\right\}\spc,\\
\beta_1 = \left(\alpha_1-1\right)/2,\spc \alpha_1-1\spc,\\
\alpha_2 = \alpha_1+2,\spc\alpha_1+3\spc,\\
\beta_2 = 2(\alpha_2-1),\spc 3(\alpha_2-1),\spc 4(\alpha_2-1)\spc.
\end{cases}
\end{align*}
A single $14$ run maximin LHD was used in this example, and the choice of the hyperparameters for each of the $5$ test functions was
based on $\displaystyle\argmax_{\zeta\in\mathcal{A}}p\left(\boldsymbol{y};\boldsymbol{\zeta}\right)$ . Interestingly enough, in all but one case - that of $f_7\left(x_1,x_2\right)$, where the selected hyperparameters were $(5,4,8,28)$ - the original choice of $(3,2,5,16)$ proved to have the upper hand; the results appear in Table \ref{tab:maximin_summary}. Identical results were obtained when the parameter $\tau$ was assigned a value of $30$, $50$ or $100$.
It is also worth mentioning that if we used the default $\boldsymbol{\zeta}=(3,2,5,16)$ for $f_7\left(x_1,x_2\right)$, the RMSPE would be $0.173$, compared to $0.163$ achieved by applying the above mentioned procedure, meaning that in this example
choosing the hyperparameters based on the marginalized likelihood proved useful.

\begin{table}[ht!]
{\footnotesize
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 &Model &$f_5\left(x_1,x_2\right)$ &$f_6\left(x_1,x_2\right)$ &$f_7\left(x_1,x_2\right)$ &$f_8\left(x_1,x_2\right)$ &$f_9\left(x_1,x_2\right)$\\[0.5em]
\hline
\multirow{3}{*}{$\begin{array}{c}\text{Empirical}\\ \text{RMSPE}\end{array}$}
&Single GP &$.376$ &$.081$  &$.155$ &$.131$ &$.113$\\
&Comb. Iso. &$.197$ &$.035$ &$.163$ &$.165$ &$.088$\\
&CGP &$.218$ &$.042$ &$.148$ &$.357$ &$.113$\\
\hline
\multirow{3}{*}{$\begin{array}{c}\text{$95\%$ PI}\\ \text{Coverage}\end{array}$}
&Single GP &$43.8\%$ &$76.0\%$ &$62.7\%$ &$100\%$ &$100\%$\\
&Comb. Iso. &$95.4\%$ &$97.3\%$ &$96.0\%$ &$100\%$ &$98.4\%$\\
&CGP &$96.6\%$ &$96.8\%$ &$86.4\%$ &$98.6\%$ &$96.0\%$\\
\hline
\end{tabular}
\caption{Model comparison after hyperparameters selection.}
\label{tab:maximin_summary}
}
\end{table}
%********************************************************************************************
%********************************************************************************************



\section{Applications}\label{sec:app}

\subsection{Ground Vibrations Simulation}\label{ex:gvs}


In this example we test our modelling approach on the data set from the study
of ground motion resulting from a strong earthquake (\citealt{Ground-vib})
performed at Tel Aviv University for the Israeli Ministry of
Infrastructure, and described in detail in Chapter \ref{intro}.\\

\noindent The experimental design used in the study was a $256$ point orthogonal
Latin hypercube, as described in \cite{orthogonal}. However, in $90$ runs
the frequency content of the signal was entirely absorbed, with no
consequent ground motion.  We limit our analysis here to the $166$ runs
that did result in surface acceleration. In addition, a $34$ point test
set was generated. We focus on the accelerations measured at a single location
on a slope for each configuration. \\

\noindent A rule of thumb suggests
that a training set should consist of about $10d$ points (where $d$ is the
dimension of the input space).  See \cite{Welch} for results in support
of this rule.  This suggests that our training set is a bit large and
that we might reserve a portion of it for testing purposes. We thus
fitted Combined GP, CGP and Ordinary Kriging models on training
sets of size $90$, repeating the process eight times, over random
subsets of points from the original design, and compared the three models by
RMSPE and interval coverage measured on a
test set consisting of the remaining $110$ points. A similar procedure was
carried out for training sets of size $50$, to see how the different models
perform with sparse training sets. The priors assigned to $p$,
$\theta_1$ and $\theta_2$ in this example were $\mathrm{U}(0,1)$, $\text{Inv-}\Gamma(3,1)$
and $\text{Inv-}\Gamma(5,75)$, respectively.\\


\noindent The results are shown in Table \ref{tab:GV}.
\begin{table}[ht!]
{\footnotesize
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Training Size &Model &RMSPE &$95\%$ PI Coverage\\[0.5em]
\hline
\multirow{3}{*}{$50$}
&Single GP &$2.985\qq(.090)$&$ 79.6\%\qq(3.4\%)$\\
&Combined GP &$2.895\qq(.100)$ &$95.1\%\qq(1.3\%)$\\
&CGP &$2.946\qq(.090)$ &$78.8\%\qq(4.0\%)$\\
\hline
\multirow{3}{*}{$90$}
&Single GP &$2.542\qq(.103)$&$87.4\%\qq(1.9\%)$\\
&Combined GP &$2.676\qq(.045)$ &$95.1\%\qq(0.6\%)$\\
&CGP &$2.392\qq(.079)$ &$89.2\%\qq(1.9\%)$\\\hline
\end{tabular}
\caption{Comparing the different emulators for the Ground Vibrations code.}
\label{tab:GV}
}
\end{table}
As one can see, the Combined GP handled the sparsity of the data slightly better than the
other two methods, but it was outpeformed (in terms of prediction) as the training size increased, with
the CGP model being the runaway winner. In terms of coverage, the Combined GP model was right
on the $95\%$ mark on both occasions, with both CGP and ordinary Kriging being too `optimistic'
and producing prediction intervals that were too short and suffered from under-coverage.\\

\noindent We offer some diagnostics, based
on the marginal posterior distributions of the Combined GP parameters, to help assess the
benefits of choosing the Combined GP as the modeling strategy: Figure \ref{fig:GV_Posteriors}
shows two different scenarios, both encountered while fitting the Combined GP emulator to the ground
vibrations code, based on different size $50$ training sets. Figure \ref{GV_Posteriors_Good} was obtained
when the RMSPE for the Combined GP was $2.543$, compared to $3.022$ by the ordinary Kriging model
(and $2.778$ by the CGP). The posterior distribution of the combination parameter $p$ is centered at
about $0.6$, implying an authentic need to combine both processes. Figure \ref{GV_Posteriors_Poor},
on the other hand, is a canonical example of a case in which avoiding the combined model is recommended:
$\pi\left(p|\boldsymbol{y}\right)$ is concentrated near $1$ and the posterior of $\theta_1$ resembles a spike at $0.2$,
meaning the second component, and the Bayesian setting as a whole, are likely to be redundant. It is thus little wonder
that the Combined GP model achieved an RMSPE of $2.923$ on that occastion, compared to
$2.689$ for ordinary Kriging.


\begin{figure}[ht!]
  \centering
  \subfloat[][]{\label{GV_Posteriors_Good}\includegraphics[width=1\textwidth]{Ground_Vibration_Posteriors.pdf}}\\
  \subfloat[][]{\label{GV_Posteriors_Poor}\includegraphics[width=1\textwidth]{Ground_Vibration_Posteriors_Poor.pdf}}
  \caption{The posterior distributions of the Combined GP parameters for two instances of size $50$ training sets of the ground vibrations simulation.}
  \label{fig:GV_Posteriors}
\end{figure}





\subsection{Heat Exchanger Simulation}

We proceed to test the Combined GP on the four dimensional computer simulation described
in \cite{Qian}. Here, the total rate of steady state heat transfer of a heat
exchanger for electronic cooling applications is modelled as a function
of the mass flow rate of entry air, the temperature of entry air, the solid material thermal
conductivity and the temperature of the heat source. The response was evaluated at a $64$-run
experimental design, constituting an orthogonal array-based LHD, and produced by a finite difference
code. An additional $14$ run test set was used to validate the resulting emulator.\\

\noindent \cite{Qian} reported a RMSPE of $2.59$ using a universal Kriging model (see \citealt[chapter~3]{santner}) with a linear trend, compared to $5.15$ achieved by ordinary Kriging, while
\cite{CGP} reduced the RMSPE to $2.24$.
We chose our hyperparameters from $624$ options, according to the method described in Section \ref{hyperpars}, given by
$$\left\{\left(\alpha_1,\beta_1,\alpha_2,\beta_2\right)\hspace{.15em}:\hspace{.15em}
\begin{array}{c}
\alpha_1=3,\ldots,9\\
\beta_1 = \left(\alpha_1-1\right)/2\\
3\leq\alpha_2 = \alpha_1-3,\ldots,\alpha_1+2\\
\beta_2 = 10\left(\alpha_2-1\right),\ldots,25\left(\alpha_2-1\right)
\end{array}
\right\}\spc.$$

\noindent The resulting prior distributions were $\theta_1\sim\text{Inv-}\Gamma(7,3)$ and $\theta_2\sim\text{Inv-}\Gamma(3,28)$, yielding a RMSPE of $1.97$ . However, in this example a choice of $\theta_1\sim\text{Inv-}\Gamma(3,1)$ and $\theta_2\sim\text{Inv-}\Gamma(5,104)$ achieved an even lower RMSPE of $1.93$ .\\

\noindent Figure \ref{Qian_Posteriors} provides us with positive diagnostics for the Combined GP model.
The posterior distribution of $p$ implies good mixing of the two components and the two other posterior
distributions show a fair degree of variability. Figure \ref{Qian_Predicted_vs_True} gives an assessment of the model's
performance, suggesting the Combined GP is a good fit for these data; the single outlier is a point on the boundary of the input space.


\begin{figure}[ht!]
  \centering
	\includegraphics[width=1\textwidth]{Qian_Posteriors.pdf}
  \caption{Posterior diagnostics for the heat exchanger simulation.}
  \label{Qian_Posteriors}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=0.55\textwidth]{Qian_Predicted_vs_True.pdf}
  \caption{Predictions versus true responses on an independent test set.}
  \label{Qian_Predicted_vs_True}
\end{figure}







%****************************************************************
%****************************************************************

\section{Adaptive Maximum Entropy Designs}\label{Batch_Sequential}

We now turn our attention to generating experimental designs that could
benefit from the Bayesian structure of model (\ref{eq:mixture}).
\textit{Maximum Entropy Designs}, experimental designs that maximize the
expected Shannon information gain, were introduced by \cite{Shewry}, and
their application to computer experiments was discussed by \cite{Sacks}.
We consider the \textit{batch sequential designs}, which consist of an
initial sample of size $n$ (for early learning and estimation of the
parameters) and a follow-up sample of size $m$ where the knowledge gained
from the initial sample can be exploited. \cite{Batch} considered several
optimization criteria for batch sequential designs, including batch
sequential maximum entropy designs.\\

\noindent In their paper, \cite{Shewry} showed that maximizing the expected information gain can be achieved by maximizing the determinant of the covariance matrix of the original vector of observations $\boldsymbol{y}$. They further showed that if the Gaussian process model is assumed, under some relaxations (see \citealt[chapter~6]{santner}) this is equivalent to maximizing the determinant of the correlation matrix $R$.\\


\noindent Consider the augmented correlation matrix
\begin{align*}
\renewcommand{\arraystretch}{1.4}
\text{
{\large
$
\boldsymbol{R}_{\text{aug}} =
\left[
\begin{array}{c|c}
\boldsymbol{R}^{\text{new}}_{\text{$m\times m$}} &\boldsymbol{R}^{\text{cross}}_{\text{$m\times n$}}\\
\hline
\boldsymbol{R}^{^\top\text{cross}}_{\text{$n\times m$}} &\boldsymbol{R}^{\text{old}}_{\text{$n\times n$}}\\
\end{array}
\right]
$ ,
}
}
\end{align*}
where $\boldsymbol{R}^{\text{old}}$ and $\boldsymbol{R}^{\text{new}}$ are the nested correlation matrices of the initial and follow-up samples, respectively, and $\boldsymbol{R}^{\text{cross}}$ is the matrix of cross-correlations. Taking advantage of the block matrix structure, a batch sequential maximum entropy design would be
\begin{align}\label{eq:batch-seq}
\mathcal{D}^{*} &= \displaystyle\argmax_{\mathcal{D}}\det\left(\boldsymbol{R}_{\text{aug}}\right) = \displaystyle\argmax_{\mathcal{D}}\left\{\det\left(\boldsymbol{R}^{\text{old}}\right)\cdot\det\left(\boldsymbol{R}^{\text{new}}-\boldsymbol{R}^{^\top\text{cross}}\boldsymbol{R}^{^{-1}\text{old}}\boldsymbol{R}^{\text{cross}}\right)\right\}\nonumber\\[1em]
&=
\displaystyle\argmax_{\mathcal{D}}\det\left(\boldsymbol{R}^{\text{new}}-\boldsymbol{R}^{^\top\text{cross}}\boldsymbol{R}^{^{-1}\text{old}}\boldsymbol{R}^{\text{cross}}\right)\spc,
\end{align}
and the optimization problem thus reduces to maximizing the determinant
of a more reasonable $m\times m$ matrix.\\


\noindent Our design algorithm takes advantage of the results in Section
\ref{Combined}, where we provided the recipe for drawing samples
$\left\{(p,\theta_1,\theta_2)\right\}$ from the posterior
$\pi\left(p,\theta_1,\theta_2\big|\boldsymbol{y}\right)$. We consider two
design approaches: (1) apply (\ref{eq:batch-seq}) to
$\widetilde{R}_{\widehat{p},\widehat{\theta}_1,\widehat{\theta}_2}$ using
a summary of the center of the posterior, say, the posterior mean or the maximum a
posteriori estimator $\left(\hat{p},\hat{\theta}_1,\hat{\theta}_2\right)$
based on (\ref{eq:logpost}), or (2) draw a random sample of batch
sequential maximum entropy designs by generating an optimal design
$\mathcal{D}^{*}_{p,\theta_1,\theta_2}$ for each triplet
$(p,\theta_1,\theta_2)$ from our sample and then summarizing the points
in that collection of designs (for example by using cluster analysis as
in \citealt{Dror}).




\begin{example}\label{Ex:ME_Design}\text{}

\fontfamily{phv}\selectfont{
We applied both above described methods to generate batch sequential
maximum entropy designs on $[-1,1]^2$ for the function $f_6\left(x_1,x_2\right)$ from
Example \ref{examp:2d}. The initial design was a $14$ point maximum
entropy design based on the prior mean ($p=0.5$, $\theta_1=1$ and
$\theta_2=4$) and $7$ new points were chosen as a follow-up sample
according to (\ref{eq:batch-seq}), first by plugging in the posterior mean estimator
$(0.174, 1.448, 5.937)$ and later for each of the $1000$ triplets drawn
from the posterior distribution (to a total of $7000$ points). In the
second method, to choose the eventual secondary design we applied
$k$-medoids clustering, using $k=7$. The resulting designs (which bear
some resemblance) can be seen in Figure \ref{fig:ME_Designs}, and
prediction and inference results appear in Table \ref{tab:ME_summary}.
Our comparison includes the two maximum entropy designs and a $21$ run
optimum Latin hypercube and data from each design were modeled both by
the combined GP and ordinary Kriging models. The best results were
obtained when the MAP estimator design was used in combination with the
combined GP model.  However, that was the least efficient design when
using ordinary Kriging.
}


\begin{figure}[ht!]
\centering
\includegraphics[width=.85\textwidth]{Clust_and_Plugin_ME_Designs.pdf}
  \caption{Left panel: Batch sequential Maximum Entropy design obtained by k-medoids clustering. Left panel: Batch sequential Maximum Entropy design obtained by plugging in the posterior means of the parameters.}
  \label{fig:ME_Designs}
\end{figure}

\begin{table}[ht!]
\begin{threeparttable}
{\footnotesize
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Design &$\begin{array}{c}\text{RMSPE}\\ \text{Single}\end{array}$ &$\begin{array}{c}\text{RMSPE}\\ \text{Combined}\end{array}$ &$\begin{array}{c}\text{RMSPE}\\ \text{CGP}\end{array}$ &$\begin{array}{c}\text{Coverage}\\ \text{Single}\end{array}$ &$\begin{array}{c}\text{Coverage}\\ \text{Combined}\end{array}$ &$\begin{array}{c}\text{Coverage}\\ \text{CGP}\end{array}$\\[0.3em]
\hline
$\begin{array}{c}\text{K-medoids}\\ \text{ME}\end{array}$ &$.051$ &$.040$ &$.042$ &$84.5\%$ &$94.9\%$ &$91.7\%$\\[.2em]
\hline
$\begin{array}{c}\text{Plug In}\\ \text{ME}\end{array}$ &$.058$ &$.033$ &$.041$ &$82.2\%$ &$96.3\%$ &$91.8\%$\\[.2em]
\hline
$\begin{array}{c}\text{Optimum}\\ \text{LHD}^*\end{array}$ &$.056\qq(.001)$ &$.041\qq(.001)$ &$.045\qq(.001)$ &$85.4\%\qq(.9)$ &$91.9\%\qq(.5)$ &$91.9\%\qq(.5)$\\[.2em]
\hline
$\begin{array}{c}\text{Maximin}\\ \text{LHD}\end{array}$ &$.036$ &$.036$ &$.040$ &$92.2\%$ &$90.2\%$ &$92.3\%$\\[.2em]
\hline
\end{tabular}
    \begin{tablenotes}
      \footnotesize
      \item $^*$ Over $100$ repetitions.
    \end{tablenotes}
\caption{Prediction and coverage comparison for experimental designs}
\label{tab:ME_summary}
}
\end{threeparttable}
\end{table}

\fontfamily{phv}\selectfont{
\noindent Figure \ref{fig:Priors_and_Posteriors} tracks the changes in the (marginal) posteriors after each stage when using the MAP batch sequential ME design. Note that after the second stage $\pi\left(p\big|\boldsymbol{y}\right)$ seems to be strongly concentrated near zero, yet the small contribution of the small-scale process proved useful in modelling $f_6\left(x_1,x_2\right)$, as evident from Table \ref{tab:ME_summary}. That could perhaps be partly explained by the relatively large variability of (the dominant parameter) $\theta_2$, in contrast to Figure \ref{GV_Posteriors_Poor}, where
 - in addition to the poor mixing of the two components - the dominant parameter $\theta_1$ seemed nearly fixed at a single value, deeming the entire Bayesian model unnecessarily rich. Contour plots of the approximated surface after each stage are displayed in Figure \ref{fig:ME_Contour_Plots}.
}
\begin{figure}[ht!]
\centering
\includegraphics[width=1\textwidth]{Priors_and_Posteriors.pdf}
\caption{Prior and posterior distributions after each stage.}
  \label{fig:Priors_and_Posteriors}
\end{figure}



\begin{figure}[ht!]
\centering
\includegraphics[width=1\textwidth]{ME_Contour_Plots.pdf}
\caption{Contour plots of the approximated surface after each stage, compared to the true contours on the right panel.}
  \label{fig:ME_Contour_Plots}
\end{figure}

\end{example}



\section{Discussion}\label{Discussion}
We have developed and implemented a Gaussian process model
which extends the standard Kriging model that has become a
popular choice to model the output of computer experiments.
Our simulation results suggest that combining Gaussian processes of different scales could improve both the prediction and coverage properties of the ordinary Kriging method, in particular when the underlying function displays nonhomogeneous behavior across different regions of the input space.\\

\begin{comment}
\noindent The decision to combine and calibrate the two Gaussian processes in a Bayesian fashion also provides us with reasonable ways to generate batch sequential experimental designs. In this work, we demonstrated these ideas by generating Maximum Entropy designs, but the same ideas could serve for the generation of any experimental design in which specification of parameters is essential (e.g. Minimum Integrated Mean Squared Error designs, see \citealt{IMSE} for details).\\
\end{comment}

\noindent In Example \ref{Ex:ME_Design}, most of the ``mass'' was placed on the
small scale process, whose correlation decays rapidly.
In the reverse case, in which the correlation function of the fitted ordinary Kriging
model is the one that decays slowly, the Gram matrix $\boldsymbol{R}$ tends to become
computationally singular very fast as the number of inputs increases. Under these
circumstances, even a small contribution of the small scale process could improve the
conditioning of $\boldsymbol{R}$ dramatically, similar to the effect of the nugget term
(see \citealt{nugget}). Indeed, throughout a large number of simulations performed for this work,
not once did the combined model malfunction due to ill-conditioning. The problem of improving
the computational stability of the Gaussian process interpolator has also been the subject of  works by \cite{booker} and \cite{ranjan}.\\

\begin{comment}
\noindent It is also natural to consider the extension of model (\ref{GRF}) to
more complicated models that involve a combination of more than two processes.
Such a model should be carefully probed, as the increased flexibility comes
at the expense of additional parameters to be calibrated and added
computational complexity. To emphasize the latest point, we note
that in both applications of Section \ref{sec:app} the anisotropic
Combined GP model proved unsuccessful compared to other modeling approaches
discussed in this work, possibly due to overparameterization.\\
\end{comment}

\noindent A valid question can be raised regarding the effectiveness of the model for moderate to large
training sets. For example, we used a $100$ run maximin LHD to fit the different models of Example
\ref{examp:2d} to $f_6\left(\boldsymbol{x}_1,\boldsymbol{x}_2\right)$. The results appear in Table \ref{tab:Large_Data}, from which
it is obvious that the Combined GP model (isotropic or anisotropic) has no advantage over the ordinary Kriging model this time.

\begin{table}[ht!]
{\footnotesize
\centering
\begin{tabular}{|c|c|c|}
\hline
Model &RMSPE &$95\%$ PI Coverage\\[0.5em]
\hline
Single GP &$.0034$&$ 93.9\%$\\
\hline
Combined Iso. &$.0036$ &$94.9\%$\\
\hline
Combined Aniso. &$.0034$ &$96.8\%$\\
\hline
CGP &$.0074$ &$98.2\%$\\
\hline
\end{tabular}
\caption{Testing the different models on $f_6\left(\boldsymbol{x}_1,\boldsymbol{x}_2\right)$ for a $100$ runs maximin LHD.}
\label{tab:Large_Data}
}
\end{table}
\noindent It is our conjecture that, while the richer structure makes up for limited data, its contribution is limited in the
presence of many observations selected using a space filling design, where the standard Kriging method is both simple and effective.  There may be advantages when the data have local clusters in parts of the space, as often happens when function calls are embedded in an optimization algorithm \citep{booker}. 

==> Chapters/Conclusion.tex <==
\section{General Comments}

\noindent Throughout this work, many calculations involved the inversion of the correlation matrix, $\boldsymbol{R}$. While the addition of a nugget term to the model improves the conditioning dramatically, the need to invert a dense matrix creates a real bottleneck in computationally intensive methods - like the ones presented in this work - especially when large datasets are concerned. In recent years, it has become customary to enforce sparsity on $\boldsymbol{R}$ through \textit{tapering} (i.e. zeroing the covariance between locations outside a neighborhood of a predetermined radius). \cite{Nychka1} and \cite{Kaufman} discuss these ideas in full length. \cite{Nychka1} uses Gaussian Markov random fields of multiple resolutions to approximate smooth correlation structures via an ensemble of random processes whose precision matrices are sparse.\\

\noindent The implementation of every single method presented in Chapters \ref{Combined_GP}, \ref{Optimal_GP_Designs} and \ref{GP_Variable_Selection}
has been done in the statistical software \textbf{\textsf{R}}. The code for these chapters is available online, on \href{https://sites.google.com/site/ofirhararishomepage/software}{{\color{blue}\underline{sites.google.com/site/ofirhararishomepage/software}}}.

\section{Future Work}

\noindent In Chapter \ref{Combined_GP}, the decision to combine and calibrate the two Gaussian processes in a Bayesian fashion also provides us with reasonable ways to generate batch sequential experimental designs. In this work, we demonstrated these ideas by generating Maximum Entropy designs, but the same ideas could serve for the generation of any experimental design in which specification of parameters is essential (e.g. Minimum Integrated Mean Squared Prediction Error designs, see \citealt{IMSE} for details).\\


\noindent It is also natural to consider the extension of the Combined GP model (\ref{GRF}) to
more complicated models that involve a combination of more than two processes.
Such a model should be carefully probed, as the increased flexibility comes
at the expense of additional parameters to be calibrated and added
computational complexity. To emphasize the latest point, we note
that in both applications of Section \ref{sec:app} the anisotropic
Combined GP model proved unsuccessful compared to other modeling approaches
discussed in this work, possibly due to overparameterization.\\

\noindent Regarding the optimal designs of Chapter \ref{Optimal_GP_Designs}, it would be interesting to see how such designs are affected by
the assignment of prior distributions to circumvent the need to specify values for the correlation parameters. A clustering procedure, like the one
proposed in Section \ref{Batch_Sequential}, could then follow to choose a particular design out of infinitely many candidates. Likewise, a multi-stage
construction may be considered, where Bayesian update and plug-in of Bayesian estimators take place.\\

\noindent In Chapter \ref{GP_Variable_Selection}, ideally, we would like to take advantage of
the Bayesian framework to provide accurate predictions, using the model averaging formula (\ref{eq:pred_averaged}). However, using model averaging to a good effect might require
an educated choice of prior distributions, along with possibly vast samples from the posterior distributions. One very interesting open question is whether a set of sparsity prior distributions exists, such that under some aggregation methods, the minimax convergence rate of the mean squared prediction error can be achieved, as in the exponential weighting scheme of \cite{Tsybakov} for linear regression models.\\

\noindent One question left unanswered in Chapter \ref{GP_Variable_Selection}, and which may be the basis for future research, is whether or not one should add some linear terms for extrapolation purposes, even when the selection process indicates otherwise. Based on the artificial example of Section \ref{sec:bayes_var_simulation}, it looks very likely that the model will toss most of the regression functions and rely on the covariance kernel. It would therefore be interesting to see if this would have a devastating effect on predictions outside the convex hull of the training data. 

==> Chapters/GP_Variable_Selection.tex <==
\section{Introduction}
\begin{comment}
\noindent Gaussian processes have been employed extensively both in regression and classification problems in machine learning (see \citealt{Rasmussen}).
While their earliest use in statistical modeling may have been in geostatistics (see e.g. \citealt{Cressie})
it has been the most popular metamodeling approach to computer simulations (see \citealt[chapter~3]{santner}).\\
\end{comment}

\noindent The problem of variable selection in Gaussian process regression has been addressed by \cite{Bingham}, while \cite{Vannucci}
extended their results to generalized linear nonparametric models. In both cases no regression terms were included, and dependence on the factors was modeled by the authors solely
via the spatial correlation structure.\\




\noindent In many applications only interpolation or smoothing are required,
and the omission of regression terms can simplify the fitting of the Kriging metamodel,
with little expense in predictive precision (see e.g. \citealt{IMSE}).  It is also known that these models have
a strong ``Kriging towards the mean'' tendency at sites far away from the training data, and it is thus
often essential to add a trend for effective extrapolation (see \citealt{trend} for the original argument). Currently,
the common practice is to either include all of the covariates both in the correlation structure and the linear component (i.e. {\it Universal Kriging}) or to omit the linear part altogether and model the data as observations from a pure (weakly) stationary random process (i.e. {\it Ordinary Kriging}). \cite{BlindKrig} proposed a Bayesian procedure for designed computer experiments, to select first- and second-order polynomials for the mean surface while leaving the covariance terms untouched. In this chapter we allow for exclusion of covariates from the correlation structure, along with their possible inclusion in the trend component, in the case that their only contribution to the output is linear.



\section{Model Assumptions}
\noindent Let $\left\{\boldsymbol{x}_1,\ldots,\boldsymbol{x}_n\right\}\subset\mathcal{X}$ be our training set, where $\mathcal{X}\subset\mathbb{R}^p$ is the experimental region, and let $\boldsymbol{y} = \left[y\left(\boldsymbol{x}_1\right),\ldots,y\left(\boldsymbol{x}_n\right)\right]^{\mathsf{T}}$ be a vector of observations from the model
\begin{align}\label{eq:model}
y\ofx = \beta_0 + \bx^{\mathsf{T}}\boldsymbol{\beta} + Z\ofx + \varepsilon\ofx\spc,
\end{align}
where $\beta_0$ is a constant, $\boldsymbol{\beta} = \left[\beta_1,\ldots,\beta_p\right]^{\mathsf{T}}$ is a vector of regression coefficients, $Z\ofx$ is a zero mean stationary Gaussian process with marginal variance $\sigma^2_{_Z}$ and a separable correlation function of the form
\begin{align}\label{eq:corr_func}
R\left(\boldsymbol{u},\boldsymbol{v};\boldsymbol{\rho}\right) = \prod_{k=1}^p\rho_j^{\left(u_k-v_k\right)^2}
\end{align}
for some vector of correlation parameters $\boldsymbol{\rho} = \left[\rho_1,\ldots,\rho_p\right]^{\mathsf{T}}$, $0\leq\rho_j\leq1$ , $1\leq j\leq p$, and $\varepsilon\ofx$ is a white noise process, independent of $Z\ofx$, with variance parameter $\sigma^2_{\varepsilon}$. Note that the closer $\rho_j$ is to $1$, the less $Z\ofx$ tends to vary in the $j$th direction, and vice versa. This point is illustrated in Figure \ref{fig:3D_Realization}, in which a single realization of $Z\ofx$ is drawn, for a relatively large value of $\rho_1$ and an extremely small value of $\rho_2$.\\

\begin{figure}[ht]
  \centering
 \includegraphics[width=.65\textwidth]{2D_Realization_2.pdf}
  \caption{A realization of $Z\ofx$ with the correlation function (\ref{eq:corr_func}), for $\rho_1= 0.75$ and $\rho_2=5\times10^{-6}$.}
  \label{fig:3D_Realization}
\end{figure}

\noindent Denoting $\lambda = \sigma^2_{\varepsilon}/\sigma^2_{_Z}$, it can be easily verified that
\begin{align}\label{eq:likelihood}
\by\big|\beta_0,\boldsymbol{\beta},\sigma^2_{_Z},\br,\lambda\sim\mathcal{N}\left\{\beta_0\boldsymbol{1}_n + \boldsymbol{X}\boldsymbol{\beta}\hspace{.1em},\hspace{.1em}\sigma^2_{_Z}\left[\boldsymbol{R}\left(\br\right)+\lambda\boldsymbol{I}\right]\right\}\spc,
\end{align}
where $\boldsymbol{X}$ is the design matrix and $\boldsymbol{R}_{ij}\left(\br\right) = R\left(\bx_i,\bx_j\right) = \displaystyle\prod_{k=1}^p\rho_k^{(\bx_{ik}-\bx_{jk})^2}$.\\

\noindent We can interpret (\ref{eq:model}) as follows: each of the $p$ covariates in $\bx$ may (or may not) make a linear contribution to the response $y\ofx$. If, in addition, it makes a nonlinear contribution, it should be captured by $Z\ofx$, whose flexible nature makes it free of any rigid structure. The white noise term, also known as the ``nugget'' (see \citealt{nugget}) and interpreted as ``measurement error'', is often omitted when using the Kriging metamodel to emulate deterministic computer simulations. However, its (possibly unnatural) inclusion has certain benefits, both numerical and in terms of the average squared prediction error. The consequent $\lambda$ term in (\ref{eq:likelihood}) is mostly
identified with the equivalent penalized least squares minimization problem in the Reproducing Kernel Hilbert Space corresponding to $R(\cdot,\cdot)$ (see \citealt{Wahba}). In this chapter, we would like to examine the possibility of leaving some of the covariates out of the correlation function. By doing that, we deliberately omit variables that are (in the case of computer experiments) known for a fact to be part of the computer code. It is then reasonable to add an error term, to avoid interpolation at the learning set, in favor of better predictions at new sites.


\section{Formalizing as a Bayesian Model}\label{sec:Bayesian}
\noindent We would now like to turn our attention to the problem of variable selection in model (\ref{eq:model}). Research on Bayesian variable selection in linear regression models has been thoroughly documented - \cite{Chipman} give a detailed account of some theoretical and computational aspects and \cite{Felix} explore the case in which $n>p$. Conversely, \cite{Bingham} and \cite{Vannucci} apply point-mass mixture prior distributions for the correlation parameters of simple Kriging models.
In this chapter, we aim to propose a unified framework, in which ``spike-and-slab'' priors, like those used by \cite{Bingham} and \cite{Vannucci}, are employed to select the components of both the structural and spatial parts of the model.


\subsection{The Posterior Distribution}
\noindent To put the above to practice, we now assume that the regression coefficients are independent, with prior distributions
\begin{align}\label{eq:beta_prior}
\beta_j\big|\omega_r \sim \omega_r\mathcal{N}\left(0,\tau^2\right) + \left(1-\omega_r\right)\delta_0\spc,
\end{align}
where $\delta_0$ is a point mass at zero. Alternatively, one can denote by $\bgamma^r=\left(\gamma^r_1,\ldots,\gamma^r_p\right)$ a vector of latent variables, in which $\gamma^r_j=\mathbbm{1}\left\{\beta_j\ne0\right\}$ indicates whether or not the $j$th covariate is included in the linear component. We may then write $\gamma^r_j\big|\omega_r\sim\mathrm{Binom}\left(1,\omega_r\right)$ and $\beta_j\big|\gamma^r_j\sim\mathcal{N}\left(0,\gamma^r_j\tau^2\right)$ .\\


\noindent Regarding the spatial component, for the $j$th variable to be inert, its corresponding correlation factor $\rho_j$ must be equal to $1$. An analogue of (\ref{eq:beta_prior}) would then be
\begin{align}\label{eq:rho_prior}
\rho_j\big|\omega_c\sim \omega_c\hspace{.1em}\mathcal{U}(0,1) + \left(1-\omega_c\right)\delta_1\spc,
\end{align}
implemented by defining the latent variables $\bgamma^c=\left(\gamma^c_1,\ldots,\gamma^c_p\right)$, where $$\gamma^c_j\big|\omega_c\sim\mathrm{Binom}\left(1,\omega_c\right)\spc\text{and}\spc \pi\left(\rho_j\big|\gamma^c_j\right) = \gamma^c_j\hspace{.1em}\mathcal{U}(0,1) + \left(1-\gamma^c_j\right)\delta_1\left(\rho_j\right)\spc.$$


\noindent Using Bayes rule, we may now write the posterior distribution
\begin{align}\label{eq:posterior}
p&\left(\bgamma^r,\bgamma^c,\omega_r,\omega_c,\beta_0,\boldsymbol{\beta},\br,\sigma^2_{_Z},\lambda\big|\by\right)\nonumber\\[1em]
 &\propto p\left(\by\big|\beta_0,\boldsymbol{\beta},\sigma^2_{_Z},\br,\lambda\right)\pi\left(\bgamma^r,\boldsymbol{\beta}\big|\omega_r\right)\pi\left(\bgamma^c,\br\big|\omega_c\right)\pi\left(\beta_0,\sigma^2_{_Z},\lambda,\omega_r,\omega_c\right)\spc,
\end{align}
where $p\left(\by\big|\beta_0,\boldsymbol{\beta},\sigma^2_{_Z},\br,\lambda\right)$ is the multivariate Normal density, as indicated in (\ref{eq:likelihood}),
\begin{align*}
\pi\left(\bgamma^r,\boldsymbol{\beta}\big|\omega_r\right) = \omega_r^{\sum_{j}\mathbbm{1}\left\{\gamma^r_j=1\right\}}\left(1-\omega_r\right)^{\sum_{j}\mathbbm{1}\left\{\gamma^r_j=0\right\}}\prod_{\gamma^r_j=1}\phi_{\tau}\left(\beta_j\right)
\end{align*}
(here $\phi_{\tau}\left(\beta_j\right)$ is the Normal pdf with zero mean and standard deviation $\tau$, evaluated at $\beta_j$) and
\begin{align*}
\pi\left(\bgamma^c,\boldsymbol{\rho}\big|\omega_c\right) = \omega_c^{\sum_{j}\mathbbm{1}\left\{\gamma^c_j=1\right\}}\left(1-\omega_c\right)^{\sum_{j}\mathbbm{1}\left\{\gamma^c_j=0\right\}}\spc.
\end{align*}

\subsection{Markov Chain Monte Carlo Sampling from the Posterior Distribution}\label{sec:MCMC}
\noindent We now apply a Metropolis Sampling algorithm to draw a random sample from the posterior distribution. A
suitable `jump' (or `proposal') distribution is required - one that will allow the resulting Markov chain to arrive at any
possible state with positive probability. Here we extend the key ideas of \cite{Vannucci}, to propose a full Metropolis-Hastings scheme:
\begin{enumerate}
\item
Update $\left(\bgamma^r,\boldsymbol{\beta}\right)$ and $\left(\bgamma^c,\boldsymbol{\rho}\right)$ : draw $k\in\left\{0,1,\ldots,2p\right\}$
from a $\mathrm{Binom}(2p,\nu)$ distribution (typically $\nu=\left(2p\right)^{-1}$) and change the present state of $k$ randomly chosen latent variables out of
$\left(\bgamma^r,\bgamma^c\right)$.
\begin{itemize}
\item[-]
If the value of $\gamma_j^r$ changes from $0$ to $1$, sample $\tilde{\beta}_j$ from a $\mathcal{N}\left(0,\tau^2\right)$ proposal.
\item[-]
If the value of $\gamma_j^c$ changes from $0$ to $1$, sample $\tilde{\rho}_j$ from a $\mathcal{U}(0,1)$ proposal.
\item[-]
If the value of $\gamma_j^r$ changes from $1$ to $0$, set $\tilde{\beta}_j=0$. This results in covariate
$\bx_j$ being omitted from the linear trend in the current iteration.
\item[-]
If the value of $\gamma_j^c$ changes from $1$ to $0$, set $\tilde{\rho}_j=1$. This results in covariate
$\bx_j$ being omitted from the correlation function in the current iteration.
\item[*]
In any of the above cases, add a small jitter to the remaining $\beta$ and $\rho$ values (while making sure all the $\rho_j$-s remain in the interval $(0,1)$).
\end{itemize}
\item
Update $\left(\beta_0,\sigma^2_{_Z},\lambda,\omega_r,\omega_c\right)$ : to simplify matters, transform the parameters to $$\mu = \log\left(\sigma^2_{_Z}\right) \spc;\spc \zeta = \log(\lambda)\spc;\spc \psi_r = \log\frac{\omega_r}{1-\omega_r}\spc\text{and}\spc\psi_c = \log\frac{\omega_c}{1-\omega_c}\spc,$$ and sample $(\tilde{\beta}_0,\tilde{\mu},\tilde{\zeta},\tilde{\psi}_r,\tilde{\psi}_c)$ from a multivariate Normal distribution about the present state, $(\beta_0,\mu,\zeta,\psi_r,\psi_c)$ . Remember to take the Jacobian term $$\dfrac{\partial\left(\sigma^2_{_Z},\lambda,\omega_r,\omega_c\right)}{\partial{\left(\mu,\zeta,\psi_r,\psi_c\right)}} = \mu\hspace{.1em}\zeta\hspace{.1em}\omega_r(1-\omega_r)\hspace{.1em}\omega_c(1-\omega_c)$$ into account in the posterior later.
\item
The proposed vector $\left(\tilde{\bgamma}^r,\tilde{\boldsymbol{\beta}},\tilde{\bgamma}^c,\tilde{\boldsymbol{\rho}},\tilde{\beta}_0,\tilde{\sigma}^2_{_Z},\tilde{\lambda},\tilde{\omega}_r,\tilde{\omega}_c\right)$ is accepted with probability
\begin{align}\label{eq:accept}
\alpha = \min\left\{1\hspace{.1em},\hspace{.1em}\dfrac{p\left(\tilde{\bgamma}^r,\tilde{\bgamma}^c,\tilde{\beta}_0,\tilde{\boldsymbol{\beta}},\tilde{\br},\tilde{\sigma}^2_{_Z},\tilde{\lambda},\tilde{\omega}_r,\tilde{\omega}_c\big|\by\right)}{p\left(\bgamma^r,\bgamma^c,\beta_0,\boldsymbol{\beta},\br,\sigma^2_{_Z},\lambda,\omega_r,\omega_c\big|\by\right)}\right\}\spc.
\end{align}
Note that (\ref{eq:accept}) holds, since by construction, the proposal distribution described above is symmetric, i.e. $$p\left(\tilde{\bgamma}^r,\tilde{\boldsymbol{\beta}},\tilde{\bgamma}^c,\tilde{\br}\big|\bgamma^r,\boldsymbol{\beta},\bgamma^c,\br\right) = p\left(\bgamma^r,\boldsymbol{\beta},\bgamma^c,\br\big|\tilde{\bgamma}^r,\tilde{\boldsymbol{\beta}},\tilde{\bgamma}^c,\tilde{\br}\right)$$ and $$p\left(\tilde{\beta}_0,\tilde{\sigma}^2_{_Z},\tilde{\lambda}\big|\beta_0,\sigma^2_{_Z},\lambda\right) = p\left(\beta_0,\sigma^2_{_Z},\lambda,\omega_r,\omega_c\big|\tilde{\beta}_0,\tilde{\sigma}^2_{_Z},\tilde{\lambda},\tilde{\omega}_r,\tilde{\omega}_c\right)\spc.$$
\end{enumerate}


\section{Prediction Strategies}\label{sec:prediction}
\noindent We now wish to take advantage of the procedure described in Section \ref{sec:MCMC}, to make accurate predictions at $m$ new sites $\boldsymbol{X}_{\text{new}}$ . We will propose two possible approaches, the first of which - based on model averaging -  is a more ``orthodox'' Bayesian approach, while the second one, in which we merely use the ideas of Section \ref{sec:MCMC} to identify the MAP model, might be characterized as opportunistic.

\subsection{Prediction based on Model Averaging}
\noindent Conditional on $\boldsymbol{\Theta} = \left(\beta_0,\boldsymbol{\beta},\br,\sigma^2_{_Z},\lambda\right)$, the joint distribution of $\boldsymbol{y}_{\mathrm{old}} = y\left(\boldsymbol{X}_{\mathrm{old}}\right)$ and $\boldsymbol{y}_{\mathrm{new}} = y\left(\boldsymbol{X}_{\mathrm{new}}\right)$ is given by
\begin{align*}
\left[
\begin{array}{c}
\boldsymbol{y}_{\mathrm{new}}\\
\hline
\boldsymbol{y}_{\mathrm{old}}
\end{array}
\right]=
\mathcal{N}\left\{\left[
\begin{array}{c}
\beta_0\boldsymbol{1}_m + \boldsymbol{X}_{\mathrm{new}}\boldsymbol{\beta}\\
\hline
\beta_0\boldsymbol{1}_n + \boldsymbol{X}_{\mathrm{old}}\boldsymbol{\beta}
\end{array}
\right]\spc;\spc
\sigma^2_Z
\left[
\begin{array}{c|c}
\boldsymbol{R}_{\mathrm{new}} + \lambda\boldsymbol{I}_m &\boldsymbol{R}_{\mathrm{new},\mathrm{old}}\\
\hline
\boldsymbol{R}_{\mathrm{new},\mathrm{old}}^{\mathsf{T}} &\boldsymbol{R}_{\mathrm{old}} + \lambda\boldsymbol{I}_n
\end{array}
\right]
\right\}\spc,
\end{align*}

\noindent where
$\boldsymbol{R}_{\mathrm{new},\mathrm{old}}$ is the cross-correlation matrix $\boldsymbol{R}_{\mathrm{new},\mathrm{old}}^{i,j} = R\left(\boldsymbol{x}_{\mathrm{new}}^i,\boldsymbol{x}_{\mathrm{old}}^j\right)$.\\

\noindent It is therefore straightforward to show that
\begin{align}\label{eq:pred_conditional}
\mathbb{E}\left\{\boldsymbol{y}_{\mathrm{new}}\Big|
\boldsymbol{y}_{\mathrm{old}},\boldsymbol{\Theta}\right\}=
\beta_0\boldsymbol{1}_m+\boldsymbol{X}_{\mathrm{new}}\boldsymbol{\beta}+\boldsymbol{R}_{\mathrm{new},\mathrm{old}}\left[\boldsymbol{R}_{\mathrm{old}} + \lambda\boldsymbol{I}_n\right]^{-1}\left(\boldsymbol{y}_{\mathrm{old}}-\beta_0\boldsymbol{1}_n - \boldsymbol{X}_{\mathrm{old}}\boldsymbol{\beta}\right)\spc,
\end{align}
and predictions, based on a sample $\left\{\boldsymbol{\Theta}_i\right\}_{i=1}^N$ from the posterior distribution (as described in section \ref{sec:MCMC}), can be made by integrating $\boldsymbol{\Theta}$ out, namely
\begin{align}\label{eq:pred_averaged}
\widehat{\boldsymbol{y}}_{\mathrm{new}} =\mathbb{E}\left\{\boldsymbol{y}_{\mathrm{new}}\Big|
\boldsymbol{y}_{\mathrm{old}}\right\} &= \int\mathbb{E}\left\{\boldsymbol{y}_{\mathrm{new}}\Big|
\boldsymbol{y}_{\mathrm{old}},\boldsymbol{\Theta}\right\}p\left(\boldsymbol{\Theta}\big|\boldsymbol{y}_{\mathrm{old}}\right)\di\boldsymbol{\Theta}\nonumber\\[1em]
&\approx \frac{1}{N}\sum_{i=1}^N\mathbb{E}\left\{\boldsymbol{y}_{\mathrm{new}}\Big|\boldsymbol{y}_{\mathrm{old}},\boldsymbol{\Theta}_i\right\}\spc.
\end{align}
This is, in fact, the usual model averaging estimator (see e.g. \citealt[Chapter~9]{Ghosh}).

\noindent If the set $\boldsymbol{X}_{\mathrm{new}}$ is known in advance, (\ref{eq:pred_conditional}) can be calculated on the fly (within each Metropolis iteration), and significant calculation time can be saved, depending on the acceptance rate of our sampling - provided that no new predictions are made whenever a new vector is rejected.

\noindent It is also worthwhile to consider ``denoising'' through elimination of highly unlikely models from (\ref{eq:pred_averaged}), by setting exceptionally small posterior probabilities (according to a predetermined threshold) to zero.

\subsection{Prediction based on Variable Selection}
\noindent Another obvious option is to regard the Bayesian mechanism of Section \ref{sec:Bayesian} as a mere selection procedure to identify influential (either linear or nonlinear) variables. In that case, inert variables in either the regression or the correlation part, will be set to $0$ or $1$, respectively, and the prediction at location $\bx$ will be
\begin{align}\label{eq:krig_nugget}
\widehat{y}\ofx = \bx^{\mathsf{T}}\widehat{\boldsymbol{\beta}} + \boldsymbol{r}_{\widehat{\boldsymbol{\rho}}}^{\mathsf{T}}\ofx\left[\boldsymbol{R}_{\widehat{\boldsymbol{\rho}}}+\widehat{\lambda}\boldsymbol{I}\right]^{-1}\left(\by-\boldsymbol{X}\widehat{\boldsymbol{\beta}}\right)\spc,
\end{align}
where $\left(\widehat{\boldsymbol{\beta}},\widehat{\boldsymbol{\rho}},\widehat{\lambda}\right)$ are the maximum likelihood estimators of $\left(\boldsymbol{\beta},\boldsymbol{\rho},\lambda\right)$, obtained by solving iteratively
\begin{align*}
\begin{cases}
\widehat{\boldsymbol{\beta}}\left(\widehat{\boldsymbol{\rho}},\widehat{\lambda}\right) = \left(\boldsymbol{X}^{\mathsf{T}}\left[\boldsymbol{R}_{\widehat{\boldsymbol{\rho}}}+\widehat{\lambda}\boldsymbol{I}\right]^{-1}\boldsymbol{X}\right)^{-1}\left[\boldsymbol{R}_{\widehat{\boldsymbol{\rho}}}+\widehat{\lambda}\boldsymbol{I}\right]^{-1}\by \spc,\\[1em]
\widehat{\sigma}^2\left(\widehat{\boldsymbol{\beta}}, \widehat{\boldsymbol{\rho}},\widehat{\lambda}\right)=n^{-1}\left(\by-\boldsymbol{X}\widehat{\boldsymbol{\beta}}\right)^{\mathsf{T}}\left[\boldsymbol{R}_{\widehat{\boldsymbol{\rho}}}+\widehat{\lambda}\boldsymbol{I}\right]^{-1}\left(\by-\boldsymbol{X}\widehat{\boldsymbol{\beta}}\right)\spc,\\[1em]
\left(\widehat{\boldsymbol{\rho}},\widehat{\lambda}\right)=\displaystyle\argmin_{\boldsymbol{\rho},\lambda}\left\{n\log\widehat{\sigma}^2\left(\widehat{\boldsymbol{\beta}}\left(\boldsymbol{\rho},\lambda\right), \boldsymbol{\rho},\lambda\right) + \log\left|\boldsymbol{R}_{\boldsymbol{\rho}}+\lambda\boldsymbol{I}\right|\right\}\spc.
\end{cases}
\end{align*}
Details of the optimization routine are given in \cite{DiceKriging}.\\

\noindent Denoting $\mathcal{M} = \left(\bgamma^r,\bgamma^c\right)$, our model of choice could then be the highest posterior probability model, i.e. $$\mathcal{M}^* = \displaystyle\argmax_{\mathcal{M}}p\left(\mathcal{M}\big|\by\right)$$ (to which we will refer in ther text as the \textit{maximum a posetriori model}, or simply - the \textit{MAP model}), or, alternatively, we may set a threshold $q$ on the \textit{posterior inclusion probability}
\begin{align*}
p_i = \sum_{\ell:\gamma_i=1}p\left(\mathcal{M}_{\ell}\big|\by\right)\spc,
\end{align*}
(where $\gamma_i$ may be either $\gamma_i^r$ or $\gamma_i^c$), and select the variable $x_i$ to either part, only if $p_i\geq q$. The choice of $q=\frac{1}{2}$ leads to what is famously known as the `median model', which - in the simpler case of linear regression with uncorrelated noise - has been shown by \cite{barbieri} to be the best predictive model, under very strict conditions on both the prior distributions and the covariates where predictions are to be made. In Section \ref{sec:bayes_var_simulation} we set the threshold on the posterior inclusion probability at a relatively high value of $0.8$.  A more educated choice of that value is proposed in Subsection \ref{subsec:Qian}, based on $v$-fold cross-validation.

\section{A Simulation Study}\label{sec:bayes_var_simulation}
We now wish to test the proposed methods on simulated data. For that purpose, we used a $35$-run Maximin Latin Hypercube design (see \citealt{jones+johnson}) in $[-0.75,0.75]^5$ to sample contaminated data from the allegedly $5$ dimensional function
\begin{align}\label{eq:bayes_var_select_sim}
y\ofx = 3X_2 + 4X_3 + 5X_4 + 5\cos\dfrac{3\pi X_1}{2} + 4\cos\dfrac{2\pi X_2}{2} + 3\cos\dfrac{\pi X_3}{2} + \varepsilon\ofx\spc,
\end{align}
where $\varepsilon\ofx\stackrel{\text{i.i.d.}}{\sim}\mathcal{N}\left(0,0.1\right)$ . Note that while (\ref{eq:bayes_var_select_sim}) consists of both linear and non-linear parts, the variables $X_1$ and $X_4$ are absent from the linear and non-linear parts, respectively, and $X_5$ is inert. \\

\noindent We assigned prior distributions as follows:
\begin{align*}
&\beta_j\big|\gamma_j^r=1\sim\mathcal{N}\left(0,5^2\right)\spc,\spc j=1,\ldots,5\spc;\spc \omega_r,\omega_c\sim\mathcal{U}(0,1)\spc;\\[0.5em]
&\beta_0\sim\mathcal{N}\left(0,10^2\right)\spc;\spc\sigma^2_{_Z}\sim\text{Inv-}\Gamma(3,2)\spc\text{and}\spc\lambda\sim\text{Inv-}\Gamma(3,0.2)\spc,
\end{align*}
and calculated the root mean square prediction error (RMSPE) on an independent $100$-run maximin LHD in the same region.
A size $250,000$ sample was drawn from the posterior distribution, as described in Section \ref{sec:MCMC}, after the first $5000$ were discarded as burn-in.

\begin{figure}[ht]
\centering
\subfloat{\label{Beta_Simulation}\includegraphics[width=.5\textwidth]{Simulation_Beta_Posteriors_Box-Plots.png}}
  \subfloat{\label{Rho_Simulation}\includegraphics[width=.5\textwidth]{Simulation_Rho_Posteriors_Box-Plots.png}}
    \caption{Box plots of the posterior distributions of the regression and correlation parameters, for the simulated data.}
  \label{Posterior_Boxplots_Simulation}
\end{figure}

\noindent Figure \ref{Posterior_Boxplots_Simulation} shows the posterior distributions of both the regression coefficients and the correlation parameters, while Figure \ref{Simulation_Inclusion_Probs} shows their respective marginal posterior inclusion probabilities. For now, we set the inclusion limit at $0.8$, leaving us with a single regression term ($X_4$) in the trend part of the model, and three covariates in the nonlinear component ($X_1$, $X_2$ and $X_3$). This is also consistent with Figure \ref{Posterior_Boxplots_Simulation}. Apparently, the Gaussian process term effectively reflects the linear effects of $X_2$ and $X_3$ as well as their nonlinear effects, which explains why they were dropped from the regression component. As expected, Figure \ref{Posterior_Boxplots_Simulation} clearly identifies $X_1$ as inactive in the trend part and $X_4$ in the non-linear component, while $X_5$ is deemed inert.\\




\begin{figure}
  \centering
 \includegraphics[width=1\textwidth]{Simulation_Posterior_Inclusion.pdf}
  \caption{The posterior inclusion probabilities for the simulated data. The dashed line marks a $80\%$ posterior inclusion frequency.}
  \label{Simulation_Inclusion_Probs}
\end{figure}

\begin{figure}
  \centering
 \includegraphics[width=.55\textwidth]{Simulation_True_vs_Fitted.pdf}
  \caption{Predictions vs. true values for the simulated example.}
  \label{Simulation_True_vs_Fitted}
\end{figure}

\noindent Table \ref{tab:Sim_Comp_Bayes_Var_Select} contains a comparison of the empirical RMSPE of several fitted models when tested on the $100$-run validation set.  The models include ordinary kriging (OK, no linear trend at all), universal kriging (UK, a linear trend which includes all of the covariates), model averaging based on (\ref{eq:pred_averaged}), variable selection based on the posterior inclusion probability ($0.8$ at least) and the empirical highest posterior probability (MAP) model.

\begin{table}[ht!]
\caption{Comparison of several prediction methodologies for the simulated data.}
\centering
{\footnotesize
\begin{tabular}{|c|c|}
\hline
{\bf\small Method} &{\bf\small RMSPE}\\
\hline
OK &$0.168$\\
\hline
UK &$0.130$\\
\hline
Averaging &$0.247$\\
\hline
Postrior Inclusion &$0.115$\\
\hline
MAP &$0.124$\\
\hline
\end{tabular}
}
\label{tab:Sim_Comp_Bayes_Var_Select}
\end{table}

\noindent Interestingly, the MAP model in this example was the one containing $\bx_2$, $\bx_3$ and $\bx_4$ in its linear part, along with $\bx_1$, $\bx_2$ and $\bx_3$ in its non-linear part, compatibile with the machanism generating the data. However, it was outperformed by the model selected according to the posterior inclusion probabilities. It is our recommendation to resist the temptation of blindly opting for the empirical MAP model when it is unclear whether or not it is the true highest posterior model - in particular when the posterior distribution is multimodal or flat near its mode. In this example, not for the only time in this chapter, model averaging proved to be a poor strategy. One possible reason could be poor estimation of the posterior distribution, resulting in excessive weight being assigned to low priority models. Figure \ref{Simulation_True_vs_Fitted} is a demonstration of the performance of the model selected by the posterior inclusion probabilities on the hold-out set.



\section{Applications}

\subsection{Heat Exchanger Emulator}\label{subsec:Qian}
\noindent We now wish to test our method on the computer simulation described
in \cite{Qian}. Here, the total rate of steady state heat transfer of a heat
exchanger for electronic cooling applications is modelled as a function
of four input factors: the mass flow rate of entry air, the temperature of entry air, the solid material thermal
conductivity and the temperature of the heat source. The response is produced by a finite difference
code and was evaluated at a $64$-run experimental design, constituting an orthogonal array-based LHD. An additional $14$-run test set was used to validate the resulting emulator. Input variables were standardized into the $[0,1]$ region before analysis to overcome the different scales. Using the prior distributions of Section \ref{sec:bayes_var_simulation}, a sample of size $155,000$ was drawn from the posterior distribution, with the first $5000$ serving as burn-in.\\



\noindent Previously, only interpolators have been attempted, as the simulation itself is deterministic. \cite{Qian} reported a RMSPE of $2.59$ using a universal Kriging model with a linear trend, compared to $5.15$ achieved by ordinary Kriging, while
\cite{CGP} reduced the RMSPE to $2.24$. Lately, \cite{CombinedGP} managed an RMSPE of $1.93$, using a convex combination of two independent Gaussian processes to model the spatial structure. Here we allowed for a non-zero nugget effect.  The different methods are compared  in Table \ref{tab:Qian_Comp_Bayes_Var_Select}.
One interesting feature is that $\bx_4$ has a strong linear effect but is slightly less dominant in the covariance.  The other factors are modeled primarily via the covariance. This slightly deviates from the work of \cite{Qian}, who used linear terms for $\bx_2$ and $\bx_4$, and modelled the correlation using all four factors.\\

The dashed, horizontal line in Figure \ref{Qian_Inclusion_Probs} marks the cutoff used in this example to omit terms from the model. The cutoff - $77\%$ - was obtained via the following procedure:  only terms with at least a $30\%$ marginal inclusion probability were considered, and terms with $90\%$ marginal inclusion probability or more were automatically included. That left $4$ competing models, of which the eventual model was chosen via $8$-fold cross-validation (fitting the model, based on $56$ observations and testing on the remaining $8$ each time). Figure \ref{fig:Boston_CV} shows the results, along with one-standard error marks, potentially serving to prioritize sparse models, in a similar manner to CART models (see \citealt[chapter~3]{cart}). Generally, using this procedure leaves us with at most $2p$ models to compare (and, in practice, typically far less), instead of $2^{2p}$ in an exhaustive search. As evident from Figure \ref{fig:Qian_CV}, in this example, a model consisting of $4$ predictors ($X_4$ in the linear part and $X_1$, $X_2$ and $X_3$ in the stochastic part), was selected.\\



\begin{figure}[ht]
\centering
\subfloat{\label{Beta_Qian}\includegraphics[width=.5\textwidth]{Qian_Beta_Posteriors_Box-Plots.png}}
  \subfloat{\label{Rho_Qian}\includegraphics[width=.5\textwidth]{Qian_Rho_Posteriors_Box-Plots.png}}
    \caption{Box plots of the posterior distributions of the regression and correlation parameters, for the heat exchanger data.}
  \label{Posterior_Boxplots_Qian}
\end{figure}


\begin{figure}[ht]
  \centering
 \includegraphics[width=1\textwidth]{Qian_Posterior_Inclusion.pdf}
  \caption{The posterior inclusion probabilities for the heat exchanger emulator. The dashed line marks a $80\%$ posterior inclusion frequency.}
  \label{Qian_Inclusion_Probs}
\end{figure}


\begin{figure}
  \centering
 \includegraphics[width=.75\textwidth]{Qian_CV.pdf}
  \caption{$8$-fold cross-validation results for the Heat Exchanger simulation data, including 1-SE marks.}
  \label{fig:Qian_CV}
\end{figure}

\begin{table}[ht!]
\caption{Comparison of several prediction methodologies for the heat exchanger example.}
\centering
{\footnotesize
\begin{tabular}{|c|c|}
\hline
{\bf\small Method} &{\bf\small RMSPE}\\
\hline
OK &$2.023$\\
\hline
UK &$2.670$\\
\hline
Averaging &$2.686$\\
\hline
Postrior Inclusion &$1.793$\\
\hline
MAP &$1.793$\\
\hline
\end{tabular}
}
\label{tab:Qian_Comp_Bayes_Var_Select}
\end{table}


\subsection{The Boston Housing Data}\label{subsec:boston}
\noindent In order to test our method on a larger-scale problem, we now analyze the Boston Housing data set, which also appeared in
\cite{Vannucci}, and - most famously - in \cite{Breiman}, where a full description of the $13$ predictors - related to the median value of owner-occupied homes in census tracts of the Boston metropolitan area - can be found.
The data set contains $506$ observations, of which we used $130$ as a training set and the other $376$ for validation. Again, we transformed the predictors so that they are all in the $[0,1]$ interval.
We produced a sample from the posterior distribution of size $250,000$ (with an additional burn-in sample of size $15,000$), and the same set of priors
as in Section \ref{sec:bayes_var_simulation}. The resulting marginal posterior distributions are shown in Figure \ref{fig:Posterior_Boxplots_Boston}, where it is evident that none of the covariates makes a pure, linear contribution to the median property value, and that the $6$th (average number of rooms per dwelling), $10$th (full-value property-tax rate per $\$10,000$), $11$th (pupil-teacher ratio by town) and $13$th (\% lower status of the population) covariates stand out
in the non-linear part of the model.

\begin{figure}[ht]
\centering
\subfloat{\label{Beta_Boston}\includegraphics[width=.5\textwidth]{Boston_Beta_Posteriors_Box-Plots.png}}
  \subfloat{\label{Rho_Boston}\includegraphics[width=.5\textwidth]{Boston_Rho_Posteriors_Box-Plots.png}}
    \caption{Box plots of the posterior distributions of the regression and correlation parameters, for the Boston Housing data.}
  \label{fig:Posterior_Boxplots_Boston}
\end{figure}

\begin{figure}
  \centering
 \includegraphics[width=1\textwidth]{Boston_Posterior_Inclusion.pdf}
  \caption{The posterior inclusion probabilities for the Boston Housing data set. The dashed line marks a $76\%$ posterior inclusion frequency.}
  \label{fig:Boston_Inclusion_Probs}
\end{figure}

\noindent Figure \ref{fig:Boston_Inclusion_Probs} shows the marginal posterior inclusion probabilities and is very much in line with Figure \ref{fig:Posterior_Boxplots_Boston}. As previously in \ref{subsec:Qian}, the cutoff - $66\%$ - was determined by a $10$-fold cross-validation procedure, shown in Figure \ref{fig:Boston_CV}. In this example, the most parsimonious model, consisting of just $4$ predictors, was singled out as the obvious choice.\\



\begin{figure}
  \centering
 \includegraphics[width=.75\textwidth]{Boston_CV.pdf}
  \caption{10-fold cross-validation results for the Boston Housing data, including 1-SE marks.}
  \label{fig:Boston_CV}
\end{figure}

\noindent It is interesting to note that while the ordinary kriging and universal kriging models achieved empirical RMSPEs of
$4.02$ and $4.01$, respectively, on the hold-out set, the selected model, based on $4$ predictors, achieved a RMSPE of $3.98$.
Although prediction is not always the main purpose of variable selection procedures of this sort, it is still encouraging
to find out that dimensionality reduction of this magnitude does not necessarily come at the expense of predictive accuracy.
For further reference, we used the Treed Gaussian Process (TGP) model, a nonstationary model, developed and implemented by \cite{TGP}, which combines partitioning of the predictor space with local, stationary GP models. In this example, the TGP model achieved a RMSPE of $4.16$.



\section{Discussion}
\noindent In this chapter, we explored variable selection in Bayesian semiparametric regression models.
Although the primary goal of these procedures is often of qualitative or explanatory nature, we keep one eye open
on the accuracy of our predictions. With that in mind, our variable selection procedure is driven by prediction
throughout, as evident from the cross-validation procedure described in Subsection \ref{subsec:boston}, and thus differs from the frequentist-like selection procedure of \cite{Bingham}, where identification of the active inputs was the sole purpose.\\



\begin{comment}
\noindent Ideally, we would like to take advantage of
the Bayesian framework to provide accurate predictions, using (\ref{eq:pred_averaged}). However, using model averaging to a good effect might require
an educated choice of prior distributions, along with possibly vast samples from the posterior disributions. One very interesting open question is whether a set of sparsity prior distributions exists, such that under some aggregation methods, the minimax convergence rate of the mean squared prediction error can be achieved, as in the exponential weighting scheme of \cite{Tsybakov} for linear regression models.\\
\end{comment}

\noindent Naturally, one may consider replacing model (\ref{eq:model}) with universal kriging models of the form
$y\ofx = \beta_0 + \boldsymbol{f}\ofx^{\mathsf{T}}\boldsymbol{\beta} + Z\ofx + \varepsilon\ofx$,
where $\boldsymbol{f}\ofx = \left[f_1\ofx,\ldots,f_p\ofx\right]^{\mathsf{T}}$ for some dictionary of regression functions. In that case, extra caution needs to be taken, as choice of regression functions already in the reproducing kernel Hilbert space associated with the covariance kernel $R\left(\cdot,\cdot\right)$ could cause a multicollinearity-like effect (see \citealt{Dizza}), resulting in the omission of crucial factors from our model.

\begin{comment}
\noindent One question left unanswered in this chapter, and which may be the basis for future reasearch, is whether of not one should some linear terms for
extrapolation purposes, even when the selection process indicates otherwise. Based on the artificial example of Section \ref{sec:bayes_var_simulation},
it looks very likely that the model will toss most of the regression functions, and rely on the covariance kernel. It would therefore be interesting to see how devastating an effect that would have on predictions outside the convex hull of the training data.
\end{comment}



==> Chapters/Isotonic.tex <==

\section{Introduction}

Isotonic modeling is a nonparametric approach for building models
whose fits are monotone in their covariates. Monotonicity
assumptions are natural to applications in biology \citep{obozinski2008consistent},
ranking \citep{Zhen2008}, medicine \citep{Sche1997}, statistics
\citep{Barl1972} and psychology \cite{Kruskal64}. Recently
\cite{luss2014generalized} developed the Generalized Isotonic
Recursive Partitioning (GIRP) algorithm that provides an effective
and efficient tool for solving large-scale isotonic modeling
problems with any differentiable convex loss function. There is,
however, a set of widely used loss functions which are not
differentiable and hold a special interest in statistical modeling
and machine learning problems. These loss functions pose additional
difficulties from both the theoretical and algorithmic side, as
shown through the next sections.\\

\noindent To formalize the isotonic modeling problem, first assume $n$ data observations
$(x_{1},y_{1})$,...,
$(x_{n},y_{n})$ and a partial order $\preceq$,
e.g., the standard Euclidean one where $x_{1}\preceq x_{2}$ if and
only if $x_{1j}\leq x_{2j\:}\forall j$ coordinate-wise. We index the
set of isotonicity constraints implied by the partial order by
$\mathcal{I}=\{(i,j):x_{i}\preceq x_{j}\}$. We define the isotonic
modeling problem as
\begin{equation}
\min{\{f(\hat{y}):\hat{y}_{i}\leq\hat{y}_{j}\quad\forall(i,j)\in\mathcal{I}\}}\label{eq:IR}
\end{equation}
in $\hat{y}\in\reals^{n}$, where $f:\reals^{n}\rightarrow\reals$
is a separable function such that
\begin{equation}
f(\hat{y})={\displaystyle \sum_{i=1}^{n}{f_{i}(\hat{y}_{i})}}\label{eq:seperable_loss_non_diff}
\end{equation}
and $f_{i}:\reals\rightarrow\reals$ is convex for all
$i=1,\ldots,n$. Typically, $f_{i}(\hat{y}_{i})=g(\hat{y}_{i},y_{i})$
measures the fit of $\hat{y_{i}}$ to the observed response.
Throughout the chapter we denote by $m=|\mathcal{I}|$ the number of
isotonic constraints and $d$ the dimension of data, i.e.,
$x_{i}\in\reals^{d}$.\\

\noindent While the assumption of isotonicity is often natural, isotonic
modeling has not been extensively applied in ``modern''
applications. This is because, as the number of observations $n$,
the data dimensionality $d$, and the number of isotonicity
constraints $m$ increase, problem (\ref{eq:IR}) suffers from
computational as well statistical (i.e., over-fitting) difficulties.
These are reviewed in \citep{luss2012efficient}, where it is argued that the
computational difficulties can be overcome using modern algorithms,
while over-fitting can be addressed by regularizing the problem. In
\citep{luss2012efficient} and \citep{luss2014generalized} this was done by early stopping,
i.e., fitting "less complex'' isotonic models than the optimal
solution of (\ref{eq:IR}). A different, more principled approach
would be to change the objective in (\ref{eq:IR}) by adding
regularization to it, in which case the function
$f_{i}(\hat{y}_{i})$ can combine a goodness of fit component with a
regularization or complexity control component.\\

\noindent The GIRP algorithm proposed in \citep{luss2014generalized} can easily
solve differentiable problems with tens of thousands of
observations, and is based on recursive partitioning of the
covariate space and construction of isotonic models of increasing
complexity, terminating in the global solution of (\ref{eq:IR}). In
this chapter we present a method for solving the isotonic modeling
problem with non-differentiable loss functions. Several widely used
non-differentiable loss functions which we focus on through the following sections are
provided in Table \ref{table:loss_functions}.


\begin{table}[h]
\begin{centering}

\begin{tabular}{|l|l|}
\hline
&\\[-2ex]
$\varepsilon$-insensitive loss & $f_{i}(\hat{y}_{i})=\left\{
\begin{array}{c}
\begin{array}{cc}
\hat{y}_{i}-y_{i}-\varepsilon & \hat{y}_{i}-y_{i}>\varepsilon\\
0 & |\hat{y}_{i}-y_{i}|<\varepsilon\\
-\hat{y}_{i}+y_{i}-\varepsilon & \hat{y}_{i}-y_{i}<-\varepsilon
\end{array}\end{array}\right\} $ \\[5ex]
\hline
&\\[-2ex]
Hinge loss  & $f_{i}(\hat{y}_{i})=\max\{0,1-\hat{y}_{i}\cdot y_{i}\}$ \\[2ex]
\hline
&\\[-2ex]
Quantile loss  & $f_{i}(\hat{y}_{i})=\left\{ \begin{array}{c}
\begin{array}{cc}
\tau(\hat{y}_{i}-y_{i}) & \hat{y}_{i}-y_{i}>0\\
-(1-\tau)(\hat{y}_{i}-y_{i}) & \hat{y}_{i}-y_{i}<0
\end{array}\end{array}\right\} $ \\[3ex]
\hline
&\\[-2ex]
$l_{2}$ loss with lasso regularization  & $f_{i}(\hat{y}_{i})=\left(\hat{y}_{i}-y_{i}\right)^{2}+\frac{\lambda}{n}|\hat{y}_{i}|$ \\[2ex]
\hline
&\\[-2ex]
$\begin{array}{c}
\text{Bernoulli log-likelihood } \\
\text{with lasso regularization}
\end{array} $
 & $f_{i}(\hat{p}_{i})=y_{i}log(\frac{1}{\hat{p}_{i}})+(1-y_{i})log(\frac{1}{1-\hat{p}_{i}})+\frac{\lambda}{n}|\hat{p}_{i}-\frac{1}{2}|$\\[2ex]
\hline
\end{tabular}
\par\end{centering}


\caption{Examples of non-differentiable loss functions solvable by our suggested
algorithm}


\label{table:loss_functions}
\end{table}

\noindent Throughout the years, a great deal of attention was given to
isotonic modeling with differentiable loss functions
(for example \citep{Barl1972}, \citep{luss2014generalized} and \citep{Maxw1985}). The non-differentiable case, on the
other hand, suffers from limited attention and is mainly focused on
the hinge loss popularized in support vector machines. For this
setup, the isotonic separation \citep{chandrasekaran2005isotonic}
provides an isotonic classification of the observations which is
done by solving a single linear program. Here we show that the
isotonic separation solution can also be achieved as a special case
of our algorithm and can be treated as a corollary. 
It is important to mention \cite{Hoch2003}, who offer a very efficient and related
algorithm for problem (\ref{eq:IR}), for both differentiable and
non-differentiable loss functions. Their algorithm is discrete in nature,
and can be used for determining an $\epsilon$-accurate
solution by solving the integer problem on an $\epsilon$-grid.
Their algorithm offers better complexity for solving problem (\ref{eq:IR}) than
our algorithm below to any desired accuracy, however our approach offers a direct formulation of the continuous non-differentiable
case in terms of sub-differnetial calculus. More importantly, our
approach offers natural statistical interpretation of the iterations of the
algorithm as a ``regularization path'' of greedy partial solutions, as
discussed in \citep{luss2014generalized} and \citep{luss2012efficient} for differentiable problems.\\

\noindent The main challenge in generalizing from the differentiable case to
handling non-differentiable loss functions is dealing with the
sub-differential algebra and its algorithmic implications, which
slightly differ between various non-differentiable functions. We
present our general algorithm and its adaptation to the loss
functions in Table~\ref{table:loss_functions} in Section
\ref{section2}, focusing on the lasso-penalized loss functions. Section \ref{s:properties} discusses the properties of our approach.
Section \ref{s:experiments} then demonstrates our suggested algorithm on
synthetic and real data sets. We first define terminology to be used
throughout the remainder of the chapter in Section \ref{def}, and then review the previously developed solution for the differentiable case in Section \ref{ss:diff_loss_functions}.\\

\section{Notation}
\label{def}
Let $V=\{x_{1},\ldots,x_{n}\}$ be the covariate vectors for $n$
training points where $x_{i}\in\mathbb{R}^{d}$ and denote $y_{i}\in\mathbb{R}$
as the $i^{th}$ observed response. 
We say $A\subseteq V$ is a group if for any $x,y,z \in V$, $x\preceq y\preceq z$ and $x,z \in A$ implies that $y \in A$. Throughout the
chapter, we will use the shorthand $i\in A=\{i:x_{i}\in A\}$. Denote
by $|A|$ the cardinality of group $A$. The \emph{fit} of a group
$A$ is denoted by
\begin{equation}
w_{A}=\argmin_{z\in\reals}{\displaystyle \sum_{i\in A}{f_{i}(z)}}.\label{eq:weight}
\end{equation}
For two groups $A$ and $B$, we denote $A\preceq B$ if $\exists x\in A,y\in B$
such that $x\preceq y$ and $\nexists x\in A,y\in B$ such that $y\prec x$
(i.e., there is at least one comparable pair of points that satisfy
the direction of isotonicity and no comparable pair which violates it). A set of groups $\mathcal{V}$ is called
isotonic if $A\preceq B\Rightarrow w_{A}\leq w_{B},\forall A,B\in\mathcal{V}$.
A subset $\mathcal{L}(\mathcal{U})$ of $A$ is a \emph{lower
set} (\emph{upper set}) of $A$ if $x\in A,y\in\mathcal{L},x\prec y\Rightarrow x\in\mathcal{L}
(x\in\mathcal{U},y\in A,x\prec y\Rightarrow y\in\mathcal{U})$. A
group $B\subseteq A$ is defined as a block of group $A$ if $w_{\mathcal{U}\cap B}\leq w_{B}$
for each upper set $\mathcal{U}$ of $A$ such that $\mathcal{U}\cap B\ne\{\}$
(or equivalently if $w_{\mathcal{L}\cap B}\geq w_{B}$ for each lower
set $\mathcal{L}$ of $A$ such that $\mathcal{L}\cap B\ne\{\}$).
We denote the optimal solution for minimizing $f(y)$ in the variable
$y$ by $y^{*}$, i.e., $y^{*}=\argmin{f(y)}$. The notation $(\partial f(\hat{y})/\partial\hat{y})|_{y}$
denotes the derivative of a function $f$ with respect to the variable
$\hat{y}$ evaluated at the point $y$ while $\partial f(\hat{y})|_{y}$
denotes its sub-differential.

\section{Previous Work}

\label{ss:diff_loss_functions} The optimal solution to the
generalized isotonic regression problem (\ref{eq:IR}) for
differentiable loss functions is known to be defined by a
partitioning of the observations $y_{i}$ into blocks in which
$\hat{y}_{i}=\hat{y}_{j}$ if observations $i$ and $j$ are in
the same block. Indeed, this structure can be seen through the
optimality conditions (i.e., Karush-Kuhn-Tucker (KKT) conditions)
for the differentiable form of problem (\ref{eq:IR}). The optimal
solution to (\ref{eq:IR}) in the differentiable case is denoted by
$\hat{y}^{*}$ and satisfies these conditions, which are given by
\begin{enumerate} [(a)]
\setlength{\itemsep}{6pt}
\item $\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|_{\hat{y}_{i}^{*}}=\sum_{j:(j,i)\in\mathcal{I}}{\lambda_{ji}}-\sum_{j:(i,j)\in\mathcal{I}}{\lambda_{ij}}\quad\forall i\in V$
\item $\hat{y}_{i}^{*}\leq\hat{y}_{j}^{*}\quad\forall(i,j)\in\mathcal{I}$
\item $\lambda_{ij}^{*}\geq0\quad\forall(i,j)\in\mathcal{I}$
\item $\lambda_{ij}^{*}(\hat{y}_{i}^{*}-\hat{y}_{j}^{*})=0\quad\forall(i,j)\in\mathcal{I}$,
\end{enumerate}
where $\lambda_{ij}^{*}$ is the optimal dual variable associated
with isotonicity constraint $\hat{y_{i}}\leq\hat{y_{j}}$. The convexity
of the loss function implies that any solution satisfying conditions
(a)-(d) is a globally optimal solution. From condition (d), $\lambda_{ij}^{*}>0\Rightarrow\hat{y}_{i}^{*}=\hat{y}_{j}^{*}$,
i.e., the optimal solution is made of blocks $V$ where $\lambda_{ij}^{*}>0$
for all $i,j\in V$, which implies that all observations within a
block $V$ are fit to the same value. Furthermore, when restricting
all fits within a block $V$ to be equal, the isotonic regression
problem over block $V$ is the following unconstrained problem
\begin{equation}
\min_{\hat{y}\in\reals}{\{{\displaystyle \sum_{i\in V}{f_{i}(\hat{y})}\}}}\label{eq:irp_weight}
\end{equation}
which can be easily solved for most widely used loss functions.
We define the minimizer of the block $V$ as the fit of the block.
Condition (b) implies that these fits must satisfy isotonicity, i.e.,
if $V^{-}\preceq V^{+}$ are isotonic blocks then $w_{V^{-}}\leq w_{V^{+}}$.
Thus, the structure of the optimal solution is a partitioning of the
set $\{1,\ldots,n\}$ into some (unknown number) $K$ blocks $\{V_{1},\ldots,V_{K}\}$
where $\hat{y}_{i}^{*}=w_{V_{k}}$ for all $i\in V_{k}$ and $\hat{y}_{i}^{*}\leq\hat{y}_{j}^{*}$
for all $(i,j)\in\mathcal{I}$.\\

\noindent Many such feasible partitions exist that are not optimal (e.g., set
$\hat{y}_{i}$ to be the fit of a group which contains all $n$ observations).
Condition (a) above must also be satisfied and gives the motivation
for how to partition the set of observations in a manner that leads
to the optimal partitioning.

\subsubsection{Isotonic recursive partitioning algorithm with differentiable loss functions}

\label{ss:Isotonic Recursive Partitioning Algorithm with Differentiable Loss Functions}

The Generalized Isotonic Recursive Partitioning Algorithm \citep{luss2014generalized} starts with the entire dataset as one group $V$ and iteratively splits it into an increasing number of groups,
until the optimal solution of (\ref{eq:IR}) is reached. At each iteration,
the algorithm chooses a sub-optimal group and partitions it into two
groups by solving a specially structured linear program that is amenable to very efficient algorithms.
If the partition puts all observations into one group, it can be shown
that the group is a block, i.e., optimal. Otherwise, the fits in the
two resulting groups are recalculated as their fits (via (\ref{eq:irp_weight})
above), while the rest of the groups and their fits remain at their
values in the previous iteration. This partitioning algorithm is thus
an iterative scheme that splits a group at each iteration and never
merges two groups back together; therefore, it is referred to as a
no-regret partitioning algorithm.
Two important theorems are proven with respect to this partitioning
scheme. The first states that the new solution
obtained after each partitioning step still satisfies isotonicity while the second shows that the partitioning scheme terminates at the globally optimal partitioning.
These theorems are made possible because of the particular splitting
criterion used in the partitioning algorithm, which is amenable to
efficient calculation as mentioned above.



\section{Isotonic Modeling with Non-differentiable Loss Functions}
\label{section2} 
\label{ss:non_diff_loss_fnc}
In this section we present our suggested isotonic
modeling algorithm for non-differentiable loss functions.
As with the differentiable case, our suggested 
partitioning algorithm is motivated by the optimality
conditions for the isotonic modeling problem. The KKT conditions for
(\ref{eq:IR}) in the non-differentiable case are identical to
conditions (a)-(d) in Section \ref{ss:diff_loss_functions} above,
with the exception that condition (a) now has a sub-differential
form:
\begin{enumerate} [(a)]
\item $0\in\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=\hat{y}_{i}^{*}}-\sum_{j:(j,i)\in\mathcal{I}}{\lambda_{ji}^{*}}+\sum_{j:(i,j)\in\mathcal{I}}{\lambda_{ij}^{*}} \quad \forall i\in V$
\end{enumerate}
where again $\lambda_{ij}^{*}$ is the optimal dual variable associated
with isotonicity constraint $\hat{y_{i}}\leq\hat{y_{j}}$. Convexity
of the loss function again implies that any solution satisfying the
optimality conditions is a globally optimal solution. The structure
of the optimal solution as a partitioning of isotonic blocks can be
seen from the sub-differential KKT conditions as described in Section
\ref{ss:diff_loss_functions}. Within each block, the fit to each
observation for the general case is taken to be the fit of the observations
in the block as defined by (\ref{eq:irp_weight}). We notice that unlike the differentiable case, here the fit of the block may not be unique. 
The sub-differential form of the KKT conditions, along with the non-uniqueness of the block fits, entiles a theoretical and algorithmic revision that is discussed next. \\

%Isotonicity of the two blocks $V^{-}$ and $V^{+}$, i.e., $V^{-}\preceq V^{+}$, means that $w_{V^{-}}\leq w_{V^{+}}$. 
\noindent Sub-gradient calculus \citep{boyd2003subgradient}
shows us that for a set of $n$ convex function $f_{1,},...,f_{n}$ with
sub differential sets $\partial f_{1},...,\partial f_{n}$ we have
\begin{equation}
\partial\left(\sum_{i=1}^{n}\, f_{i}\right)=\sum_{i=1}^{n}\partial f_{i}
\end{equation}
where the summation of the sets $\partial\left(\sum_{i=1}^{n}\, f_{i}\right)$
implies the Minkowski sum. Therefore, using the convexity of the loss
function and the sub-differential KKT conditions we suggest that the
fit of the block V is any $w_{V}$ that satisfies
\begin{equation}
0\in\sum_{i\in V}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}.\label{eq:block_min_non_diff}
\end{equation}
In order to derive our partitioning step we first introduce two
propositions. 


% Consider a group
%$V$ where $\hat{y}_{i}^{*}=w_{V}$ for all $i\in V$ and denote a
%partitioning of $V$ into three isotonic groups as $V^{-}, V^{0}$
%and $V^{+}$ such that $V^{-}\preceq V^{0}\preceq V^{+}$. We claim
%that if there exists such a partitioning that satisfies
%\begin{equation}
 %    \begin{aligned}
%0\in&\sum_{i\in V^{0}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}},\\
%&\sum_{i\in V^{+}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}-\sum_{i\in V^{-}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\prec0
%\label{eq:opt_cond_non_diff}
%\end{aligned}
%\end{equation}

%then the partitioning to the three blocks $V^{-}, V^{0}, V^{+}$ with
%the corresponding fits $w_{V^{-}}, w_{V}, w_{V^{+}}$ achieves a
%lower global loss than $V$. Notice that the notation of the minus
%sign between two sets $A$ and $B$ denotes the Minkowski difference $A-B=\{a-b,\, a\in A,b\in
%B\}$ and the right hand side of (\ref{eq:opt_cond_non_diff})
%suggests that every element in the set is strictly smaller than 0.
%Through the steps of our proof we show that this claim also holds
%for partitioning where one of the three groups, $V^{-}, V^{0}$ or
%$V^{+}$, is empty. To prove this claim we introduce a couple of
%propositions. 

\label{Proposition_1}
\begin{proposition} Assume every partitioning of a group $V$ into two
isotonic groups $V^{-}$ and $V^{+}$ satisfies
\begin{equation}
     \begin{aligned}
0\in\sum_{i\in V^{-}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\,,\,0\in\sum_{i\in V^{+}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}},\label{eq:prop1_non_diff}
\end{aligned}
\end{equation}
then the group $V$ is a block (i.e. optimal and shall not be partitioned).
\end{proposition} \begin{proof} 
As we demonstrated in (\ref{eq:block_min_non_diff}), the
fit of the block $V^{-} (V^{+})$ is any $w_{V}$ which satisfies the right (left) hand side of (\ref{eq:prop1_non_diff}). This means $w_{V}$, the minimizer of $V$, is also a minimizer of $V^{-}$ and $V^{+}$ for any isotonic partitioning of $V$. Therefore, the partitioning of $V$ is redundant, thus $V$ is a block. \end{proof}
 

\begin{proposition} 
\label{Proposition_2}
Any partitioning
of $V$ into two groups $V^{-} \preceq V^{+}$ that satisfies
\begin{equation}
     \begin{aligned}
\sum_{i\in V^{+}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}-\sum_{i\in V^{-}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\succ0\label{eq:non_diff_violation}
\end{aligned}
\end{equation}
necessarily violates isotonicity. Notice the minus
sign refers to Minkowski difference $A-B=\{a-b,\, a\in A,b\in B\}$. \end{proposition} 
\begin{proof}
Denote $A=\sum_{i\in V^{+}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}$
and $B=\sum_{i\in V^{-}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}$. Assuming $A-B\succ0$ we have $max\{B\}<min\{A\}$ which means either $0\prec A$ or $0\succ B$. Therefore either $\sum_{i\in V^{-}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\prec0$ or $\sum_{i\in V^{+}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\succ0$.\\

\noindent According to sub-gradient optimization theory \citep{boyd2003subgradient} if a function $f(x)$
is convex with a corresponding sub-differential $\partial f(x)$ and
$x^{*}$ is its optimal point, then for any $g\in\partial f(x)$ and
for a small $t>0$ we have
\begin{equation}
\left|\left|x-tg-x^{*}\right|\right|_{2}<\left|\left|x-x^{*}\right|\right|_{2}.
\end{equation}
In other words, $-g$ is a decent direction for $\left|\left|x-x^{*}\right|\right|_{2}$
for any $f(x^{*})<f(x)$. Therefore, if we denote $w_{V^{+}}$ as
the optimal point of $\sum_{i\in V^{+}}f_{i}(\hat{y}_{i})$ we have
that $-g$ is a decent direction for $\left|\left|w_{V}-w_{V^{+}}\right|\right|_{2}$
for every $g\in\sum_{i\in V^{+}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}$.
However, since $\sum_{i\in V^{+}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\succ0$
we get that descent direction to $w_{V^{+}}$ is necessarily negative, i.e. $w_{V^{+}}<w_{V}$, 
which contradicts the isotonic nature of the partitioning. 
Same derivation
applies for $w_{V^{-}}$ and $\sum_{i\in V^{-}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\prec0$. This means that any partitioning that satisfies (\ref{eq:non_diff_violation})
necessarily violates the isotonic nature of the partitioning. 
\end{proof} 

\noindent Combining these propositions we conclude that if every partitioning
of $V$ into two groups $V^{-} \preceq V^{+}$ satisfies
\begin{equation}
     \begin{aligned}
\sum_{i\in V^{+}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}-\sum_{i\in V^{-}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\succeq0,
\end{aligned}
\end{equation}
then no further partitioning can reduce the global cost (\ref{eq:IR}). Furthermore, as a result of Proposition \ref{Proposition_2} we see that if there exists a partitioning of $V$ into two groups $V^{-} \preceq V^{+}$ such that either $\sum_{i\in V^{-}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\succ0$ or $\sum_{i\in V^{+}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\prec0$ then we can further reduce the global cost.\\

\noindent Note that it is possible that $\sum_{i\in V^{-}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\succ0$ while $0 \in \sum_{i\in V^{+}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}$ (or conversely, $0 \in \sum_{i\in V^{-}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}$ and $\sum_{i\in V^{+}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\prec0$). In this case we may still improve our objective. This motivates our formulation of the partition problem in terms of three sets rather than two. In other words, in order to find the best partitioning we combine the two descent conditions and further allow a "zero element set" $V^{0}$ such that $0\in\sum_{i\in V^{0}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}$. This leads to the following optimization problem
\begin{align}
\label{eq:opt_prob_non_diff}
\min_{\substack{V^{-} \preceq V^{0} \preceq V^{+}\\ V^{-} \cup V^{0} \cup V^{+} = V}}\Bigg\{\max\Bigg\{& \sum_{i\in V^{+}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}} -\sum_{i\in V^{-}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\Bigg\},\; s.t.\; 0\in\sum_{i\in V^{0}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\Bigg\}
\end{align}

\noindent We notice that if this optimization problem achieves a non-negative
value then we cannot further decrease the global cost. Notice that since the sub-differential is a convex set the optimality of the maximization operator suggests that the constraint $0\in\sum_{i\in V^{0}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}$ is always met (hence redundant), otherwise it means we can decrease the minimum further
more.\\
%Introducing the auxiliary variables $u_{iu},u_{il}\in\{0,1\}$ such that
%$u_{i}=u_{iu}-u_{il}$ we have
%\begin{align}\label{eq:piecewise_derivation_2}
%\underset{i\in V}{\sum}z(u_{il},u_{iu}) &= \\[0.5em]
%&\sum_{\substack{i\in V\\w_{V}-y_{i}\neq\varepsilon_{1}\\w_{V}-y_{i}\neq\ -\varepsilon_{2}}}(u_{iu}-u_{il})\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}}+\nonumber \\[0.5em]
%&\sum_{\substack{i\in V\\w_{V}-y_{i}=-\varepsilon_{2}}}u_{il}\rho+
%\sum_{\substack{i\in V\\ w_{V}-y_{i}=\varepsilon_{1}}}u_{iu}\tau. \nonumber
%\end{align}
%Notice that since $\rho,\tau \geq 0$, we have that $u_i=0$ corresponds to $u_{iu}=u_{il}=0$ (as opposed to $u_{iu}=u_{il}=1$) from cost minimization reasons.


\noindent Let us denote the assignment of every observation $i \in V$ to each of the three sets $\left(V^{-}, V^{0}, V^{+}\right)$ by $u_{i}\in\left\{ -1,0,1\right\}$, respectively. Further, define  auxiliary variables $u_{iu},u_{il}\in\{0,1\}$ such that  $u_{i}=u_{iu}-u_{il}$.
It is later shown that the structure of our optimization problem (\ref{eq:opt_prob_non_diff}) leads to an integer linear problem of the form

\begin{equation}
\begin{aligned}
\min_{\substack{u_{il},u_{iu}\in\left\{0,1\right\}}}\Bigg\{& \sum_{i\in V}(z_{il}u_{il}+z_{iu}u_{iu}):\, u_{iu}\leq u_{ju}, u_{il} \geq  u_{jl}\,\,\forall(i,j)\in I \Bigg\} 
\label{opt_problem1}
\end{aligned}
\end{equation} where $z_{il}, z_{iu}$ are specifically defined for every type of loss function. To efficiently solve this optimization problem we would like to reformulate it as linear program without the integrality constraints.


\noindent It is well known \citep{Murt1983} that when a set of constraints
has a special structure known as totally unimodular, the linear
program relaxation to a binary problem (with
$u_{i}\in[-1,1]$) is solved on the boundary of the feasible region
with $u_{i}^{*}\in\{-1,1\}$ for all $i=1,\ldots{},n$. In
\citep{luss2012efficient} it was shown that the isotonic constraints for a
binary problem always comply with the conditions for unimodularity.
However, in our current problem formulation we have
a different set of constraints for the set of variables $u_{il},u_{iu}\in\left\{0,1\right\}$.
As mentioned above, we define $u_{i}=u_{iu}-u_{il}$, where $u_{i}$ are to satisfy isotonic constraints. Here we argue that the corresponding set of constraints for variables $u_{il},u_{iu}\in\left\{0,1\right\}$ also satisfies the totally unimodluar conditions.\\

\noindent Let us denote the matrix form of the isotonic constraints for $u_{i}\in\{-1,0,1\}$ as $A$ with a set of rows $A_x$.
Further, denote the equivalent isotonic constraints using the auxiliary variables $u_{il},u_{iu}\in\left\{0,1\right\}$ as $\tilde{A}$ with a set of rows $\tilde{A}_x$.
Notice that $\tilde{A}$ has twice as many rows as $A$, where  $A_x(k)=\tilde{A}(2k)$ and $-A_x(k)=\tilde{A}(2k+1)$.  
We claim this representation preserves
the totally unimodular constraints structure of the matrix $A$. We start with the following proposition.


\begin{proposition}
\label{Proposition_Murty}
 Assume $A$ is a totally unimodular matrix with a set of rows $A_x$ and $B$ is another matrix with a set of rows $B_x$. If every row in $A_x$ appears at least once in $B_x$ and every row in $B_x$ appears exactly once in $A_x$, then $B$ is also totally unimodular.
\end{proposition} \begin{proof}
A unimodular matrix is a square integer matrix having determinant $+1$ or $-1$.
A totally unimodular matrix is a matrix (not necessarily square or non-singular itself) that each of its square non-singular submatrices is unimodular.
Therefore, if $A$ is a totally unimodular matrix with a set of rows $A_x$ and  $B_x$ contains only the rows of $A_x$, each row at least once, then
for each square submatrix $\bar{B}$ of $B$ we have:
\begin{enumerate} [a.]
\item If a row in $A_x$ appears more than once in $\bar{B}_x$ then $\bar{B}_x$ is a singular matrix.
\item If every row in $A_x$ appears at most once in $\bar{B}_x$ then $\bar{B}_x$ is a unimodular matrix, as $A$ is a totally unimodular matrix.
\end{enumerate}
We conclude that every square non-singular submatrix of $B$ is unimodular, hence $B$ is totally unimodular
\end{proof}

\noindent Let us now define a matrix $B$ such that $A_x(k)=B_x(2k)=B_x(2k+1)$. Further, define a diagonal matrix $H$ such that $H(i,i)=(-1)^{i+1}$. Notice the auxiliary isotonic constraints matrix $\tilde{A}$ can be simply expressed  as $\tilde{A}=B\cdot H$. Since $B$ is totally unimodular (following Proposition \ref{Proposition_Murty}) and the determinant of $H$ is $+1$ or $-1$ we conclude that $\tilde{A}$ is totally unimodular and we are safe to apply Murty's relaxation and achieve the optimal
solution with a simple LP. This two-cuts partitioning step leads to a recursive algorithm which generalizes the GIRP \citep{luss2014generalized} in the sense that in each
iteration it partitions a group into three isotonic groups. More
specifically, at each iteration the algorithm chooses a group and partitions it into three isotonic groups $V^{-}\preceq
V^{0}\preceq V^{+}$ . If the partition puts all observations into
one group then we have that the group is a block, i.e., optimal.
Otherwise, the fits of  $V^{-}$ and $V^{+}$ are recalculated via
(\ref{eq:irp_weight}) while $V^{0}$ remains at its current fit
$w_{V}$. The rest of the groups and their fits remain at their
values in the previous iteration. It is important to notice that for
differentiable loss functions with observations in general locations
(probability of two observations with the same value is zero), the
use of $V^{0}$ is redundant as any partitioning that changes a group
necessarily yields a change in the group's fit. In the non
differentiable setup it is not always true. This yields this
necessary adjustment. A complete pseudo-code for an example non-differentiable loss function (lasso Bernoulli log-likelihood) is given in the subsection \ref{ss:Bernoulli}.\\

\noindent As with the GIRP,  two important theorems are proven in Section \ref{s:properties} with respect to this partitioning scheme, with
necessary adjustments to non-differentiable loss functions and the
2-cuts partitioning step. The first states that the partitioning
scheme terminates at the globally optimal partitioning with no
regret. The second theorem shows that the new solution obtained
after each partitioning step still satisfies isotonicity. This means that at each
iteration, the fits from the partitioning provide a potential isotonic prediction model. Hence, it produces a
path of increasingly complex
isotonic solutions (since each iteration adds a partition), terminating in the optimal solution of (\ref{eq:IR}).\\
\noindent We continue deriving our suggested sub-differential algorithm for
several specifically interesting loss functions, provided in
Table~\ref{table:loss_functions}. Notice that the major contribution
of our suggested algorithm is that it provides a general framework
for deriving an isotonic modeling solution for any desired convex
non-differentiable loss function and is not limited to the ones
in Table~\ref{table:loss_functions}.

\subsection{Algorithms for Some Widely Used Non-differentiable Loss Functions}
\label{ss:widely_used}

\subsubsection{Piecewise linear loss functions}

A large number of commonly used non-differentiable loss functions
are piecewise linear. Typical examples are the absolute loss,
$\varepsilon$-insensitive loss and quantile loss. For
simplicity of presentation, we give the explicit derivation of our
suggested algorithm for a 3-piece linear loss function
(\ref{eq:piecewise_linear_non_diff}) which generalizes the examples
given above. This derivation can be easily extended to any piecewise
linear loss function. The 3-piece linear loss function is defined as:
\begin{align}
\label{eq:piecewise_linear_non_diff}
f_{i}(\hat{y}_{i})&=&\left\{ 
\begin{array}{cc}
\tau\left(\hat{y}_{i}-y_{i}-\varepsilon_{1}\right) & \hat{y}_{i}-y_{i}>\varepsilon_{1}\\
0 & -\varepsilon_{2}<\hat{y}_{i}-y_{i}<\varepsilon_{1}\\
-\rho\left(\hat{y}_{i}-y_{i}+\varepsilon_{2}\right) & \hat{y}_{i}-y_{i}<-\varepsilon_{2}
\end{array}\right\}
\end{align}
for  $\varepsilon_{1},\varepsilon_{2},\rho,\tau>0$. Therefore, its sub-differential is:
\begin{equation}
\partial f_{i}(\hat{y}_{i})=\left\{ \begin{array}{cc}
\{\tau\} & \hat{y}_{i}-y_{i}>\varepsilon_{1}\\
{}[0,\tau] & \hat{y}_{i}-y_{i}=\varepsilon_{1}\\
\{0\} & -\varepsilon_{2}<\hat{y}_{i}-y_{i}<\varepsilon_{1}\\
{}[-\rho,0] & \hat{y}_{i}-y_{i}=-\varepsilon_{2}\\
\{-\rho\} & \hat{y}_{i}-y_{i}<-\varepsilon_{2}
\end{array}\right\} .
\end{equation}
%$\sum_{\substack{i=0 \\ i\neq 4}}^n
Applying this to the partitioning step (\ref{eq:opt_prob_non_diff})
we have
\begin{align}\label{eq:piecewise_derivation}
&\min_{C_{V}}\Bigg\{ \max\Bigg\{\underset{_{i\in V^{+}}}{\sum}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}-\underset{_{i\in V^{-}}}{\sum}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\Bigg\} \Bigg\} \nonumber \\[0.5em]
 & =\min_{C_{V}}\Bigg\{\max\Bigg\{\sum_{\substack{i\in V^{+}\\w_{V}-y_{i}\neq\varepsilon_{1}\\w_{V}-y_{i}\neq\ -\varepsilon_{2}}}\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}}+\sum_{\substack{i\in V^{+}\\w_{V}-y_{i}=\varepsilon_{1}}}\partial f_{i}(\hat{y}_{i})\big|{}_{\hat{y}_{i}=w_{V}}-\nonumber\\[0.5em]
&\sum_{\substack{i\in V^{-}\\w_{V}-y_{i}\neq\varepsilon_{1}\\w_{V}-y_{i}\neq\ -\varepsilon_{2}}}\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}}-\sum_{\substack{i\in V^{-}\\w_{V}-y_{i}=-\varepsilon_{2}}}\partial f_{i}(\hat{y}_{i})\big|{}_{\hat{y}_{i}=w_{V}}\Bigg\}\Bigg\}
\end{align}
where $C_{V}$ is the set of all isotonic preserving cuts and the minimization is over all $(V^{-},V^{0},V^{+})\in C_{V}$. Notice the equality follows from
\begin{align}
&\min\left\{ \sum_{w_{V}-y_{i}=\varepsilon_{1}}\partial f_{i}(\hat{y}_{i})\big|{}_{\hat{y}_{i}=w_{V}}\right\}=\max\left\{ \sum_{w_{V}-y_{i}=-\varepsilon_{2}}\partial f_{i}(\hat{y}_{i})\big|{}_{\hat{y}_{i}=w_{V}}\right\} =0.
\end{align}
\noindent The optimal cut problem can therefore be expressed as the following optimization problem
\begin{equation}
\begin{aligned}
\min_{\substack{u_{i}\in\left\{ -1,0,1\right\}}}\Bigg\{ \sum_{i\in V}z_{i}(u_{i})\,:\, u_{i}\leq u_{j}\,\,\, \forall(i,j)\in I \Bigg\}, \label{optimal_cut_pw_linear}
\end{aligned}
\end{equation}
where
\[
z(u_{i})=\left\{ \begin{array}{cc}
u_{i}\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}} & w_{V}-y_{i}\neq\varepsilon_{1},-\varepsilon_{2}\\
\tau & w_{V}-y_{i}=\varepsilon_{1},\, u_{i}=1\\
\rho & w_{V}-y_{i}=-\varepsilon_{2},\, u_{i}=-1\\
0 & \text{o.w.}
\end{array}\right\} .
\]
Let us now introducing the auxiliary variables $u_{iu},u_{il}\in\{0,1\}$ such that
$u_{i}=u_{iu}-u_{il}$. This allows us to rewrite the summation term of (\ref{optimal_cut_pw_linear}) as
\begin{align}\label{eq:piecewise_derivation_2}
\underset{i\in V}{\sum}z(u_{il},u_{iu}) =\sum_{\substack{i\in V\\w_{V}-y_{i}\neq\varepsilon_{1}\\w_{V}-y_{i}\neq\ -\varepsilon_{2}}}(u_{iu}-u_{il})\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}}+\sum_{\substack{i\in V\\w_{V}-y_{i}=-\varepsilon_{2}}}u_{il}\rho+
\sum_{\substack{i\in V\\ w_{V}-y_{i}=\varepsilon_{1}}}u_{iu}\tau. 
\end{align}
Notice that since $\rho,\tau \geq 0$, we have that $u_i=0$ corresponds to $u_{iu}=u_{il}=0$ (as opposed to $u_{iu}=u_{il}=1$) from cost minimization reasons. This formulation leads to the following integer linear
problem:
\begin{equation}
\begin{aligned}
\min_{\substack{u_{il},u_{iu}\in\left\{0,1\right\}}}\Bigg\{& \sum_{i\in V}(z_{il}u_{il}+z_{iu}u_{iu}):\, u_{iu}\leq u_{ju}, u_{il}\geq u_{jl}\,\,\forall(i,j)\in I \Bigg\} \label{eq:linear_prob_non_diff}
\end{aligned}
\end{equation}
where

\begin{align}
&z_{iu}=\left\{ \begin{array}{cc}
\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}} & w_{V}-y_{i}\neq\varepsilon_{1},-\varepsilon_{2}\\
\tau & w_{V}-y_{i}=\varepsilon_{1}
\end{array}\right\} \,,\,\nonumber
\end{align}

\begin{align}
&z_{il}=\left\{ \begin{array}{cc}
-\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}} & w_{V}-y_{i}\neq\varepsilon_{1},-\varepsilon_{2}\\
\rho & w_{V}-y_{i}=-\varepsilon_{2}
\end{array}\right\}\nonumber.
\end{align}


\noindent As discussed in the previous section, our generalization of the
result of \cite{Murt1983} shows that this problem can be solved by a
simple LP, as the constraints of this problem are totally unimodular.

\subsubsection{The hinge loss function}

The hinge loss function holds a special interest in maximum margin classification problems
in support vector machines (SVMs) and is therefore presented separately. It is defined as
\begin{equation}
f_{i}(\hat{y}_{i})=\left\{ \begin{array}{cc}
1-\hat{y}_{i}\cdot y_{i} & \,\,\,\hat{y}_{i}\cdot y_{i}<1\\
0 & o.w.
\end{array}\right\}
\end{equation}
and it is easy to show that if we limit ourselves to a
classification problem in which $y_{i}\in\{-1,1\}$, the optimal
values $\hat{y}_{i}$ can take on when minimizing (\ref{eq:IR}) are
simply $\hat{y}_{i}\in\{-1,1\}$. Deriving the sub-differential of
the hinge loss function we have
\begin{equation}
\partial f_{i}(\hat{y}_{i})=\left\{ \begin{array}{cc}
\{-y_{i}\} & \,\,\hat{y}_{i}\cdot y_{i}<1\\
{}[-y_{i},0] & \,\,\hat{y}_{i}\cdot y_{i}=1, y_{i}=1\\
{}[0,-y_{i}] & \,\,\hat{y}_{i}\cdot y_{i}=1, y_{i}=-1\\
\{0\} & \,\,\hat{y}_{i}\cdot y_{i}>1
\end{array}\right\},
\end{equation}
which leads, in the same manner as in (\ref{eq:piecewise_derivation}), to a partitioning step
\begin{align}
&\hspace{-1em}\min_{C_{V}}\Bigg\{\max\Bigg\{\sum_{\substack{i\in V^{+}\\w_{V}\cdot y_{i}\neq1}}\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}}+\sum_{\substack{i\in V^{+}\\w_{V}\cdot y_{i}=1}}\partial f_{i}(\hat{y}_{i})\big|{}_{\hat{y}_{i}=w_{V}}-\nonumber \\[0.5em]
&\sum_{\substack{i\in V^{-}\\w_{V}\cdot y_{i}\neq1}}\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}}-\sum_{\substack{i\in V^{-}\\w_{V}\cdot y_{i}=1}}\partial f_{i}(\hat{y}_{i})\big|\,\,{}_{\hat{y}_{i}=w_{V}}\Bigg\}\Bigg\}.\label{eq:hinge_loss}
\end{align}
As before, this optimal cut problem (\ref{eq:hinge_loss}) can be
expressed as an optimization problem (\ref{optimal_cut_pw_linear})
with
\begin{equation}
\hspace{-3em}z(u_{i})=\left\{\begin{array}{cc}
u_{i}\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}} & \substack{w_{V}\cdot y_{i}\neq1, \\ u_i \neq 0}\\
y_i & \substack{w_{V}\cdot y_{i}=1, y_{i}=1,\\ u_i=-1}\\
-y_{i} & \substack{w_{V}\cdot y_{i}=1, y_i=-1\\ u_{i}=1}
\\
0 & \text{o.w.}
\end{array}\right\}.
\end{equation}
Therefore, similarly to (\ref{eq:piecewise_derivation_2}), we use the auxiliary variables $u_{iu},u_{il}\in\{0,1\}$ to obtain 
\begin{align}
\underset{i\in V}{\sum}z(u_{il},u_{iu})& =\sum_{\substack{i\in V\\w_{V}\cdot y_{i}\neq1}}(u_{iu}-u_{il})\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}}+\\[0.5em] \nonumber
&\sum_{\substack{i\in V\\w_{V}\cdot y_{i}=1\\y_{i}=1}}u_{il}y_{i}+\sum_{\substack{i\in V\\w_{V}\cdot y_{i}=1\\y_{i}=-1}}u_{iu}(-y_{i}).
\end{align}
Notice that as in (\ref{eq:piecewise_derivation_2}), we have that $u_i=0$ corresponds to $u_{iu}=u_{il}=0$ from cost minimization reasons. This formulation leads to an integer linear problem
(\ref{eq:linear_prob_non_diff}) with
\begin{align}
z_{iu}=&\left\{ \begin{array}{cc}
\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}} & w_{V}\cdot y_{i}\neq1\\
-y_i & w_{V}\cdot y_{i}=1, y_i=-1\\0 & \text{o.w.}\end{array}\right\}
 \,,\,\,\nonumber
\end{align}

\begin{align}
z_{il}=&\left\{ \begin{array}{cc}
\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}} & w_{V}\cdot y_{i}\neq1\\
y_i & w_{V}\cdot y_{i}=1, y_i=1\\0 & \text{o.w.}\end{array}\right\}
 \,.\,\,\nonumber
\end{align}
As in the previous example, we can apply the same continuous relaxation discussed in
(\ref{opt_problem1}) to achieve a simple linear program. We also notice that since
$w_{V}\in\{-1,1\}$ the hinge loss problem is solved in a single partitioning
step. We prove this by contradiction. Assume an additional optimal
cut is applied, which partitions one of the groups into two separate
sub-groups. These sub groups too are fitted with either $-1$ or $1$. This
contradicts the optimality of the previous cut since we found a cut
which isotonically partitions all of the observations to $-1$ and $1$
and achieves a lower global cost. This result coincides with isotonic
separation literature \citep{chandrasekaran2005isotonic} which shows
that optimal isotonic classification is made by solving a single linear
program, corresponding to a single optimal split.

\subsubsection{Comparison to a linear program solution}

Piecewise linear loss functions are a simple example which
demonstrates our suggested algorithm. It is clear however, that one
can solve problem (\ref{eq:IR}) with piecewise linear loss by simply
reformulating it to a single linear program with (linear) isotonicity
constraints. Our suggested algorithm on the other hand, obtains the
solution by recursively applying an LP solver to problems of
decreasing size. A comprehensive discussion on the complexity of our
suggested algorithm is followed in the next 
section. It is important however to state that one major advantage of our scheme,
even for loss functions that can be directly solved by a single LP,
is regularization.\\

\noindent Our suggested algorithm obtains the solution to the problem
(\ref{eq:IR}) by recursively partitioning the covariate space into
progressively smaller regions and fitting the best constant in each
region, referred to here as the fits of the blocks, as in (\ref{eq:weight}). As such, we argue that it
is natural to think of the resulting sequence of models created from
early stopping as a regularization path of models of increasing
complexity, indexed by the number of iterations of the algorithm.
Other examples of using early stopping for regularization include
training neural networks with back propagation \citep{Caru2000} and
boosting \citep{rosset2004boosting}. Extensive experience of the
usefulness of regularization in high dimensional fitting
\citep{Wahb1990,Tibs1996}, and especially in nonparametric
models like isotonic regression, suggests that regularization,
embodied in this case by early stopping of the algorithm, can lead
to reduced over-fitting and hence improved predictive performance.

\subsubsection{$l_{2}$ regression with lasso regularization}

\label{ss:l_2 reg with lasso} While regularization by early stopping can help prevent over-fitting, it lacks a clear interpretation in terms of the problem being solved. Instead, the most common
approach to regularization is to impose an additional term to the
minimization objective, which is a penalty that prevents
the model from being too complex. One of the most important
regularization functions is the $l_{1}$ norm which is commonly
referred to as lasso. For the lasso problem with $l_{2}$
loss presented in Table \ref{table:loss_functions}, the minimizer of
a block $V$ is simply a soft-thresholding version of the least
square minimizer
\begin{equation}
w_{V}=\left\{ \begin{array}{cc}
\bar{y}_{V}-\lambda/2 & \,\,\bar{y}_{V}>\lambda/2\\
0 & \,\,|\bar{y}_{V}|<\lambda/2\\
\bar{y}_{V}+\lambda/2 & \,\,\,\,\bar{y}_{V}<-\lambda/2
\end{array}\right\}
\end{equation}
and the sub-differential of the lasso problem, evaluated at $\hat{y}_{i}=w_{V}$, is simply \renewcommand{\arraystretch}{1.5}
\begin{align}
\partial f_{i}(\hat{y}_{i})&\big|{}_{\hat{y}_{i}=w_{V}}=\left\{ \begin{array}{cc}
2\left(w_{V}-y_{i}\right)+\lambda/n & \,\,w_{V}>0\\
2\left(w_{V}-y_{i}\right)+[-\lambda,\lambda]/n & \,\,w_{V}=0\\
2\left(w_{V}-y_{i}\right)-\lambda/n & \,\,w_{V}<0
\end{array}\right\} .
\end{align}
We would now like to apply our partitioning step as in (\ref{eq:piecewise_derivation}).
Let us differintiate between the three cases of $w_V$. For $w_V>0$ and $w_V<0$ we notice that the loss function is differentiable which leads to a single cut partitioning step, just like in the GIRP \citep{luss2014generalized}. Threfore, the single cut partitioning step for the $w_V>0$ case is simply
 
\begin{align}
% & \min_{(V^{-},V^{0},V^{+})\in C_{V}}\Bigg\{ \max\Bigg\{ \sum_{i\in V^{+}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}-\nonumber\\
%&\hspace{11.5em}\sum_{i\in V^{-}}\partial f_{i}(\hat{y}_{i})|_{\hat{y}_{i}=w_{V}}\Bigg\} \Bigg\} =\nonumber \\[0.5em]
% & \min_{(V^{-},V^{0},V^{+})\in C_{V}}\Bigg\{\max\Bigg\{\sum_{\substack{i\in V^{+}\\\hat{y}_{i}\neq0}}\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}}+\nonumber \\[0.5em]
%&\hspace{1em}\sum_{\substack{i\in V^{+}\\\hat{y}_{i}=0}}\partial f_{i}(\hat{y}_{i})\big|{}_{\hat{y}_{i}=w_{V}}-\sum_{\substack{i\in V^{-}\\ \hat{y}_{i}\neq0}}\frac{\partial f_{i}(\hat{y}_{i})}{\partial\hat{y}_{i}}\big|{}_{\hat{y}_{i}=w_{V}}-\nonumber \\[0.5em]
%&\hspace{10.5em}\sum_{\substack{i\in V^{-}\\\hat{y}_{i}=0}}\partial f_{i}(\hat{y}_{i})\big|\,\,{}_{\hat{y}_{i}=w_{V}}\Bigg\}\Bigg\}=\nonumber \\[0.5em]
  \min_{V^{-},V^{+}}\Bigg\{ \sum_{i\in V^{+}}\Bigg(2\left(w_V-y_{i}\right)+\frac{\lambda}{n}\Bigg)-\sum_{i\in V^{-}}&\Bigg(2\left(w_V-y_{i}\right)+\frac{\lambda}{n}\Bigg)\Bigg\} .
\end{align}
The corresponding linear integer problem is
\begin{align}
\min_{\substack{u_{i}\in\left\{-1,1\right\}}}\Bigg\{ \sum_{i\in V}u_i\Bigg(2\left(w_V-y_{i}\right)+\frac{\lambda}{n}\Bigg):\, 
 u_i\leq u_j\,\forall(i,j)\in I \Bigg\}\nonumber
\end{align}
which may be formulated as a simple LP, as discussed in the previous section. Notice that the $w_V<0$ case may be immediately obtained by replacing $+\lambda/n$ with $-\lambda/n$.  
On the other hand, for $w_V=0$ we have a two-cut partitioning step which may be formulated as
\begin{align}
\label{l2_non_diff}
\min_{\substack{u_{il},u_{iu}\in\left\{0,1\right\}}}\Bigg\{ \sum_{i\in V}2(&u_{iu}-u_{il})(w_V-y_{i})+\sum_{i\in V}\frac{\lambda}{n}(u_{iu}+u_{il}):\, \\\nonumber
& u_{iu}-u_{il}\leq u_{ju}-u_{jl}\,\forall(i,j)\in I \Bigg\}.\nonumber
\end{align}
Notice that $u_i=0$ is exclusively covered by $u_{il}=u_{iu}=0$, just like in previous examples. This means that the constraints of (\ref{l2_non_diff}) may be replaced with $u_{iu}\leq u_{ju},\, u_{il}\geq u_{jl} \,\,\,\, \forall(i,j)\in I$, leading to a simple LP formulation, as discussed in (\ref{opt_problem1}).

\subsubsection{Bernoulli log-likelihood with lasso regularization}
\label{ss:Bernoulli} Bernoulli log-likelihood is another widely used loss function which is relevant for classification problems.
Here we assume our observations are binary and would like to fit a
probability $\hat{p}_{i}$ for each observation $y_{i}$. As
in the $l_{2}$ case, the lasso regularization term prevents the
model from over-fitting $\hat{p}_{i}$ and keeps it closer to a
constant fit (for example, representing the overall probability
$P(Y=1)$, if this is known). In this work we use $\frac{1}{2}$ as
the constant for illustrative purposes, which can be thought of as
representing a prior belief that both classes are equally likely. As
in previous sections we denote the minimizer of a block $V$ as
$w_{V}$. The sub-differential of the Bernoulli log-likelihood problem, evaluated at $\hat{y}_{i}=w_{V}$, is just
\begin{align}
\partial f_{i}(\hat{p}_{i})&\big|{}_{\hat{y}_{i}=w_{V}}=\left\{ \begin{array}{cc}
\frac{- y_{i}}{w_{V}}+\frac{1- y_{i}}{1-w_{V}}+\frac{\lambda}{n} & \,\,w_{V}>\frac{1}{2}\\
\frac{- y_{i}}{w_{V}}+\frac{1- y_{i}}{1-w_{V}} +[\frac{-\lambda}{n},\frac{\lambda}{n}] & \,\,w_{V}=\frac{1}{2}\\
\frac{- y_{i}}{w_{V}}+\frac{1- y_{i}}{1-w_{V}} -\frac{\lambda}{n} & \,\,w_{V}<\frac{1}{2}
\end{array}\right\} .
\end{align}
As in the  $l_{2}$ regression example, we separate our analysis into three different cases. For $w_V>0$ and $w_V<0$ we have a differentiable loss function for which a single cut partitioning step suffices, as demonstrated in \citep{luss2014generalized}. For example, for $w_V>0$ we have 
\begin{align}
 & \min_{V^{+},V^{-}}\Bigg\{ \sum_{i\in V^{+}}\left( \frac{- y_{i}}{w_{V}} +\frac{1- y_{i}}{1-w_{V}}+\frac{\lambda}{n}\right) -\sum_{i\in V^{-}}\left(\frac{- y_{i}}{w_{V}} +\frac{1- y_{i}}{1-w_{V}}+\frac{\lambda}{n}\right)\Bigg\},
\end{align}
which leads to a linear integer problem 
\begin{equation}
\label{logistic_diff}
\min_{\substack{u_{i}\in\left\{0,1\right\}}}\Bigg\{ \sum_{i\in V}u_{i}\Bigg(\frac{- y_{i}}{w_{V}} +\frac{1- y_{i}}{1-w_{V}}+\frac{\lambda}{n}\Bigg):\,  u_{i}\leq u_{j}\,\forall(i,j)\in I \Bigg\}.\nonumber
\end{equation}
This problem  may be solved as a simple LP, as previously discussed. For $w_V=0$ we need again the two-cut partitioning formulation, which may be expressed as  
\begin{align}
\label{logistic_non_diff}
\min_{\substack{u_{il},u_{iu}\in\left\{0,1\right\}}}\Bigg\{ &\sum_{i\in V}(u_{iu}-u_{il})\Bigg(\frac{- y_{i}}{w_{V}} +\frac{1- y_{i}}{1-w_{V}}\Bigg)+\sum_{i\in V}\frac{\lambda}{n}(u_{iu}+u_{il}):\, \\\nonumber
& u_{iu}-u_{il}\leq u_{ju}-u_{jl}\,\forall(i,j)\in I \Bigg\}.\nonumber
\end{align}
Notice that the $u_i=0$ case is still exclusively covered by $u_{il}=u_{iu}=0$, just like in previous examples.  This means that the constraints of (\ref{logistic_non_diff}) may also be replaced with $u_{iu}\leq u_{ju},\, u_{il}\geq u_{jl} \,\,\,\, \forall(i,j)\in I$, leading to a simple LP formulation, as demonstrated in (\ref{opt_problem1}).\\

\noindent To conclude this section we present in Algorithm \ref{alg:algorithm} an explicit a pseudo code for the Bernoulli log-likelihood with lasso regularization problem which also comes handy in our experiments section. The additional notation we introduce in the algorithm is the model $M_k$ we get after iteration $k$, which is obtained by fitting each group in $M_k$ to its weight. For a set of groups $\mathcal{V}=\{V_1,\ldots,V_k\}$, denote $w_\mathcal{V}=\{w_{V_1},\ldots,w_{V_k}\}$.  Then model $M_k=(\mathcal{V},w_\mathcal{V})$ contains the partitioning $\mathcal{V}$ as well as a fit to each of the observations, which is the weight, as defined by (\ref{eq:weight}), of the group it belongs to in the partition.

\begin{algorithm}
\caption{Isotonic Modeling for Bernoulli log-likelihood with Lasso Regularization}
\begin{algorithmic} [1]
\REQUIRE Observations $(x_1,y_1),\ldots,(x_n,y_n)$ and partial order
$\mathcal{I}$.
\REQUIRE $k=0,\mathcal{A}=\{\{x_1,\ldots,x_n\}\}$,$\mathcal{C}=\{(0,\{\},\{x_1,\ldots,x_n\},\{\})\}$,$\mathcal{B}=\{\}$, $M_0=(\mathcal{A},w_\mathcal{A})$.
\WHILE{$\mathcal{A}\ne\{\}$}
\STATE Let $(val,w^-,w^0,w^+)\in\mathcal{C}$ be the potential partition with largest $val$.
\STATE Update $\mathcal{A}=(\mathcal{A}\setminus (w^-\cup w^0\cup w^+))\cup\{w^-,w^0,w^+\}$, $\mathcal{C}=\mathcal{C}\setminus(val,w^-,w^0,w^+)$.
\STATE $M_k=(\mathcal{A},w_\mathcal{A})$.
\FORALL{$v\in\{w^-,w^0,w^+\}\setminus\{\}$}
%\STATE Set $c_i=-\frac{y_{i}}{\hat{p}_{i}}+\frac{1- y_{i}}{1-\hat{p}_{i}}$ $\forall i\in v$ where $w_v$ is the weight (\ref{eq:weight}) of the observations in $v$.
\STATE Depending on the value of $w_V$, solve the LP formulation of (\ref{logistic_diff}) or (\ref{logistic_non_diff}) with input $u$ and get $u^*=\argmin{\mbox{LP}}$.
\IF{$u_1^*=\ldots=u_n^*$ (group is optimally divided)}
\STATE Update $\mathcal{A}=\mathcal{A}\setminus v$ and $\mathcal{B}=\mathcal{B}\cup \{v\}$. \ELSE
\STATE Let $v^-=\{x_i:u^*_i=-1\}, v^+=\{x_i:u^*_i=+1\}, v^0=\{x_i:u^*_i=0\},$.
\STATE Update $\mathcal{C}=\mathcal{C}\cup\{(c^Tu^*,v^-,v^0,v^+)\}$
\STATE Update $\mathcal{B}=\mathcal{B}\cup\{v^0\}$
\ENDIF
\ENDFOR
\STATE $k=k+1$.
\ENDWHILE
\RETURN $\mathcal{B}$, a partitioning of observations corresponding to the optimal groups.
\end{algorithmic}
\label{alg:algorithm}
\end{algorithm}

\section{Properties of the Non-differentiable Partitioning Algorithm }

\label{s:properties} We start by presenting two theorems, proving
two important properties of our algorithm. Theorem
\ref{th:no_regret_cut} proves the convergence of the greedy
splitting algorithm to the global minimum solving problem
(\ref{eq:IR}) for non-differentiable loss functions. Its proof is
given in Appendix \ref{isotonic_proofs}.

\begin{theorem} \label{th:no_regret_cut} Assume group $V$ is the union
of blocks from the optimal solution to problem (\ref{eq:IR}). Then
the cuts made by solving (\ref{eq:opt_prob_non_diff}) at a particular
iteration do not cut through any block in the global optimal solution.
\end{theorem}

\noindent Since our suggested Algorithm starts with the union of all blocks
for the first partition, we can conclude from this theorem that our
method never cuts a block when generating partitions. From the derivation
of the partitioning problem, it is clear that if an isotonic partition
can be made, it will be made; that is, the algorithm will not stop
early. Convergence of algorithm to the global isotonic solution with
no regret then follows by repeatedly applying Theorem \ref{th:no_regret_cut}
until all blocks of the optimal solution are identified. The next
theorem states that our suggested algorithm provides isotonic solutions
at each iteration. This result implies that the path of solutions
generated by our algorithm can be regarded as a regularization path
for the isotonic regression problem (\ref{eq:IR}). 

\begin{theorem} \label{th:isotonic_solutions} Model $M_{k}$ generated
after iteration $k$ of our suggested Algorithm is in the class of
isotonic models \cal C. \end{theorem}

\noindent Proofs of both these theorems is given in Appendix \ref{isotonic_proofs}.

\subsection{Computational Complexity Analysis}
The complexity analysis depends on the number of
observations $n$ and isotonic constraints $m$, and the
resulting complexity of solving each linear program. Additionally,
computing the fit of a group $V$ via (\ref{eq:weight}) requires an effort that
is linear in the log of the required accuracy (for loss functions that cannot
be solved analytically), denoted by $L$.
Our linear program is dual to a linear maximum
flow network problem \citep{networkflows}, which is a well studied
problem. It can be solved in $O(mn\log n)$ \citep{Slea1983}
or $O(n^3)$ \cite{Gali1980} in the general case that we consider;
special cases such as $d = 2$ or where the observations
lie on a grid can be computed even faster \cite{Spou2003}. The
choice of algorithm depends on $m$ which is $O(n^2)$ in
the worst case. Given that our suggested algorithm
requires at most $n$ iterations, this leads to worst
case complexities of $O(mn^2 \log n + nL)$ or $O(n^4+nL)$. A recent
problem reduction by \cite{stout2012isotonic} can be used to obtain
an equivalent representation of the desired problem
with $d$-dimensional data and $O(n log^{d-1} n)$ constraints
and observations, which can be useful when $m$ is
large. The solution of \cite{Hoch2003}, based
on a discretization of the continuous problem and
a clever approach for solving all sub-optimization problems with little
overhead, offers a reduced overall worst-case complexity of $O(mn\log\frac{m}{n^2} + nL)$
for reaching the optimal solution to (\ref{eq:IR}), without generating partial solutions.
Finally, \cite{luss2012efficient} show that IRP performs
in similar complexity $O(Cn^3+nL)$ in practice, where $C$ is a function of the
fraction of observations on each of the cut at each
iteration. The same result applies here.  In practice, our implementation, available from the first author's website \footnote{https://sites.google.com/site/amichaipainsky/software} solves problems of thousands of observations in any dimension in up to 120 seconds. For
example, our simulations in the next section comprise solving a
Bernoulli log-likelihood lasso problem on 5,000 observations in
dimension 5 and repeating this exercise one hundred times. This
takes about 20 minutes on a standard office PC.

\subsection{Degrees of Freedom of Lasso Regularized Isotonic Modeling}

The concept of degrees of freedom is commonly used in statistics to measure the complexity
of a model (or more accurately, a modeling approach). This concept captures
the amount of fitting the model performs, as expressed by the optimism of
the training sample error estimates, compared to out-of-sample predictive performance.
Here we briefly review the main ideas of this general approach, and then apply them to lasso regularized isotonic modeling.\\

\noindent Following \cite{efron1986biased} and \cite{hastie2005elements}, assume
the values $x_1...x_n$  are fixed in advance (the fixed-x assumption),
and that the model gets one vector of observations $y=(y_1...y_n)$
for training, drawn according to $P(y|x)$ at the n data points. Denote by $y^{new}$
another independent vector drawn according to the same distribution. $y$ is
used for training a model $\hat{f}(x)$ and generating predictions $\hat{y_i}=\hat{f}(x_i)$ at the n
data points.
We define the in-sample mean squared error as
\begin{equation}
MRSS=\frac{1}{n}\|y-\hat{y}\|^2_2
\end{equation}
and compare it to the expected error the same model incurs on the new, independent
copy, denoted in \citep{hastie2005elements} as $ERR_{in}$,
 \begin{equation}
ERR_{in}=\frac{1}{n}\mathbb{E}_{y^{new}}\|y^{new}-\hat{y}\|^2_2
\end{equation}
The difference between the two is the optimism of the in-sample prediction.
As \cite{efron1986biased} and others have shown, the expected optimism in MRSS is
 \begin{equation}
\mathbb{E}_{y,y^{new}}(ERR_{in}-MRSS)=\frac{2}{n}\sum_{i}cov(y_i,\hat{y_i})\label{eq:ERR-MRSS}
\end{equation}
For linear regression with homoskedastic errors with variance $\sigma^2$, it is easy
to show that (\ref{eq:ERR-MRSS}) is equal to $\frac{2}{n}d\sigma^2$ where $d$ is the number of regressors,
henceforth, the degrees of freedom. %This naturally leads to defining the equivalent
%degrees of freedom of a modeling approach as
%\begin{align}
%df&=\frac{1}{\sigma^2}\sum_{i}cov(y_i,\hat{y_i})\nonumber\\[0.5em]
%&=\frac{n}{2\sigma^2}\mathbb{E}_{y,y^{new}}(ERR_{in}-MRSS)\label{estimate_df}
%\end{align}
In nonparametric models, one usually cannot calculate the actual
degrees of freedom of a modeling approach, but it is often easier to
generate unbiased estimates $\hat{df}$ of $df$ using Stein lemma
\citep{stein1981estimation}. In \citep{meyer2000degrees} the authors 
demonstrate the applicability of this theory in shape-restricted
nonparametric regression. Specifically, their Proposition 2, adapted
to our notation, implies that if we assume that $y_i$ have i.i.d
Gaussian noise with variance $\sigma^2$, then the unbiased estimator
$\hat{df}$ for degrees of freedom in isotonic regression is the
expected number of blocks $D$ in the solution $\hat{y}$ to the $l^2$
isotonic modeling problem. That is,
\begin{equation}
\mathbb{E}(D)=\frac{\sigma^2}{n}\sum_{i}cov(y_i,\hat{y_i})
\end{equation}
In other words, the expected number of blocks in the optimal
solution to the $l_2$ isotonic regression problem is proportional to
the degrees of freedom in this modeling problem. For the standard
($l_2$) lasso regression problem \cite{zou2007degrees} show that for
every regularization parameter $\lambda$ the unbiased estimate for
the degrees of freedom is the number of nonzero coefficients in the
model. Our isotonic $l_2$ lasso problem introduced in Section
\ref{ss:l_2 reg with lasso} above is not a standard lasso problem,
as it has added isotonicity constraints. Thus, it does not comply
with \citep{zou2007degrees} formulation. However, we empirically
evaluated the regularization behavior of the algorithm (Figure
\ref{fig:optimism}). We can see that the number of blocks in the
regularized solution at each value of $\lambda$ is an unbiased
estimate of the number of degrees of freedom not only for the
non-regularized solution ($\lambda=0$) as it suggested in \citep{meyer2000degrees}, but for the entire range of lasso regularization.  While
this explicit result is expected to hold for $l_2$ lasso only, the
important general conclusion is that the lasso-regularized versions
of both the $l_2$ and Bernoulli log-likelihood offer a smooth
regularization approach with gradually increasing model complexity,
allowing flexibility in model selection, as we illustrate in the
next section.

\begin{figure}[h]
\begin{center}
\includegraphics[trim=4.0cm 5.9cm 3.8cm 5.9cm, clip=true,width = 0.76\textwidth]{optimismBW_new2}
\caption{Expected number of blocks and degrees of freedom in lasso
regularized $l_2$ isotonic regression. The same simulation setup was
repeated 1000 times. The observed number of blocks at each $\lambda$
values averaged (dashed line), and the optimism was independently
estimated using (\ref{eq:ERR-MRSS}).  We observe that the number of blocks is an
unbiased estimate of optimism at values of $\lambda$. }
\label{fig:optimism}
\end{center}
\end{figure}


\section{Experiments}
\label{s:experiments} In this section we demonstrate our suggested
algorithm and we choose to focus on isotonic fitting using Bernoulli
log-likelihood with lasso regularization as the most interesting
combination of challenging optimization problem (non-quadratic loss, non differentiable penalty) and useful application. In the
synthetic data experiments we generate covariate variables and
corresponding binary observations according to different models. We
fit isotonic models using a train set and compare our results on the test set with both non-regularized and non-isotonic models. This gives us insight on
the behavior of regularized isotonic modeling in different
environments. In the real world experiments we demonstrate our
algorithm on three commonly used datasets. We again fit a model using a train set and validate our results on a designated test set.  We compare the results we achieve with different modeling methods which are later discussed. We show our suggested algorithm surpasses all of them quite significantly when the isotonic assumption is valid.


\subsection{Synthetic Data Experimental Results}
In the first synthetic data experiment we sample covariate variables
from a standard uncorrelated multi-normal d-dimensional distribution.
The corresponding observations are then generated according to following
model
\begin{align}
y_{i}=\left({\mathrm{sign}\left({\displaystyle \sum_{j=1}^{d}x_{ij}^{3}+a\cdot z_{i}}\right)+1}\right)/2,
\end{align}
where $x_{ij}$ are normally distributed covariate variables, $z_{i}$ is a noise
term sampled from a standard normal distribution, uncorrelated with
$x_{ij}$ and $a$ is the noise standard deviation. Notice that the $x_{ij}^{3}$ transformation is used as a surrogate for an "unknown non-linear relationship". Therefore, we are not interested in comparing to methods that take advantage of the knowledge of this specific transformation to fit appropriate models. \\

\noindent In order to evaluate our predictions we need to determine a desired metric. 
We first notice that the Bernoulli log-likelihood loss function may lead to an unbounded objective in the case of misclassification. The misclassification error metric, on the other hand, may lead to inconsistent behavior as it imposes a "hard decision" instead of a softer fit of probability. We therefore choose to evaluate our predictions using
Mean Square Error (MSE). We repeat this validation multiple times to
achieve an averaged MSE and confidence intervals. We
repeat this procedure on a range of $\lambda$ values to find
the value that achieves minimal MSE.\\

\noindent We start with a two dimensional covariate variables ($d=2$) experiment.
Figure \ref{fig:2d} presents the MSE curve and its corresponding confidence
intervals for different levels of noise (the multiplicative factor
$a$). In each chart the horizontal line corresponds to the MSE of a
standard logistic regression model. Notice that
the point $\lambda=0$ corresponds to a non-regularized isotonic model maximizing Bernoulli log-likelihood.\\

\begin{figure}[h]
\centering
\includegraphics[trim=6cm 1.5cm 7cm 1.5cm, clip=true,angle=270, width = 1\textwidth]{figure1_gray_new}
\caption{2D synthetic data experiments for isotonic Bernoulli log-likelihood modeling with lasso regularization and logistic regression. The horizonal axis corresponds to different $\lambda$ values while the vertical axis is the MSE. Each chart demonstrates to a different level of noise.}
\label{fig:2d}
\end{figure}


\noindent Looking at our results, we may first notice that the trend of the MSE chart is similar in all
six scenarios: it starts with a decrease as $\lambda$ increases,
followed by an increase at larger values of $\lambda$. This suggests
that some regularization does improve the performance of our modeling as we expected.
However, as we increase $\lambda$ we converge towards a constant
$\hat{p}$=$\frac{1}{2}$ model which asymptotically results with
a MSE of 0.25. As we compare to the logistic regression model we see that we
significantly surpass its performance in low noise level scenarios.
However, as we increase the noise level both models fail to perform very
well and achieve MSE values which are closer to 0.25, with a slight
advantage to the logistic regression model. We now increase the dimension ($d=3,4$) and repeat the experiment. Figure \ref{fig:34d} presents the MSE for different
noise levels.

\begin{figure}[h]
\centering
\includegraphics[trim=4.7cm 4.3cm 5cm 3.8cm, clip=true,width = 0.9\textwidth]{figure2_gray_new}
\caption{3D and 4D synthetic data experiments for isotonic Bernoulli log-likelihood modeling with lasso regularization and logistic regression.The horizontal axis corresponds to different $\lambda$ values while the vertical axis is the MSE.}
\label{fig:34d}
\end{figure}

\noindent We again observe the same MSE trend, suggesting that in higher
dimensions too we achieve better results by introducing some
regularization. As we compare our performance to logistic regression
we see that the regularized isotonic approach is still preferable in lower noise
level. However, we notice that as we fix the noise level and increase the dimension the isotonic model becomes less favorable.
This happens since the increase of dimension results with fewer partial order constraints between observations, which negatively impacts the effectiveness of the non-parametric isotonic approach. In other words this phenomenon demonstrates the curse of
dimensionality in our isotonic modeling approach. Yet, if the covariate
variables are highly (and positively) correlated then there would
still be some partial order even in high dimensions. Figure \ref{fig:high_d} demonstrates
higher dimensional datasets sampled from an uncorrelated (on the left)
and highly correlated (on the right) multi-normal distribution. We see that
isotonic modeling with uncorrelated covariate variables suffers
from the curse of dimensionality and preforms quite poorly compared to
the logistic regression. However, as we introduce correlation to
the covariate variables the isotonic modeling surpasses the logistic
approach quite significantly, even with 8-dimensional data set.\\

\begin{figure}[h]
\centering
\includegraphics[trim=4.5cm 4.5cm 4cm 3.9cm, clip=true,width = 0.9\textwidth]{figure5_gray_new}
\caption{High dimensional synthetic data experiment for isotonic
Bernoulli log-likelihood modeling with lasso regularization and
logistic regression. The horizontal axis corresponds to different $\lambda$ values while the vertical axis is the MSE. } \label{fig:high_d}
\end{figure}

\noindent We now turn to the second synthetic experiment in which the observations
are generated according to a multiplicative model:
\begin{equation}
y_{i}=\left({\mathrm{sign}\left({\displaystyle \prod_{j=1}^{d}x_{ij}^{3}+a\cdot z_{i}}\right)+1}\right)/2.
\end{equation}
\noindent We follow the same experimental setup to
attain the results presented in Figure \ref{fig:multiplicative}.

\begin{figure}[h]
\centering
\includegraphics[trim=2.2cm 7.5cm 2.2cm 6.6cm, clip=true,width = .9\textwidth]{figure4_gray_new}
\caption{Multiplicative model experiment for isotonic Bernoulli
log-likelihood with lasso regularization and logistic regression. The horizontal axis corresponds to different $\lambda$ values while the vertical axis is the MSE.}
\label{fig:multiplicative}
\end{figure}
\noindent As in the first experiment we observe the same MSE trend with the
same favorable isotonic modeling approach in lower
noise level and lower dimensions. We notice however that the MSE values
are significantly higher compared to the previous experiment due
to a more challenging model structure. More precisely, both modeling
approaches are barely able to achieve results which surpass a constant
model with an MSE value of $0.25$.


\subsection{Real-world Data Experimental Results}

We now turn to examine our suggested method on real-world datasets.
For illustrative purposes we subsample the datasets so the classes are evenly distributed and apply lasso regularization with a constant value of $p=\frac{1}{2}$.
We start with the Adult data set, publicly available at
UCI repository \citep{Bache+Lichman:2013}. The goal of this data
set is to determine whether a person earns over 50K dollars a year. It contains
15 covariate variables and 48842 individuals. For the purpose of our
experiment we select a subset of ordered covariates, leaving the
categorical variables aside. We are then left with the following
six covariate variables: \textit{Age, Education, Capital gain, Capital loss,
Hours per week} and \textit{Sex}. We suggest that these variables are
isotonic in the sense that an educated adult who works more hours-per-week
is more likely to have a higher income than a less educated younger
person who works fewer hours. Figure \ref{fig:realWorld}.A demonstrates test set performance along the regularization path of our isotonic regression algorithm, applied on this data set. We see that indeed, some regularization does improve our performance, compared to the non regularized model.
We would now like to further validate our approach and suggest an experiment
in which we infer the optimal $\lambda$ on the train set rather than on the test set.
In other words, we split the dataset to a train and test sets, conduct a k-fold cross validation on the train set (with a different $k$ for different experiments), choose
the optimal $\lambda$ based on the train set and only then go back to the
test set to evaluate the MSE. This procedure is repeated multiple
times, where each time we choose a different test set, to achieve an averaged MSE and corresponding confidence intervals.
Table \ref{table:realWorldResults} demonstrates our results compared to a logistic regression model, a linear kernel support vector machine (SVM) and a radial basis function (RBF) kernel SVM. 
We see that our suggested approach surpasses all three methods as the RBF kernel SVM demonstrates the most competitive results. 
We further examine our method (and our isotonic assumption), applying a non-negative logistic regression to this data set. The non-negative logistic regression forces non-negative coefficients to the variables which we assume to be isotonic.
This modeling approach shows to achieve approximately the same MSE as the non-constrained logisitic regression.  The reason is that the non-constrained logistic regression already results with non-negative coefficients in five of the six variables, where the single negative coefficient is very close to zero. This also shows our isotonic assumption is likely valid.\\
 

\noindent In the second real data experiment we analyze the Phoneme dataset, a part of the Elana project \footnote{https://www.elen.ucl.ac.be/neural-nets/Research/Projects/ELENA/databases/REAL/phoneme/}. The aim of this dataset is to distinguish between nasal sounds
(class 0) and oral sounds (class 1). The phonemes are
transcribed as follows: \textit{sh} as in she, \textit{dcl} as in dark, \textit{iy} as the vowel
in she, \textit{aa} as the vowel in dark, and \textit{ao} as the first vowel in water.
We argue that some of the covariate variables (the phonemes)
may be isotonic with respect to the observations (oral/nasal sounds). We apply an isotonic Bernoulli log-likelihood model to verify this assumption. Figure \ref{fig:realWorld}.B demonstrates the MSE for different regularization values. As in the previous example we see that some regularization reduces the
MSE quite significantly. This example also demonstrates the convergence of the
confidence interval towards the MSE curve as $\lambda$ increases.
The reason is that as we increase $\lambda$ we tend towards a
constant model which results with a more stable model (bias-variance
trade-off). As in the previous example we conduct an additional
experiment and apply the $\lambda$ inference on the train set. The results we achieve are compared against different modeling methods as appears in Table \ref{table:realWorldResults}. We see that the RBF kernel SVM is the most competitive approach, achieving almost the same MSE as our approach. As we further apply non-negative logistic regression to this data set we notice a slight increase in the MSE, compared to the non-constrained regression. The reason behind this may be that the isotonic assumption in this data set is harder to justify, compared to the previous data set.\\ 
 
\noindent In the third real world data experiment we examine the German Credit dataset which is also available from the UCI repository. This dataset classifies 1000 customers as holding good or bad credit risks and contains 20 covariate variables from which we selected
only the ordered ones: \textit{Status of existing checking account, Savings
account/bonds, Present employment since, Job, Age, Number of existing
credits at this bank, Number of people being liable to provide maintenance
for.} As in the Adult dataset it seems reasonable to assume that these covariates are isotonically associated with the  target variable. Figure \ref{fig:realWorld}.C shows the regularization path of our suggested algorithm, applied on this data set. It is quite evident that when the dataset is relatively small (as in this example)
introducing regularization prevents model over-fitting, hence improves
the performance on the test set. Table \ref{table:realWorldResults} summarizes the results we achieve compared to different modeling methods.  As in previous examples the RBF kernel SVM is the most competitive method, but still achieves a greater MSE than our suggested approach. As we further apply non-negative logistic regression to this data set we validate our isotonic assumption as we witness the same results as the non-constrained regression. 


\begin{figure}[h]
\centering
\includegraphics[trim=3cm 5.2cm 2.75cm 4.7cm,clip=true,width = .85\textwidth]{realDataRevisedPaper1_new}
\caption{Lasso regularized isotonic Bernoulli log-likelihood modeling in the three real world data experiments. The horizontal axis corresponds to different $\lambda$ values while the vertical axis is the MSE.}
\label{fig:realWorld}
\end{figure}




\begin{table}[ht]
\caption{Real world data experiments results. "Our method" refers to our isotonic Bernoulli log-likelihood with lasso regularization method. 
For methods that have parameters (regularization parameter $\lambda$ in both SVM Methods and in our method, and also the kernel parameter $\gamma$ for kernel SVM), these parameters were chosen using 10-fold CV on the training data \newline}

\renewcommand{\baselinestretch}{1}\footnotesize
\label{table:realWorldResults} 
\centering
\begin{tabular}{|M{2cm}|M{1.8cm}|M{2.5cm}|M{1.8cm}|M{1.8cm}|M{1.8cm}|N}  

\hline
\begin{tabular}{@{}c@{}} Dataset \\ ($\#$ train, $\#$ test) \end{tabular}
&\begin{tabular}{@{}c@{}} Logistic\\ Regression \end{tabular}
&\begin{tabular}{@{}c@{}} Non-negative \\  Logistic Regression \end{tabular}
&\begin{tabular}{@{}c@{}}Linear \\  SVM \end{tabular}
&\begin{tabular}{@{}c@{}} RBF \\  SVM \end{tabular}
&\begin{tabular}{@{}c@{}} Our \\  Method \end{tabular}&\\[20pt]

\hline

\begin{tabular}{@{}c@{}} Adult \\ $(14896,784)$ \end{tabular}   
&\begin{tabular}{@{}c@{}}$0.1290$ \\  $(\pm1.6\cdot10^{-4})$\end{tabular}
&\begin{tabular}{@{}c@{}}$0.1288$ \\  $(\pm1.5\cdot10^{-4})$\end{tabular}
&\begin{tabular}{@{}c@{}}$0.1314$ \\ $(\pm3.9\cdot10^{-4})$\end{tabular}
&\begin{tabular}{@{}c@{}}$0.1295$ \\ $(\pm4.2\cdot10^{-4})$\end{tabular}
&\begin{tabular}{@{}c@{}}$\bold{0.1248}$ \\ $(\pm4.8\cdot10^{-4})$\end{tabular}   & \\[32pt]  

\hline


\begin{tabular}{@{}c@{}} Phoneme \\ $(4860,540)$ \end{tabular}     
&\begin{tabular}{@{}c@{}}$0.1756$ \\  $(\pm1.1\cdot10^{-5})$\end{tabular}
&\begin{tabular}{@{}c@{}}$0.1781$ \\  $(\pm1.0\cdot10^{-5})$\end{tabular}
&\begin{tabular}{@{}c@{}}$0.1632$ \\ $(\pm4.9\cdot10^{-5})$\end{tabular}
&\begin{tabular}{@{}c@{}}$\bold{0.1545}$ \\ $(\pm7.2\cdot10^{-5})$ \end{tabular}
&\begin{tabular}{@{}c@{}}$0.1546$ \\  $(\pm7.3\cdot10^{-4})$\end{tabular}   & \\[32pt]   
\hline






\begin{tabular}{@{}c@{}} German \\ credit \\$(900,100)$ \end{tabular}     
&\begin{tabular}{@{}c@{}}$0.2031$ \\  $(\pm1.9\cdot10^{-5})$\end{tabular}
&\begin{tabular}{@{}c@{}}$0.2031$ \\  $(\pm1.9\cdot10^{-5})$\end{tabular}
&\begin{tabular}{@{}c@{}}$0.2108$ \\ $(\pm8.1\cdot10^{-5})$\end{tabular}
&\begin{tabular}{@{}c@{}}$0.2011$ \\ $(\pm8.5\cdot10^{-5})$ \end{tabular}
&\begin{tabular}{@{}c@{}}$\bold{0.1985}$ \\  $(\pm9.8\cdot10^{-5})$\end{tabular}   & \\[32pt]   
\hline





\end{tabular}
\end{table}
\vspace{1em}

\section{Discussion}
\label{s:conclusion} In this work we present an approach for isotonic modeling
with non-differentiable loss functions. Based on the subdifferential
KKT conditions of the problem, our method
introduces a greedy partitioning algorithm which in every
step solves a simple LP to split the observations into isotonic
blocks while decreasing the global loss. Our partitioning
algorithm is proven to converge to the optimal solution
while maintaining the isotonic constraints in each of its
steps. In addition we show a connection between the number
of blocks in the optimal solution and the degrees of
freedom of our problem. In our practical part we focus on
log-likelihood losses with lasso regularization. Through
synthetic and real world data experiments we demonstrate
the isotonic lasso-regularized Bernoulli log-likelihood
modeling approach, and compare it to standard modeling
approaches. We show that for datasets in which the isotonic
assumption is reasonable, the isotonic model consistently
achieves better results than these competitors. Moreover,
we show that through lasso regularization we significantly
improve the predictive performance of the model. We thus
recommend regularized isotonic modeling (with both
differentiable and non-differentiable loss functions) as a
useful tool in the predictive modeling toolbox.


==> Chapters/Optimal_GP_Designs.tex <==
\section{Introduction}
\begin{comment}
Gaussian Processes are used to model data in numerous scientific and
engineering fields and applications, including geostatistics
(\citealt{Cressie}), machine learning (\citealt{Ordinal}),
electronics (\citealt{Semiconductors}) and many others. In
particular, it has gained popularity in recent years in the field of
computer experiments (\citealt{Sacks}), where it is often used as a
surrogate model for an otherwise rather complex mathematical model,
coded into computer programs whose run time is typically long. As
the computer run time increases, strategic choice of the set of
inputs becomes a necessity. Suitable sampling methods include
model-independent designs like Latin hypercube sampling of different
types as in \cite{LHS} or criterion-based designs which relate
directly to the underlying Gaussian process model, such as the maximum entropy design
suggested by \cite{Shewry}. Thorough reviews of the above (and many
other criteria and methods) can be found in \cite{Kleijnen},
\cite{jones+johnson}, as well as in \cite{Sigal}.\\
\end{comment}

\noindent Minimum integrated mean squared prediction error (IMSPE) designs in the
setting of computer experiments were first introduced by
\cite{Sacks}. They have been elaborately described by
\citet[chapter~5]{santner}, and implemented in JMP's Design of
Experiments package. \cite{picheny} used the IMSPE criterion to choose inputs sequentially in their
exploration of regions of special interest within an experimental
region. Numerical integration has been the method of choice for
deriving minimum IMSPE designs.
In this article, we study the nature of the criterion and propose an
alternative.\\

\noindent In Section \ref{IMSE_Intro} we use Mercer's Theorem and the
Karhunen-Lo\`eve decomposition of random processes to shed new light on the
integrated mean squared prediction error criterion, provide a lower bound
and explain what it means to achieve it. In Section \ref{error} we give guidelines
to controlling the relative approximation error, based on the energy conserved when
truncating the Karhunen-Lo\`eve expansion.
We proceed from theory to practice in Section
\ref{simulation} by working an example with an anisotropic,
two-dimensional process, and generate several minimum integrated
mean squared prediction error designs. We then proceed
in Section \ref{batch} to take advantage of the structured nature of
our criterion to suggest a sequential sampling scheme in batches
(often referred to as ``adaptive design''), and then extend
our framework in Section \ref{unknown_inter} to the slightly more
complicated case of an unknown model intercept, where we investigate
the optimality (or lack thereof) of the designs derived in earlier
sections.\\


\noindent The perception of the Gaussian process model as an infinite
Bayesian linear regression model motivates design criteria that extend
beyond IMSPE-optimality. Two such criteria are Bayesian A-optimality, which
we discuss in Section \ref{A-opt}, and Bayesian D-optimality in Section \ref{D-opt}.
We compare the different optimal designs with the maximin Latin hypercube design
and study their robustness with respect to the correlation parameters in Section \ref{sec:comparison}.
We conclude with a discussion in Section \ref{discussion}.



\section{Spectral Decomposition and Integrated Mean Squared Prediction Error}\label{IMSE_Intro}
\begin{comment}
\subsection{The Classical Approach to Minimum IMSPE Designs}\label{classical}
In their seminal paper, \cite{Sacks} proposed to model a deterministic computer response in the experimental region $\mathcal{X}\subset\mathbb{R}^d$, typically compact and simply connected, as a realization of a stochastic process
\begin{align}\label{univer_krig}
y\ofx = \boldsymbol{f}^{\mathsf{T}}\ofx\boldsymbol{\beta} + Z\ofx\spc,
\end{align}
where $$\boldsymbol{f}\ofx=\left[f_1\ofx,\ldots,f_p\ofx\right]^{\mathsf{T}}$$ is a vector of known regression functions, $$\boldsymbol{\beta}=\left[\beta_1,\ldots,\beta_p\right]^{\mathsf{T}}$$ is a vector of parameters and $Z(\boldsymbol{x})$ is a stationary Gaussian process with mean 0, correlation function
$R(\boldsymbol{x}_1,\boldsymbol{x}_2)=R\left(\boldsymbol{x}_1-\boldsymbol{x}_2\right)$
and marginal variance $\sigma^2$.\\

\noindent Let $\boldsymbol{y} =
\left[y(\boldsymbol{x}_1),\ldots,y(\boldsymbol{x}_n)\right]^{\mathsf{T}}$
be the set of measurements at the experimental design $\mathcal{D} =
\left\{\boldsymbol{x}_1,\ldots,\boldsymbol{x}_n\right\}\subset
\mathcal{X}$ and denote by $\boldsymbol{F}$ the matrix whose
elements are $\boldsymbol{F}_{ij} = f_j(\boldsymbol{x}_i)$. It is common
practice to make predictions at new sites $\boldsymbol{x}$ using
the best linear unbiased predictor, which here matches the universal
Kriging predictor
\begin{align}\label{univ_krig_pred}
\widehat{y}\ofx = \mathbb{E}\left\{y(\boldsymbol{x})\big|\boldsymbol{y}\right\} = \boldsymbol{f}^{\mathsf{T}}\ofx\widehat{\boldsymbol{\beta}} + \boldsymbol{r}^{\mathsf{T}}\ofx\boldsymbol{R}^{-1}\left(\boldsymbol{y}-\boldsymbol{F}\widehat{\boldsymbol{\beta}}\right)\spc,
\end{align}
where $\boldsymbol{r}(\boldsymbol{x}) =
\left[R(\boldsymbol{x},\boldsymbol{x}_1),\ldots,R(\boldsymbol{x},\boldsymbol{x}_n)\right]^{\mathsf{T}}$
is the vector of correlations, $\boldsymbol{R}_{ij} =
R(\boldsymbol{x}_i,\boldsymbol{x}_j)$ is the correlation matrix at the design sites and
\begin{align}\label{WLS}
\widehat{\boldsymbol{\beta}} = \left(\boldsymbol{F}^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{F}\right)^{-1}\boldsymbol{F}^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{y}
\end{align}
is the generalized least squares estimator.\\

\noindent Using (\ref{univ_krig_pred}), yields the mean squared prediction error
\begin{align}\label{MSPE_universal}
\mathrm{MSPE} &=
\mathbb{E}\left[\big\{\widehat{y}(\boldsymbol{x})-y(\boldsymbol{x})\big\}^2\Big|\boldsymbol{y}\right]\\[1em] &=\var\left\{y(\boldsymbol{x})\big|\boldsymbol{y}\right\} =
\sigma^2\left\{1 - \left[\boldsymbol{f}^{\mathsf{T}}\ofx\hspace{.7em}\boldsymbol{r}^{\mathsf{T}}\ofx\right]
\left[
\begin{array}{ccc}
\boldsymbol{0} & &\boldsymbol{F}^{\mathsf{T}}\\[.5em]
\boldsymbol{F} & &\boldsymbol{R}
\end{array}
\right]^{-1}
\left[
\begin{array}{c}
\boldsymbol{f}\ofx\\[.1em]
\boldsymbol{r}\ofx
\end{array}
\right]\right\}
\spc,
\end{align}
and \cite{IMSE} generated experimental designs which minimize the Integrated MSPE (IMSPE) criterion
\begin{align}\label{IMSPE_original}
\dfrac{\mathcal{J}\left(\mathcal{D},\widehat{y}\right)}{\sigma^2}=\mathrm{vol}\left(\mathcal{X}\right)-\mathrm{tr}
\left\{
\left[
\begin{array}{ccc}
\boldsymbol{0} & &\boldsymbol{F}^{\mathsf{T}}\\[.5em]
\boldsymbol{F} & &\boldsymbol{R}
\end{array}
\right]^{-1}\int_{\mathcal{X}}
\left[
\begin{array}{ccc}
\boldsymbol{f}\ofx\boldsymbol{f}^{\mathsf{T}}\ofx & &\boldsymbol{f}\ofx\boldsymbol{r}^{\mathsf{T}}\ofx\\[.5em]
\boldsymbol{r}\ofx\boldsymbol{f}^{\mathsf{T}}\ofx & &\boldsymbol{r}\ofx\boldsymbol{r}^{\mathsf{T}}\ofx
\end{array}
\right]
\di \boldsymbol{x}
\right\}
\end{align}
where $\mathrm{vol}(\mathcal{X})$ is the volume (the Lebesgue measure) of the experimental region $\mathcal{X}$.
The numerical integration is often simplified when both the
regressors and the correlation function are separable, reducing the
calculation to evaluating multiple univariate integrals. See
\citet[chapter~3]{santner} for details.
\end{comment}

\subsection{IMSPE-optimal Designs: a Short Review}\label{classical}
\noindent As we mentioned earlier, in Chapter \ref{overview},
when we model a deterministic computer response in the experimental region $\mathcal{X}\subset\mathbb{R}^d$, typically compact and simply connected, as a realization of a stochastic process
\begin{align}\label{univer_krig}
y\ofx = \boldsymbol{f}^{\mathsf{T}}\ofx\boldsymbol{\beta} + Z\ofx\spc,
\end{align}
the mean squared prediction error is given by
\begin{align}\label{MSPE_universal}
\mathrm{MSPE} &=
\mathbb{E}\left[\big\{\widehat{y}(\boldsymbol{x})-y(\boldsymbol{x})\big\}^2\Big|\boldsymbol{y}\right]\\[1em] &=\var\left\{y(\boldsymbol{x})\big|\boldsymbol{y}\right\} =
\sigma^2\left\{1 - \left[\boldsymbol{f}^{\mathsf{T}}\ofx\hspace{.7em}\boldsymbol{r}^{\mathsf{T}}\ofx\right]
\left[
\begin{array}{ccc}
\boldsymbol{0} & &\boldsymbol{F}^{\mathsf{T}}\\[.5em]
\boldsymbol{F} & &\boldsymbol{R}
\end{array}
\right]^{-1}
\left[
\begin{array}{c}
\boldsymbol{f}\ofx\\[.1em]
\boldsymbol{r}\ofx
\end{array}
\right]\right\}
\spc,
\end{align}
where $\widehat{y}(\boldsymbol{x})$ is the universal Kriging predictor
\begin{align}\label{univ_krig_pred}
\widehat{y}\ofx = \mathbb{E}\left\{y(\boldsymbol{x})\big|\boldsymbol{y}\right\} = \boldsymbol{f}^{\mathsf{T}}\ofx\widehat{\boldsymbol{\beta}} + \boldsymbol{r}^{\mathsf{T}}\ofx\boldsymbol{R}^{-1}\left(\boldsymbol{y}-\boldsymbol{F}\widehat{\boldsymbol{\beta}}\right)\spc.
\end{align}
\noindent \cite{IMSE} generated experimental designs $\mathcal{D}=\left\{\bx_1,\ldots,\bx_n\right\}\subset\mathcal{X}$, which minimized the Integrated MSPE (IMSPE) criterion
\begin{align}\label{IMSPE_original}
\dfrac{\mathcal{J}\left(\mathcal{D},\widehat{y}\right)}{\sigma^2}=\mathrm{vol}\left(\mathcal{X}\right)-\mathrm{tr}
\left\{
\left[
\begin{array}{ccc}
\boldsymbol{0} & &\boldsymbol{F}^{\mathsf{T}}\\[.5em]
\boldsymbol{F} & &\boldsymbol{R}
\end{array}
\right]^{-1}\int_{\mathcal{X}}
\left[
\begin{array}{ccc}
\boldsymbol{f}\ofx\boldsymbol{f}^{\mathsf{T}}\ofx & &\boldsymbol{f}\ofx\boldsymbol{r}^{\mathsf{T}}\ofx\\[.5em]
\boldsymbol{r}\ofx\boldsymbol{f}^{\mathsf{T}}\ofx & &\boldsymbol{r}\ofx\boldsymbol{r}^{\mathsf{T}}\ofx
\end{array}
\right]
\di \boldsymbol{x}
\right\}
\end{align}
where $\mathrm{vol}(\mathcal{X})$ is the volume (the Lebesgue measure) of the experimental region $\mathcal{X}$.
The numerical integration is often simplified when both the
regressors and the correlation function are separable, reducing the
calculation to evaluating multiple univariate integrals. See
\citet[chapter~3]{santner} for details.


\subsection{A Spectral Approach Based on the Karhunen-Lo\`eve Expansion}

\noindent Although the general model includes an arbitrary
regression function, many authors have limited the model to an
intercept, using the covariance function to model the dependence on
$\boldsymbol{x}$ (see, for example, \citealt{IMSE} and
\citealt{Dizza}). This leads to the simpler Gaussian process model
\begin{align}\label{gauss_proc}
y(\boldsymbol{x}) = \beta_0 + Z(\boldsymbol{x})\spc,
\end{align}
where $Z(\boldsymbol{x})$ is a stationary
Gaussian process as in Subsection \ref{classical}.\\

\noindent Suppose now that $R(,)\in \mathcal{C}\left(\mathcal{X}^2\right)$ and
consider the Karhunen-Lo\`eve expansion of $Z(\boldsymbol{x})$ (see
\citealt[chapter~1]{Wahba}),
\begin{align}\label{model}
Z(\boldsymbol{x}) = \sum_{i=1}^{\infty}\alpha_i\varphi_i(\boldsymbol{x})\spc,
\end{align}
where the $\alpha$'s are independent
$\mathcal{N}(0,\lambda_i)$ random variables and the $\lambda_i$'s and
$\varphi_i$'s are the eigenvalues and the pairwise orthogonal
eigenfunctions, respectively, of the integral operator defined by
$R(\cdot,\cdot)$, i.e.
\begin{align}\label{eigenfuncs}
\int_{\mathcal{X}} R(\boldsymbol{x},\boldsymbol{y})\varphi_i(\boldsymbol{y})\di \boldsymbol{y} = \lambda_i\varphi_i(\boldsymbol{x})
\end{align}
and
\begin{align}\label{orthogonal}
\int_{\mathcal{X}}\varphi_i(\boldsymbol{x})\varphi_j(\boldsymbol{x})\di \boldsymbol{x} = \delta_{ij},
\end{align}
where $\delta_{ij}$ is Kronecker's delta.\\

\noindent We assume for now that $\beta_0$ is a known constant.  In that case, using the same notation as in Subsection \ref{classical},
for an arbitrary $\boldsymbol{x}\in\mathcal{X}$
\begin{align*}
y(\boldsymbol{x})\big|\boldsymbol{y}\sim\mathcal{N}\bigg[\beta_0 +
\boldsymbol{r}^{\mathsf{T}}(\boldsymbol{x})\boldsymbol{R}^{-1}\left(\boldsymbol{y}-\beta_0\boldsymbol{1}_n\right)\spc,\spc
\sigma^2\left\{1-\boldsymbol{r}^{\mathsf{T}}(\boldsymbol{x})\boldsymbol{R}^{-1}\boldsymbol{r}(\boldsymbol{x})\right\}\bigg]\spc.
\end{align*}
Denoting the ordinary Kriging estimator at $\boldsymbol{x}$ by
\begin{align}\label{kriging}
\widehat{y}(\boldsymbol{x}) = \mathbb{E}\left\{y(\boldsymbol{x})\big|\boldsymbol{y}\right\} = \beta_0 + \boldsymbol{r}^{\mathsf{T}}(\boldsymbol{x})\boldsymbol{R}^{-1}\left(\boldsymbol{y}-\beta_0\boldsymbol{1}_n\right)\spc,
\end{align}
the MSPE at $\boldsymbol{x}$ is given by
\begin{align}\label{MSE_Expression}
\mathbb{E}\left[\big\{\widehat{y}(\boldsymbol{x})-y(\boldsymbol{x})\big\}^2\Big|\boldsymbol{y}\right] = \var\left\{y(\boldsymbol{x})\big|\boldsymbol{y}\right\} = \sigma^2\left\{1-\boldsymbol{r}^{\mathsf{T}}(\boldsymbol{x})\boldsymbol{R}^{-1}\boldsymbol{r}(\boldsymbol{x})\right\}\spc.
\end{align}
The IMSPE, according to
(\ref{MSE_Expression}) (assuming $\mathcal{X}$ is compact), is thus
\begin{align}\label{IMSE1}
\mathcal{J}\left(\mathcal{D},\widehat{y}\right) = \int_{\mathcal{X}}\mathbb{E}\left[\big\{\widehat{y}(\boldsymbol{x})-y(\boldsymbol{x})\big\}^2\Big|\boldsymbol{y}\right]\di \boldsymbol{x} = \sigma^2\left\{\mathrm{vol}(\mathcal{X})-\int_{\mathcal{X}}\boldsymbol{r}^{\mathsf{T}}(\boldsymbol{x})\boldsymbol{R}^{-1}\boldsymbol{r}(\boldsymbol{x})\di \boldsymbol{x}\right\}\spc.
\end{align}

\noindent From Mercer's Theorem we have the representation
\begin{align}\label{mercer}
R(\boldsymbol{x},\boldsymbol{y}) = \sum_{i=1}^{\infty}\lambda_i\varphi_i(\boldsymbol{x})\varphi_i(\boldsymbol{y})\spc,
\end{align}
$\lambda_1\geq\lambda_2\geq\cdots>0$ are all real, and convergence in (\ref{mercer}) is absolute and uniform,
hence
\begin{align}\label{IMSE2}
\boldsymbol{r}(\boldsymbol{x})^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{r}(\boldsymbol{x}) &= \sum_{i=1}^n\sum_{j=1}^n\boldsymbol{R}^{-1}_{ij}\sum_{k=1}^{\infty}\lambda_k\varphi_k(\boldsymbol{x}_i)\varphi_k(\boldsymbol{x})\sum_{l=1}^{\infty}\lambda_l\varphi_l(\boldsymbol{x}_j)\varphi_l(\boldsymbol{x})\nonumber\\[1em]
&= \sum_{k=1}^{\infty}\sum_{l=1}^{\infty}\left\{\sum_{i=1}^n\sum_{j=1}^n\lambda_k\lambda_l\boldsymbol{R}^{-1}_{ij}\varphi_k(\boldsymbol{x}_i)\varphi_l(\boldsymbol{x}_j)\right\}\varphi_k(\boldsymbol{x})\varphi_l(\boldsymbol{x})\nonumber\\[1em]
& = \sum_{k=1}^{\infty}\sum_{l=1}^{\infty}\left\{\lambda_k\lambda_l\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_l\right\}\varphi_k(\boldsymbol{x})\varphi_l(\boldsymbol{x})\spc,
\end{align}
where $\boldsymbol{\phi}_p = \left[\varphi_p(\boldsymbol{x}_1),\ldots,\varphi_p(\boldsymbol{x}_n)\right]^{\mathsf{T}}$\spc.\\

\noindent Using (\ref{orthogonal}) and (\ref{IMSE2}) in (\ref{IMSE1}) we have
\begin{align}\label{IMSE3}
\frac{\mathcal{J}\left(\mathcal{D},\widehat{y}\right)}{\sigma^2} = \mathrm{vol}(\mathcal{X}) - \sum_{k=1}^{\infty}\lambda_k^2\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k\spc.
\end{align}

\noindent An IMSPE-optimal design would therefore be $\mathcal{D^*} = \displaystyle\argmax_{\mathcal{D}}\hspace{.1em}\sum_{k=1}^{\infty}\lambda_k^2\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k$ .\\

\noindent For the rest of this chapter it will be convenient to assume that
$\sigma^2=1$.  Our results are affected by this assumption only via
the scaling evident in (\ref{IMSE3}).

\noindent Other works that discuss Mercer's expansion of covariance
kernels in the context of optimal experimental designs include
\cite{Muller2} and \cite{Muller1}.\\

\noindent We will now give a characterization of the structure of an ideal IMSPE-optimal design. We then proceed to work out an example in
Section \ref{simulation} and analyze it in light of these results.


\begin{lemma}\label{Steves_Lemma}
For any size $n$ design $\mathcal{D}$
\begin{enumerate}
\item
$\displaystyle\sum_{j=1}^{\infty}\lambda_j\boldsymbol{\phi}_j^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_j=n$\spc.
\item
For all $k\in\mathbb{N}$, $\lambda_k\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k\leq1$ \spc.
\end{enumerate}
\end{lemma}
\begin{proof}
\text{ }\\
\vspace{-3.5em}
\begin{enumerate}
\item
\begin{align*}
n&=\mathrm{tr}\left\{\boldsymbol{I}\right\} = \sum_{i=1}^n\left[\boldsymbol{R}^{-1}\boldsymbol{R}\right]_{ii} = \sum_{i=1}^n\sum_{k=1}^n\boldsymbol{R}^{-1}_{ik}R\left(\boldsymbol{x}_k,\boldsymbol{x}_i\right)\\[1em]&=\sum_{i=1}^n\sum_{k=1}^n\boldsymbol{R}^{-1}_{ik}\sum_{j=1}^{\infty}\lambda_j\varphi_j\left(\boldsymbol{x}_k\right)\varphi_j\left(\boldsymbol{x}_i\right) = \sum_{j=1}^{\infty}\lambda_j\sum_{i=1}^n\sum_{k=1}^n\boldsymbol{R}^{-1}_{ik}\varphi_j\left(\boldsymbol{x}_i\right)\varphi_j\left(\boldsymbol{x}_k\right) \\[1em] &= \sum_{j=1}^{\infty}\lambda_j\boldsymbol{\phi}_j^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_j\spc.
\end{align*}

\item
\fontfamily{phv}\selectfont{
Since
$\boldsymbol{R} = \displaystyle\sum_{j=1}^{\infty}\lambda_j\boldsymbol{\phi}_{j}\boldsymbol{\phi}_{j}^{\mathsf{T}}$ ,
we may write $$\boldsymbol{R} = \boldsymbol{R}_{(k)} + \boldsymbol{R}_{(-k)}\spc,$$ where
$
\boldsymbol{R}_{(k)} = \lambda_k\boldsymbol{\phi}_{k}\boldsymbol{\phi}_{k}^{\mathsf{T}}$ , $\boldsymbol{R}_{(-k)} = \displaystyle\sum_{j\ne k}\lambda_j\boldsymbol{\phi}_{j}\boldsymbol{\phi}_{j}^{\mathsf{T}}$ and $\boldsymbol{R}$, $\boldsymbol{R}_{(k)}$ and $\boldsymbol{R}_{(-k)}$ are all symmetric, positive semi-definite matrices. Now, $\boldsymbol{R}-\boldsymbol{R}_{(k)}=\boldsymbol{R}_{(-k)}\succeq \boldsymbol{0}$, hence $\boldsymbol{R}\succeq\boldsymbol{R}_{(k)}$, and thus for any $\varepsilon>0$, $\boldsymbol{R}+\varepsilon\boldsymbol{I}\succeq\boldsymbol{R}_{(k)}+\varepsilon\boldsymbol{I}$ , or equivalently $$\left[\boldsymbol{R}+\varepsilon\boldsymbol{I}\right]^{-1}\preceq\left[\boldsymbol{R}_{(k)}+\varepsilon\boldsymbol{I}\right]^{-1}\spc.$$
Having established that,
\begin{align*}
\boldsymbol{\phi}_k^{\mathsf{T}}\left[\boldsymbol{R}+\varepsilon\boldsymbol{I}\right]^{-1}\boldsymbol{\phi}_k&\leq\boldsymbol{\phi}_k^{\mathsf{T}}\left[\boldsymbol{R}_{(k)}+\varepsilon\boldsymbol{I}\right]^{-1}\boldsymbol{\phi}_k=\boldsymbol{\phi}_k^{\mathsf{T}}\left[\lambda_k\boldsymbol{\phi}_{k}\boldsymbol{\phi}_{k}^{\mathsf{T}}+\varepsilon\boldsymbol{I}\right]^{-1}\boldsymbol{\phi}_k \\[1em]&= \boldsymbol{\phi}_k^{\mathsf{T}}\left\{\frac{1}{\varepsilon}\left[\boldsymbol{I}-\frac{\lambda_k}{\varepsilon+\lambda_k\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{\phi}_k}\boldsymbol{\phi}_{k}\boldsymbol{\phi}_{k}^{\mathsf{T}}\right]\right\}\boldsymbol{\phi}_k = \frac{\boldsymbol{\phi}_{k}^{\mathsf{T}}\boldsymbol{\phi}_{k}}{\varepsilon + \lambda_k\boldsymbol{\phi}_{k}^{\mathsf{T}}\boldsymbol{\phi}_{k}}\spc,
\end{align*}
hence
\begin{align*}
\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k=\lim_{\varepsilon\to0}\boldsymbol{\phi}_k^{\mathsf{T}}\left[\boldsymbol{R}+\varepsilon\boldsymbol{I}\right]^{-1}\boldsymbol{\phi}_k\leq\frac{1}{\lambda_k}\spc.
\end{align*}
}
\end{enumerate}
\end{proof}

\begin{theorem}\label{big_one}
Let $\mathcal{D}$ be a size $n$ design satisfying
\begin{align}\label{big_theorem}
\lambda_k\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k =
\begin{cases}
\begin{array}{ccc}
1 & &k\leq n\spc,\\[1em]
0 & &k>n\spc.
\end{array}
\end{cases}
\end{align}
Then $\mathcal{J}\left(\mathcal{D},\widehat{y}\right)\leq\mathcal{J}\big(\widetilde{\mathcal{D}},\widehat{y}\big)$ for any other size $n$ design $\widetilde{\mathcal{D}}\subset\mathcal{X}$; i.e. $\mathcal{D}$ is IMSPE-optimal.  We will call such a design $\mathcal{D}$ an IMSPE-perfect design.
\end{theorem}
\begin{proof}
Denote $u_k\left(\mathcal{D}\right)=\lambda_k\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k$. By Lemma \ref{Steves_Lemma},  the optimization problem for a size $n$ IMSPE-optimal design $\mathcal{D}$ can be written
\begin{align*}
\max_{\mathcal{D}}\hspace{.1em}\sum_{k=1}^{\infty}\lambda_ku_k\left(\mathcal{D}\right)\spc\text{s.t.}\spc\sum_{k=1}^{\infty}u_k\left(\mathcal{D}\right)=n\spc\text{and}\spc 0\leq u_k\left(\mathcal{D}\right)\leq1\spc.
\end{align*}
Because $\lambda_1\geq\lambda_2\geq\cdots>0$ , a design $\mathcal{D}$ for which $u_1=\cdots=u_n=1$ and $u_k=0$ for $k>n$ is IMSPE-optimal.
\end{proof}



\begin{rembold}\label{first_insight}
\fontfamily{phv}\selectfont{
Suppose a design $\mathcal{D}$ is IMSPE-perfect. Then, when evaluated at $\mathcal{D}$, the correlation matrix
$$\boldsymbol{R} = \displaystyle\sum_{j=1}^{\infty}\lambda_j\boldsymbol{\phi}_{j}\boldsymbol{\phi}_{j}^{\mathsf{T}} = \displaystyle\sum_{j=1}^{n}\lambda_j\boldsymbol{\phi}_{j}\boldsymbol{\phi}_{j}^{\mathsf{T}}$$
depends only on the first $n$ eigenfunctions. Likewise, the vector of correlations at any $\boldsymbol{x}\in\mathcal{X}$,
$$\boldsymbol{r}\ofx = \displaystyle\sum_{j=1}^{\infty}\lambda_j\varphi_j\left(\boldsymbol{x}\right)\boldsymbol{\phi}_{j} = \displaystyle\sum_{j=1}^{n}\lambda_j\varphi_j\left(\boldsymbol{x}\right)\boldsymbol{\phi}_{j}$$ will be independent of $\varphi_{n+1}\ofx$, $\varphi_{n+2}\ofx,\ldots$ It follows that the prediction $\widehat{y}\ofx$ at any $\boldsymbol{x}\in\mathcal{X}$, given by (\ref{kriging}), will be identical to the prediction based on the finite-dimensional Bayesian linear regression model
$$y\ofx = \alpha_1\varphi_1\ofx + \cdots + \alpha_n\varphi_n\ofx$$ with priors given by independent random variables $\alpha_j\sim\mathcal{N}\left(0\hspace{.1em},\hspace{.1em}\lambda_j\right)$ , $j=1,\ldots,n$ . Although IMSPE-perfect designs generally do not exist, this insight tells us that the pursuit of an IMSPE-optimal design is in fact an attempt to reduce the Gaussian process model to the most parsimonious Bayesian linear regression model that we can fit without losing any information.
}
\end{rembold}

\begin{rembold}\label{second_insight}
\fontfamily{phv}\selectfont{
Theorem \ref{big_one} provides us with a lower bound for the IMSPE criterion,
\begin{align}\label{low_bound1}
\mathcal{J}\left(\mathcal{D},\widehat{y}\right) \geq \mathrm{vol}\left(\mathcal{X}\right) - \sum_{k=1}^n\lambda_k\spc.
\end{align}
Moreover,
using the fact that for a stationary Gaussian process
\begin{align}\label{eq:trace_class}
\sum_{k=1}^{\infty}\lambda_k = \int_{\mathcal{X}}R\left(\boldsymbol{x},\boldsymbol{x}\right)\di\boldsymbol{x} = R\left(\boldsymbol{0}\right)\int_{\mathcal{X}}\di \boldsymbol{x} = \mathrm{vol}\left(\mathcal{X}\right)\spc,
\end{align}
(see \citealt{trace_class}) the lower bound (\ref{low_bound1}) can be rewritten as
$$\mathcal{J}\left(\mathcal{D},\widehat{y}\right) \geq \sum_{k=n+1}^{\infty}\lambda_k\spc.$$
}
\end{rembold}

\section{Approximate IMSPE-optimal Designs}\label{error}
The eigenvalues $\left\{\lambda_k\right\}$ are known to decay rather
rapidly. In fact, it has been shown \citep{Frauenfelder} that for
piecewise analytic $R(\boldsymbol{x},\boldsymbol{y})$ there exist
constants $c_1$ and $c_2$ such that $\lambda_k\leq c_1\exp\left(-c_2
k^{1/d}\right)$.  The leading eigenfunctions thus play a dominant
role, which suggests truncating the expansion in (\ref{IMSE3}) at some
index $M$.  We write the approximate IMSPE as
\begin{align}\label{approx_IMSPE}
\widetilde{\mathcal{J}}_{_M}\left(\mathcal{D},\widehat{y}\right) =
\mathrm{vol}(\mathcal{X}) -
\sum_{k=1}^{M}\lambda_k^2\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k
= \mathrm{vol}(\mathcal{X}) -
\mathrm{tr}\left\{\boldsymbol{\Lambda}^2\boldsymbol{\Phi}^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\Phi}\right\}\spc,
\end{align}
where
\begin{align*}
\boldsymbol{\Lambda} =
\mathrm{diag}\left(\lambda_1,\ldots,\lambda_M\right)\spc \text{and}
\spc\boldsymbol{\Phi}_{ij} =
\varphi_{j}\left(\boldsymbol{x}_i\right)\spc , \spc1\leq i \leq
n\spc , \spc1\leq j\leq M\spc.
\end{align*}
An approximate minimum IMSPE
experimental design would then be
\begin{align}\label{Design}
\mathcal{D}^{*}=\displaystyle\argmin_{\mathcal{D}\subset\mathcal{X}}\widetilde{\mathcal{J}}_{_M}\left(\mathcal{D},\widehat{y}\right)
=
\displaystyle\argmax_{\mathcal{D}\subset\mathcal{X}}\mathrm{tr}\left\{\boldsymbol{\Lambda}^2\boldsymbol{\Phi}^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\Phi}\right\}\spc.
\end{align}

\noindent Denote the relative truncation error of order $M$ by
\begin{align}\label{relative_error}
r_{_M} = 1- \dfrac{\displaystyle\sum_{k=1}^M\lambda_k^2\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k}{\displaystyle\sum_{j\geq 1}\lambda_j^2\boldsymbol{\phi}_j^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_j} = \dfrac{\displaystyle\sum_{k\geq M+1}\lambda_k^2\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k}{\displaystyle\sum_{j\geq 1}\lambda_j^2\boldsymbol{\phi}_j^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_j}\spc.
\end{align}
Now, for a fixed $\epsilon>0$, let $M\leq n$ be large enough such that $\displaystyle\sum_{k= M+1}^{\infty}\lambda_k\bigg/\displaystyle\sum_{j=1}^{\infty}\lambda_j\leq\epsilon$. Suppose that $\mathcal{D}$ is a size $n$ design for which $\lambda_j\boldsymbol{\phi}_j^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_j = 1$
for $j=1,\ldots,M$, which we will call an IMSPE $M$-perfect design. Then, from Theorem \ref{big_one} and Remark \ref{second_insight},
\begin{align}\label{rel_err_bound}
r_{_M} = 1- \dfrac{\displaystyle\sum_{k=1}^M\lambda_k}{\displaystyle\sum_{j= 1}^{\infty}\lambda_j^2\boldsymbol{\phi}_j^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_j}\leq
1- \dfrac{\displaystyle\sum_{k=1}^M\lambda_k}{\displaystyle\sum_{j=1}^n\lambda_j}\leq
1- \dfrac{\displaystyle\sum_{k=1}^M\lambda_k}{\displaystyle\sum_{j=1}^{\infty}\lambda_j}\leq\epsilon\spc.
\end{align}
This means that for any $\epsilon > 0$ we can control the relative truncation error  of the approximate IMSPE-optimal design at level $\epsilon$ by choosing $M$ large enough so that $100(1-\epsilon)\%$ of the process' energy is conserved, provided that an IMSPE $M$-perfect design exists.
In practice, as we will demonstrate in Section \ref{simulation}, IMSPE $M$-perfect designs often exist for $M < n$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{A Worked Example}\label{simulation}
We proceed to use (\ref{Design}) to generate approximate minimum
IMSPE designs for a two
dimensional Gaussian process with the Gaussian correlation function
\begin{align}\label{gaussian_cor}
R(\boldsymbol{x},\boldsymbol{w}) =
\exp\left\{-\left(x_1-w_1\right)^2-2\left(x_2-w_2\right)^2\right\}\spc,
\end{align}
where the experimental region is chosen to be
$\mathcal{X}=[-1,1]^2$. In order to derive the decomposition
(\ref{mercer}) one must first solve numerically the integral equation
(\ref{eigenfuncs}), for which Galerkin-type methods may be applied
(see \citealt{Galerkin}). We are helped by the fact that the
correlation function (\ref{gaussian_cor}) is separable, implying that
the set of eigenfunctions corresponding to
$R(\boldsymbol{x},\boldsymbol{w})$ consists of functions of the
form
$\left\{\varphi_i(h_1)\psi_j(h_2)\right\}$,
where $\left\{\varphi_i\right\}$ and $\left\{\psi_j\right\}$ are the
eigenfunctions corresponding to the univariate correlation functions
\begin{align*}
R_1\left(h_1\right) = \exp\left\{-h_1^2\right\}\spc \text{and}
\spc R_2\left(h_2\right) = \exp\left\{-2h_2^2\right\}\spc,
\end{align*}
respectively (here $\boldsymbol{h} = \boldsymbol{x}-\boldsymbol{w}$). Similarly, the set of eigenvalues corresponding to
$R(\boldsymbol{x},\boldsymbol{w})$ is of the form
$\left\{\lambda_i\mu_j\right\}$, where $\left\{\lambda_i\right\}$
and $\left\{\mu_j\right\}$ are the sets of eigenvalues corresponding
to the univariate processes mentioned above. All figures appearing in
this chapter are based on the correlation function (\ref{gaussian_cor}).\\


\noindent To solve (\ref{eigenfuncs}) for the univariate case, we follow the
path described in \citet[chapter~4]{Rasmussen}.  We choose a grid of
size $L$, $-1\leq t_1 < t_2 <\cdots < t_L \leq 1$, and calculate the
spectral decomposition
$\widetilde{\boldsymbol{R}}=\boldsymbol{U}\boldsymbol{D}\boldsymbol{U}^\top$,
where $\widetilde{\boldsymbol{R}}$ is the Gram matrix
$\widetilde{\boldsymbol{R}}_{ij}=R(t_i,t_j)$.  Arranging the
diagonal of $\boldsymbol{D}$ in decreasing order, the first $M$
eigenvalues of the correlation function are then approximated by
$\lambda_i = 2\boldsymbol{D}_{ii}/L$ and the value of the $i$-th
eigenfunction at any $x\in [-1,1]$ is approximated by Nystr\"{o}m's
method as
\begin{align*}
\varphi_i(x)\approx \dfrac{L^{1/2}}{2^{1/2}\boldsymbol{D}_{ii}}\hspace{.1em}\boldsymbol{r}^{\mathsf{T}}(x)\boldsymbol{u}_i\spc,
\end{align*}
where $\boldsymbol{r}(x) =
\left[R(x,t_1),\ldots,R(x,t_L)\right]^{\mathsf{T}}$ and
$\boldsymbol{u}_i$ is the $i$-th column of the eigenvector matrix
$\boldsymbol{U}$. Other interpolation methods (e.g. interpolating splines)
are acceptable when the grid is reasonably fine.\\

\noindent The numerical approach here parallels the one proposed by
\cite{Dizza} to explore regression aspects of Gaussian process
models.

\begin{figure}[ht]
\centering
\includegraphics[width=0.6\textwidth]{EigenVals.pdf}
\caption{First $17$
eigenvalues of the Fredholm integral operator for the Gaussian
correlation function $R(\boldsymbol{x},\boldsymbol{w}) =
\exp\left\{-\left(x_1-w_1\right)^2-2\left(x_2-w_2\right)^2\right\}$
in the logarithmic scale.}
  \label{Eigenvals}
\end{figure}



\noindent In our example we chose a uniform grid of size $50$ for the
univariate processes. By truncating the (two dimensional) expansion
(\ref{model}) at $M=17$, we still retained $99.51\%$ of the process'
energy - calculated by
$\sum_{i=1}^{17}\lambda_i/\sum_{j=1}^{2500}\lambda_j$ . Figure
\ref{Eigenvals} shows the $17$ largest eigenvalues in the
logarithmic scale; Figure \ref{Eigenfuncs} shows the first $6$
eigenfunctions, which serve as the building blocks of the process.
Figure \ref{Realization} displays a single realization of the
truncated process, obtained by taking a random combination of the
first $17$ eigenfunctions, as in (\ref{model}). Not surprisingly
(given the properties of the Gaussian kernel), the resulting surface
is the graph of a $\mathcal{C}^{\infty}$ function. In Figure \ref{IMSPE_Designs}
the reader gets to see the resulting designs for several sample sizes.

\begin{figure}[ht!]
\centering
\includegraphics[width=.9\textwidth]{EigenFuncs_colors.pdf}
\caption{First $6$ eigenfunctions}
  \label{Eigenfuncs}
\end{figure}

\begin{figure}[ht!]
\centering
\includegraphics[width=.9\textwidth]{Realization.pdf}
\caption{A single realization from the truncated process.}
  \label{Realization}
\end{figure}


\begin{figure}[ht!]
\centering
\includegraphics[width=.33\textwidth, angle=90]{SeveralDesigns.pdf}
  \caption{Approximate minimum IMSPE designs consisting of $7$, $15$ and $25$ points.}
  \label{IMSPE_Designs}
\end{figure}


\noindent Note that we chose $M=17$ as it is the smallest $M$ to satisfy
$$\epsilon=\sum_{k=M+1}^{\infty}\lambda_k\Bigg/\sum_{j=1}^{\infty}\lambda_j=4.92\times10^{-3}< 0.005\spc.$$
We then proceeded to generate approximate minimum IMSPE designs of various sizes.
\begin{figure}[ht]
\centering
\subfloat[][]{\label{Rel_Error}\includegraphics[width=.5\textwidth]{Relative_Error.pdf}}
  \subfloat[][]{\label{First_Terms}\includegraphics[width=0.5\textwidth]{First_17_Terms.pdf}}
    \caption{Left panel: Ideal and true relative truncation error vs. $n$. Right panel: Analyzing the $17$-level optimality of a size $24$ IMSPE-optimal design.}
  \label{Error Analysis Plots}
\end{figure}
Figure \ref{Rel_Error} shows the relative truncation error (\ref{relative_error}) for approximate
IMSPE-optimal designs of multiple sizes, alongside the ``ideal'' relative error (assuming an IMSPE $M$-perfect design exists) given by
\begin{align*}
\widetilde{r}_{_M}(n) =
\begin{cases}
\begin{array}{ccc}
0 & &M \geq n\spc,\\[1em]
\displaystyle\sum_{k=M+1}^{n}\lambda_k\bigg/\displaystyle\sum_{j=1}^n\lambda_j & &M<n\spc.
\end{array}
\end{cases}
\end{align*}

\noindent In Figure \ref{First_Terms} the reader can examine the leading IMSPE terms of a size $24$ IMSPE-optimal design.
Evidently, the first $M=17$ components $\lambda_k\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k$ , $k=1,\ldots,17$,
all equal (or nearly equal) the maximum value of $1$, hence an IMSPE $17$-perfect design practically exists in this case, and the relative truncation error is controlled at
$\epsilon=0.00492$, following the discussion in Section \ref{error} and as Figure
\ref{Rel_Error} clearly shows.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\section{The Relation to Bayesian Linear Regression}\label{bayes-reg}
It is perhaps expected that expression (\ref{approx_IMSPE}) should be
related to the truncated process
\begin{align}\label{regression}
y\left(\boldsymbol{x}\right) = \beta_0 + \sum_{i=1}^M\lambda_i^{1/2}\alpha_i\varphi_i\left(\boldsymbol{x}\right)\spc,\spc \boldsymbol{\alpha}=\left[\alpha_1,\ldots,\alpha_M\right]^{\mathsf{T}}\sim\mathcal{N}_M\left(\boldsymbol{0},\boldsymbol{I}\right)\spc,
\end{align}
that is: the Bayesian linear regression model with no measurement error. The following Proposition shows how closely related the two are.

\begin{proposition}
Let $y\ofx$ be the process (\ref{regression}), and let
\begin{align}\label{truncated_kriging}
\widehat{y}\ofx =
\beta_0+\boldsymbol{\phi}^M\ofx^{\mathsf{T}}\boldsymbol{\Lambda}{\boldsymbol{\Phi}}^{\mathsf{T}}\boldsymbol{\mathcal{R}}^{-1}\left(\boldsymbol{y}-\beta_0\boldsymbol{1}_n\right)\spc,
\end{align}
with $$\boldsymbol{\mathcal{R}} = \boldsymbol{\Phi}\boldsymbol{\Lambda}\boldsymbol{\Phi}^{^{\mathsf{T}}} \spc\text{and}\spc \boldsymbol{\phi^M}\ofx = \left[\varphi_1\ofx,\ldots,\varphi_M\ofx\right]^{\mathsf{T}}\spc,$$
be the kriging estimator based on $n$ observations.  Then
\begin{align}\label{IMSPE_proposition}
\mathcal{J}\left(\mathcal{D},\widehat{y}\right) = \mathrm{tr}\left(\boldsymbol{\Lambda}\right) - \mathrm{tr}\left\{\boldsymbol{\Lambda}^2\boldsymbol{\Phi}^{\mathsf{T}}\boldsymbol{\mathcal{R}}^{-1}\boldsymbol{\Phi}\right\}\spc.
\end{align}
\end{proposition}
\begin{proof}
First, note that $\boldsymbol{y}$ is marginally normal, with $$\boldsymbol{y}\big|\boldsymbol{\alpha}=\beta_0
+ \boldsymbol{\Phi}\boldsymbol{\Lambda}^{1/2}\boldsymbol{\alpha}$$ and
\begin{align*} \var\left(\boldsymbol{y}\right)=\boldsymbol{\Phi}\boldsymbol{\Lambda}^{1/2}\boldsymbol{I}\boldsymbol{\Lambda}^{1/2}\boldsymbol{\Phi}^{\mathsf{T}} = \boldsymbol{\mathcal{R}}\spc.
\end{align*}
The posterior predictive distribution $\pi\left(y\ofx\big|\boldsymbol{y}\right)$ at any $x\in\mathcal{X}$ is
\begin{align*}
\mathcal{N}\left\{\beta_0+\boldsymbol{\phi}^M\ofx^{\mathsf{T}}\boldsymbol{\Lambda}\boldsymbol{\Phi}^{\mathsf{T}}\boldsymbol{\mathcal{R}}^{-1}\left(\boldsymbol{y}-\beta_0\boldsymbol{1}_n\right)\spc,\spc\boldsymbol{\phi}^M\ofx^{\mathsf{T}}\boldsymbol{\Lambda}\left(\boldsymbol{I}-\boldsymbol{\Phi}^{\mathsf{T}}\boldsymbol{\mathcal{R}}^{-1}\boldsymbol{\Phi}\boldsymbol{\Lambda}\right)\boldsymbol{\phi}^M\ofx\right\}\spc,
\end{align*}
so it is natural to choose our predictor to be
\begin{align*}
\widehat{y}\ofx = \mathbb{E}\left\{y\ofx\big|\boldsymbol{y}\right\}
=
\beta_0+\boldsymbol{\phi}^M\ofx^{\mathsf{T}}\boldsymbol{\Lambda}\boldsymbol{\Phi}^{\mathsf{T}}\boldsymbol{\mathcal{R}}^{-1}\left(\boldsymbol{y}-\beta_0\boldsymbol{1}_n\right)\spc.
\end{align*}
Then the mean squared prediction error is given by
\begin{align}\label{MSPE_regression}
\mathbb{E}\left[\left\{y\ofx-\widehat{y}\ofx\right\}^2\bigg|\boldsymbol{y}\right] = \var\left\{y\ofx\big|\boldsymbol{y}\right\} = \boldsymbol{\phi}^M\ofx^{\mathsf{T}}\boldsymbol{\Lambda}\left(\boldsymbol{I}-\boldsymbol{\Phi}^{\mathsf{T}}\boldsymbol{\mathcal{R}}^{-1}\boldsymbol{\Phi}\boldsymbol{\Lambda}\right)\boldsymbol{\phi}^M\ofx\spc.
\end{align}
Now, for any matrix $\boldsymbol{A}_{M\times M} = \left(a_{ij}\right)$ one has
\begin{align}\label{matrix_integral_property}
\int_{\mathcal{X}}\boldsymbol{\phi}^M\ofx^{\mathsf{T}}\boldsymbol{A}\boldsymbol{\phi}^M\ofx\di\boldsymbol{x} = \sum_{i=1}^M\sum_{j=1}^Ma_{ij}\int_{\mathcal{X}}\varphi_i\ofx\varphi_j\ofx\di\boldsymbol{x} = \mathrm{tr}\left(\boldsymbol{A}\right)\spc.
\end{align}
Applying (\ref{matrix_integral_property}) to (\ref{MSPE_regression}) we have
\begin{align*}
\mathcal{J}\left(\mathcal{D},\widehat{y}\right)& = \int_{\mathcal{X}}\boldsymbol{\phi}^M\ofx^{\mathsf{T}}\boldsymbol{\Lambda}\boldsymbol{\phi}^M\ofx\di\boldsymbol{x} -\int_{\mathcal{X}}\boldsymbol{\phi}^M\ofx^{\mathsf{T}}\boldsymbol{\Lambda}\boldsymbol{\Phi}^{\mathsf{T}}\boldsymbol{\mathcal{R}}^{-1}\boldsymbol{\Phi}\boldsymbol{\Lambda}\boldsymbol{\phi}^M\ofx\di\boldsymbol{x} =\\[1em]
&= \mathrm{tr}\left(\boldsymbol{\Lambda}\right) - \mathrm{tr}\left\{\boldsymbol{\Lambda}^2\boldsymbol{\Phi}^{\mathsf{T}}\boldsymbol{\mathcal{R}}^{-1}\boldsymbol{\Phi}\right\}\spc.
\end{align*}
\qed
\end{proof}

\begin{rembold}
\fontfamily{phv}\selectfont{
The Gram matrix $\boldsymbol{R}$ has elements
\begin{align*}
R_{ij} = R\left(\boldsymbol{x}_i,\boldsymbol{x}_j\right) = \sum_{k=1}^{\infty}\lambda_k\varphi_k\left(\boldsymbol{x}_i\right)\varphi_k\left(\boldsymbol{x}_j\right)\spc.
\end{align*}
We may thus think of $\boldsymbol{\mathcal{R}}$ as an approximation of $\boldsymbol{R}$. Similarly, the predictor (\ref{truncated_kriging}) is merely a truncated version of the usual Kriging predictor (\ref{kriging}).
}
\end{rembold}

\begin{rembold}
\fontfamily{phv}\selectfont{
For any correlation function of a stationary process $R\left(\boldsymbol{x},\boldsymbol{y}\right) = R\left(\boldsymbol{x}-\boldsymbol{y}\right)$ and compact $\mathcal{X}\in\mathbb{R}^d$,
\begin{align*}
\sum_{i=1}^{\infty}\lambda_i =
\int_{\mathcal{X}}R\left(\boldsymbol{x},\boldsymbol{x}\right)\di\boldsymbol{x}
= R\left(\boldsymbol{0}\right)\int_{\mathcal{X}}\di\boldsymbol{x}
= \mathrm{vol}\left(\mathcal{X}\right)\spc.
\end{align*}
Thus, if we choose large enough $M$, expressions
(\ref{IMSPE_proposition}) and (\ref{approx_IMSPE}) become arbitrarily
close.
}
\end{rembold}
\end{comment}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{Batch Sequential Designs}\label{batch}
Suppose now that we have the privilege of selecting $n_2$ additional
inputs, having already run the experiment on the original design of
size $n_1$ and re-estimated the model's unknown parameters. The
topic of batch sequential designs for computer experiments has been
discussed by \cite{Batch} amongst others.\\

\noindent Using the same notation as in Section \ref{IMSE_Intro}, we can now write
\begin{align*}
\renewcommand{\arraystretch}{1.4}
\text{
{\large
$
\boldsymbol{R}_{\text{aug}} =
\left[
\begin{array}{c|c}
\boldsymbol{R}^{\text{new}}_{\text{$n_2\times n_2$}} &\boldsymbol{R}^{\text{cross}}_{\text{$n_2\times n_1$}}\\
\hline
\boldsymbol{R}^{^\top\text{cross}}_{\text{$n_1\times n_2$}} &\boldsymbol{R}^{\text{old}}_{\text{$n_1\times n_1$}}\\
\end{array}
\right]
$ ,
}
}
\end{align*}
where $\boldsymbol{R}_{\text{aug}}$, $\boldsymbol{R}^{\text{new}}$, $\boldsymbol{R}^{\text{old}}$ and $\boldsymbol{R}^{\text{cross}}$ are the augmented correlation matrix, the matrix of correlations within the new inputs, the matrix of correlations within the original design and the cross correlation matrix. Similarly
\begin{align*}
\renewcommand{\arraystretch}{1.4}
\text{
{\large
$
\boldsymbol{\Phi}_{\text{aug}} =
\left[
\begin{array}{c}
\boldsymbol{\Phi}^{\text{new}}_{\text{$n_2\times M$}} \\
\hline
\boldsymbol{\Phi}^{\text{old}}_{\text{$n_1\times M$}}\\
\end{array}
\right]
$ ,
}
}
\end{align*}
and, using basic block matrix identities, we can write
\begin{align}\label{batch_seq_decomp}
&\mathrm{tr}\left\{\boldsymbol{\Lambda}^2\boldsymbol{\Phi}_{\text{aug}}^{\mathsf{T}}\boldsymbol{R}_{\text{aug}}^{-1}\boldsymbol{\Phi}_{\text{aug}}\right\} \\[1em]
& = \mathrm{tr}\bigg[\boldsymbol{\Lambda}^2\left\{\left(\boldsymbol{\Phi}_{_{\text{new}}}^{\mathsf{T}}-\boldsymbol{\Phi}_{_{\text{old}}}^{\mathsf{T}}\boldsymbol{R}_{_{\text{old}}}^{-1}\boldsymbol{R}_{_{\text{cross}}}^{\mathsf{T}}\right)\boldsymbol{Q}_1^{-1}\boldsymbol{\Phi}_{_{\text{new}}} + \left(\boldsymbol{\Phi}_{_{\text{old}}}^{\mathsf{T}}-\boldsymbol{\Phi}_{_{\text{new}}}^{\mathsf{T}}\boldsymbol{R}_{_{\text{new}}}^{-1}\boldsymbol{R}_{_{\text{cross}}}\right)\boldsymbol{Q}_2^{-1}\boldsymbol{\Phi}_{_{\text{old}}}\right\}\bigg]\spc,
\end{align}
where
\begin{align*}
\boldsymbol{Q}_1 = \boldsymbol{R}_{\text{new}} - \boldsymbol{R}_{\text{cross}}^{\mathsf{T}}\boldsymbol{R}_{\text{old}}^{-1}\boldsymbol{R}_{\text{cross}}\spc \spc\text{and}\spc \spc\boldsymbol{Q}_2 = \boldsymbol{R}_{\text{old}} - \boldsymbol{R}_{\text{cross}}\boldsymbol{R}_{\text{new}}^{-1}\boldsymbol{R}_{\text{cross}}^{\mathsf{T}}\spc.
\end{align*}
Note that $\boldsymbol{R}_{\text{old}}$ and $\boldsymbol{\Phi}_{\text{old}}$ are at this stage fixed matrices that need not be updated. When the second batch grows large, expression (\ref{batch_seq_decomp}) could prove to be handy, as it requires the inversion of smaller matrices than $\boldsymbol{R}_{\text{aug}}$ .\\

\noindent Figure \ref{Batch_Seq} shows examples of batch-sequential approximate minimum IMSPE designs, using the same correlation function as before.
\begin{figure}[ht!]
\centering
\subfloat[][]{\label{Batch_Seq_No_Nugget}\includegraphics[width=.5\textwidth]{IMSPE_Design_8_4_Points.pdf}}
\subfloat[][]{\label{Batch_Seq_Nugget}\includegraphics[width=0.5\textwidth]{BatchSeq8_7_after.pdf}}
\caption{Batch sequential approximate IMSPE-optimal designs. Figure \ref{Batch_Seq_No_Nugget}: size $8+4$ design.
Figure \ref{Batch_Seq_Nugget}: size $8+7$ design with nugget parameter $\lambda=0.1$.}
\label{Batch_Seq}
\end{figure}


\begin{rembold}
\fontfamily{phv}\selectfont{
So far we have ignored the possibility of measurement error, as no such
error exists in deterministic computer experiments.
Adding an error term, as in \cite{nugget}, would mean extending (\ref{gauss_proc}) to
\begin{align}\label{eq:nugget}
y\ofx = \beta_0 + Z\ofx + \varepsilon\ofx\spc,
\end{align}
where
$\varepsilon\left(\boldsymbol{x}_i\right)\sim\mathcal{N}\left(\boldsymbol{0},\tau^2\right)$
. Denoting $\lambda = \tau^2/\sigma^2$, it is easy to show that the
best linear unbiased predictor is now
\begin{align*}
\widehat{y}\ofx = \mathbb{E}\left\{y(\boldsymbol{x})\big|\boldsymbol{y}\right\} = \beta_0 + \boldsymbol{r}^{\mathsf{T}}(\boldsymbol{x})\left(\boldsymbol{R}+\lambda\boldsymbol{I}\right)^{-1}\left(\boldsymbol{y}-\beta_0\boldsymbol{1}_n\right)\spc,
\end{align*}
and the mean squared prediction error is
\begin{align*}
\mathbb{E}\left[\big\{\widehat{y}(\boldsymbol{x})-y(\boldsymbol{x})\big\}^2\Big|\boldsymbol{y}\right]
= \var\left\{y(\boldsymbol{x})\big|\boldsymbol{y}\right\}
=
\sigma^2\left\{1+\lambda-\boldsymbol{r}^{\mathsf{T}}(\boldsymbol{x})\left(\boldsymbol{R}+\lambda\boldsymbol{I}\right)^{-1}\boldsymbol{r}(\boldsymbol{x})\right\}\spc.
\end{align*}
The IMSPE becomes
\begin{align*}
\mathcal{J}\left(\mathcal{D},\widehat{y}\right)={\sigma^2}\left\{\left(1+\lambda\right)\mathrm{vol}(\mathcal{X}) - \sum_{k=1}^{\infty}\lambda_k^2\boldsymbol{\phi}_k^{\mathsf{T}}\left(\boldsymbol{R}+\lambda\boldsymbol{I}\right)^{-1}\boldsymbol{\phi}_k\right\}
\end{align*}
and, employing the truncated process, a corresponding approximate minimum mean squared prediction error design will now be
\begin{align}\label{eq:batchseq}
\mathcal{D}^{*} = \displaystyle\argmax_{\mathcal{D}\subset\mathcal{X}}\mathrm{tr}\left\{\boldsymbol{\Lambda}^2\boldsymbol{\Phi}^{\mathsf{T}}\left(\boldsymbol{R}+\lambda\boldsymbol{I}\right)^{-1}\boldsymbol{\Phi}\right\}\spc.
\end{align}
Adding the error term, also called the nugget term, is often
beneficial from the computational point of view, as the correlation
matrix $\boldsymbol{R}$ tends to become numerically singular as the
number of input vectors becomes large relative to the dimension of
the input space. Examples showing solutions of (\ref{eq:batchseq}) appear in Figure \ref{Batch_Seq_Nugget}, as well as in Figure \ref{11_pts_Nugget}.
}

\begin{figure}
  \centering
 \includegraphics[width=0.6\textwidth]{Design_Nugget.pdf}
  \caption{Size $11$ design, with and without the nugget term.}
  \label{11_pts_Nugget}
\end{figure}
\end{rembold}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Extending to Models with Unknown Intercept}\label{unknown_inter}
When the constant $\beta_0$ is unknown, it is common practice to
assign it an improper prior $\pi\left(\beta_0\right)\propto 1$. It
can be shown (see \citealt[chapter~4]{santner}) that now
\begin{align*}
\widehat{y}\ofx = \mathbb{E}\left\{y\ofx\big|\boldsymbol{y}\right\} = \widehat{\beta}_0 + \boldsymbol{r}^{\mathsf{T}}\ofx\boldsymbol{R}^{-1}\left(\boldsymbol{y}-\widehat{\beta}_0\boldsymbol{1}_n\right)
\end{align*}
for
\begin{align*}
\widehat{\beta}_0 = \mathbb{E}\left(\beta_0\big|\boldsymbol{y}\right) = \dfrac{\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{y}}{\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n}\spc,
\end{align*}
and the mean squared prediction error is
\begin{align}\label{MSE_Expression_2}
\mathbb{E}\left[\big\{\widehat{y}(\boldsymbol{x})-y(\boldsymbol{x})\big\}^2\Big|\boldsymbol{y}\right]
=
\sigma^2\left[1-\boldsymbol{r}^{\mathsf{T}}(\boldsymbol{x})\boldsymbol{R}^{-1}\boldsymbol{r}(\boldsymbol{x})+\frac{\left\{1-\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{r}(\boldsymbol{x})\right\}^2}{\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n}\right]\spc.
\end{align}
The additional uncertainty with respect to $\beta_0$ is expressed in
the third term in (\ref{MSE_Expression_2}).

\noindent Calculations of a similar nature to (\ref{IMSE2}) yield
\begin{align}\label{advanced1}
\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{r}(\boldsymbol{x}) = \sum_{k=1}^{\infty}\left(\lambda_k\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k\right)\varphi_k(\boldsymbol{x})
\end{align}
and
\begin{align}\label{advanced2}
\left\{\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{r}(\boldsymbol{x})\right\}^2
=
\sum_{k=1}^{\infty}\sum_{l=1}^{\infty}\left(\lambda_k\lambda_l\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_l\right)\varphi_k(\boldsymbol{x})\varphi_l(\boldsymbol{x})\spc.
\end{align}
If we now denote the IMSPE of the predictor $\widehat{y}\ofx$ at $\mathcal{D}$ by $\mathcal{H}\left(\mathcal{D},\widehat{y}\right)$, then,
plugging (\ref{advanced1}) and (\ref{advanced2}) into
(\ref{MSE_Expression_2}) and integrating over the experimental region
yields

\begin{align}\label{IMSPE_advanced}
\mathcal{H}\left(\mathcal{D},\widehat{y}\right) = \mathcal{J}\left(\mathcal{D},\widehat{y}\right)
&+\frac{1}{\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n}\bigg\{\mathrm{vol}\left(\mathcal{X}\right) - 2\sum_{k=1}^{\infty}\left(\lambda_k\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k\right)\int_{\mathcal{X}}\varphi_k(\boldsymbol{x})\di \boldsymbol{x}\nonumber\\[1em] &+ \sum_{k=1}^{\infty}\lambda_k^2\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k\bigg\}
\end{align}
where $\mathcal{J}\left(\mathcal{D},\widehat{y}\right)$ is (\ref{IMSE3}).
Using previous notations, we can approximate (\ref{IMSPE_advanced}) by the truncated criterion
\begin{align}\label{approx_IMSPE_advanced}
\widetilde{\mathcal{H}}_{_M}\left(\mathcal{D},\widehat{y}\right) = \widetilde{\mathcal{J}}_{_M}\left(\mathcal{D},\widehat{y}\right) +
\frac{1}{\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n}
\left\{
\mathrm{vol}\left(\mathcal{X}\right) - 2\boldsymbol{a}^{\mathsf{T}}\boldsymbol{\gamma} + \boldsymbol{a}^{\mathsf{T}}\boldsymbol{a}
\right\}\spc,
\end{align}
where
\begin{align*}
\boldsymbol{a} = \boldsymbol{\Lambda}\boldsymbol{\Phi}^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n\spc ,\spc \boldsymbol{\gamma} = \left[\int_{\mathcal{X}}\boldsymbol{\phi}_1(\boldsymbol{x})\di\boldsymbol{x},\ldots,\int_{\mathcal{X}}\boldsymbol{\phi}_M(\boldsymbol{x})\di\boldsymbol{x}\right]^{\mathsf{T}}\spc \text{and} \spc \widetilde{\mathcal{J}}_{_M}\left(\mathcal{D},\widehat{y}\right)\spc \text{is}\spc (\ref{approx_IMSPE}).
\end{align*}
The vector of integrals $\boldsymbol{\gamma}$ only needs to be
evaluated once, and is particularly simple to calculate numerically
in the separable case, where the problem reduces to one dimensional
integrals.

\begin{rembold}%[fontfamily=helvetica]
\fontfamily{phv}\selectfont{
The last result can be generalized to the universal Kriging model (\ref{univer_krig}) by
\begin{align*}
\widetilde{\mathcal{H}}_{_M}\left(\mathcal{D},\widehat{y}\right) =& \widetilde{\mathcal{J}}_{_M}\left(\mathcal{D},\widehat{y}\right) \\[1em]
+&\mathrm{tr}\left\{
\left(\boldsymbol{F}^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{F}\right)^{-1}
\left[
\int_{\mathcal{X}}\boldsymbol{f}\ofx\boldsymbol{f}^{\mathsf{T}}\ofx\di\boldsymbol{x}
-2\boldsymbol{A}^{\mathsf{T}}\int_{\mathcal{X}}\boldsymbol{\phi}\ofx\boldsymbol{f}^{\mathsf{T}}\ofx\di\boldsymbol{x}
+ \boldsymbol{A}^{\mathsf{T}}\boldsymbol{A}
\right]
\right\}\spc,
\end{align*}
where
$\boldsymbol{A} = \boldsymbol{\Lambda}\boldsymbol{\Phi}^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{F}$\spc and\spc $\boldsymbol{\phi}\ofx = \left[\varphi_1\ofx,\ldots,\varphi_M\ofx\right]^{\mathsf{T}}$ .
}
\end{rembold}

\noindent In Table \ref{tab:IMSPE_comp} we compare the approximate integrated
mean squared prediction error (as calculated in
(\ref{approx_IMSPE_advanced})) of the optimal designs obtained under
the assumption that $\beta_0$ was known, with the minimizers of
(\ref{approx_IMSPE_advanced}). Figure \ref{Both_14_pts_IMSPE_Designs}
compares the two criteria for a $14-$run design optimized for
the correlation function (\ref{gaussian_cor}).


\begin{table}[ht!]
\caption{Approximate IMSPE for different design sizes}
\centering
{\small
\begin{tabular}{c c c c}
\midrule
\midrule
Design Size &$\begin{array}{c}\text{Approx. IMSPE}\\ \text{(known $\beta_0$)}\end{array}$ &$\begin{array}{c}\text{Approx. IMSPE}\\ \text{(unknown $\beta_0$)}\end{array}$ &$\Delta$\\
\midrule
\midrule
$8$ &$0.33925$ &$0.33882$ &$4.24\times10^{-4}$\\
\midrule
$10$ &$0.18665$ &$0.18644$ &$2.17\times10^{-4}$\\
\midrule
$12$ &$0.10669$ &$0.10662$ &$6.76\times10^{-5}$\\
\midrule
$14$ &$0.06551$ &$0.06548$ &$3.03\times10^{-5}$\\
\midrule
$20$ &$0.02110$ &$0.02110$ &$9.10\times10^{-7}$\\
\midrule
\end{tabular}
}
\label{tab:IMSPE_comp}
\end{table}


\noindent Figure \ref{Criteria_Difference} shows exactly how fast
the designs based on criteria (\ref{approx_IMSPE}) and
(\ref{approx_IMSPE_advanced}) become virtually indistinguishable.

\begin{figure}[ht!]
\centering
    \includegraphics[width=.8\textwidth]{With_and_without_intercept.pdf}
    \caption{Optimal designs with $5$ and $14$ runs according to (\ref{approx_IMSPE}) and (\ref{approx_IMSPE_advanced}). The design for the known intercept model (\ref{approx_IMSPE}) consists of the solid points.}
  \label{Both_14_pts_IMSPE_Designs}
\end{figure}

\begin{figure}[ht!]
\centering
\includegraphics[width=.6\textwidth]{Criteria_Difference.pdf}
\caption{The gap from the optimum ($\Delta$) of (\ref{approx_IMSPE_advanced}) for designs based on (\ref{approx_IMSPE}), by sample size.}
  \label{Criteria_Difference}
\end{figure}




\section{Bayesian A-optimal Designs}\label{A-opt}
For the simple model (\ref{gauss_proc})
\begin{align}\label{simple_cov}
\var\left\{y(\boldsymbol{x})\big|\boldsymbol{y}\right\} &=
\mathrm{cov}\left(\beta_0 + \sum_{k=1}^{\infty}\alpha_k\varphi_k(\boldsymbol{x})\hspace{.15em},\hspace{.15em}\beta_0+\sum_{l=1}^{\infty}\alpha_l\varphi_l(\boldsymbol{x})\bigg|\boldsymbol{y}\right)\nonumber\\[1em] &=\sum_{k=1}^{\infty}\sum_{l=1}^{\infty}\mathrm{cov}\left(\alpha_k,\alpha_l\big|\boldsymbol{y}\right)\varphi_k(\boldsymbol{x})\varphi_l(\boldsymbol{x})\spc,
\end{align}
where the $\alpha_i$'s are independent $\mathcal{N}(0,\lambda_i)$ random variables, as in (\ref{model}). From (\ref{simple_cov}) and the orthonormality of $\left\{\varphi_i\ofx\right\}$,
\begin{align}\label{simple_A-opt}
\mathcal{J}\left(\mathcal{D},\widehat{y}\right) &= \int_\mathcal{X}\var\left\{y(\boldsymbol{x})\big|\boldsymbol{y}\right\}\di\boldsymbol{x} =
\sum_{k=1}^{\infty}\sum_{l=1}^{\infty}\mathrm{cov}\left(\alpha_k,\alpha_l\big|\boldsymbol{y}\right)\int_\mathcal{X}\varphi_k(\boldsymbol{x})\varphi_l(\boldsymbol{x})\di\boldsymbol{x}\nonumber\\[1em] &= \sum_{k=1}^{\infty}\var\left\{\alpha_i\big|\boldsymbol{y}\right\}\spc.
\end{align}
Experimental designs whose purpose is to minimize the total variance of the estimators for the model's parameters are known as A-optimal designs (see \citet[chapter~10]{OptimalDesigns} for example). We learn from (\ref{simple_A-opt}) that in the simple case in which the constant $\beta_0$ is assumed to be known, IMSPE-optimal designs are in fact Bayesian A-optimal designs for the multipliers of the eigenfunctions. Bayesian optimal designs for the linear regression model have been discussed in the works of \cite{Studden}, and within a decision-theoretic framework in \cite{BayesOptimalDesigns}.\\

\noindent Suppose now that $\beta_0\sim\mathcal{N}(0,\tau^2)$. For $k \geq 1$ ,
\begin{align*}
\left[
\begin{array}{c}
\alpha_k\\
\boldsymbol{y}
\end{array}
\right]
\sim
\mathcal{N}\left\{\boldsymbol{0}\spc,\spc
\left[
\begin{array}{cc}
\lambda_k &\lambda_k\boldsymbol{\phi}_k^{\mathsf{T}}\\[1em]
\lambda_k\boldsymbol{\phi}_k &\boldsymbol{R}+\tau^2\boldsymbol{1}_n\boldsymbol{1}_n^{\mathsf{T}}
\end{array}
\right]
\right\}\spc,
\end{align*}
therefore
\begin{align}\label{post_var_alpha_1}
\var\left\{\alpha_k\big|\boldsymbol{y}\right\} &= \lambda_k - \lambda_k^2\boldsymbol{\phi}_k^{\mathsf{T}}\left[\boldsymbol{R}+\tau^2\boldsymbol{1}_n\boldsymbol{1}_n^{\mathsf{T}}\right]^{-1}\boldsymbol{\phi}_k \notag\\[1em] &= \lambda_k - \lambda_k^2\boldsymbol{\phi}_k^{\mathsf{T}}\left[\boldsymbol{R}^{-1} - \dfrac{1}{1/\tau^2 + \boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n}\cdot\boldsymbol{R}^{-1}\boldsymbol{1}_n\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\right]\boldsymbol{\phi}_k\spc.
\end{align}
A vague prior $\pi(\beta_0)\propto 1$ can be assigned by taking
limits as $\tau\rightarrow\infty$ in (\ref{post_var_alpha_1}), which
leads to
\begin{align}\label{post_var_alpha_2}
\var\left\{\alpha_k\big|\boldsymbol{y}\right\} = \lambda_k - \lambda_k^2\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\left[\boldsymbol{I}-\frac{1}{\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n}\cdot\boldsymbol{1}_n\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\right]\boldsymbol{\phi}_k\spc.
\end{align}
From (\ref{eq:trace_class}), and inspired by (\ref{simple_A-opt}), we may define a modified A-optimality criterion by
\begin{align*}
\mathcal{Q}\left(\mathcal{D},\widehat{y}\right) = \sum_{k=1}^{\infty}\var\left\{\alpha_i\big|\boldsymbol{y}\right\} = \mathcal{J}\left(\mathcal{D},\widehat{y}\right) + \frac{1}{\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n}\sum_{k=1}^{\infty}\lambda_k^2\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k\spc,
\end{align*}
and a truncated version would be
\begin{align}\label{approx_A_opt}
\widetilde{\mathcal{Q}}_{_M}\left(\mathcal{D},\widehat{y}\right) = \widetilde{\mathcal{J}}_{_M}\left(\mathcal{D},\widehat{y}\right) +
\frac{\boldsymbol{a}^{\mathsf{T}}\boldsymbol{a}}{\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n}\spc,
\end{align}
using the notations of Section \ref{unknown_inter}. Despite the similarity of (\ref{approx_IMSPE_advanced}) and (\ref{approx_A_opt}), the two criteria produce fundamentally different designs, as evident in Figure \ref{A_vs_IMSPE}.

\begin{figure}[ht]
\centering
\includegraphics[width=.8\textwidth]{A_vs_IMSPE.pdf}
\caption{Comparison of size $18$ IMSPE-optimal and A-optimal designs, using $\lambda = 0.1$ nugget parameter (using $M=11$ terms).}
  \label{A_vs_IMSPE}
\end{figure}

\noindent Exact Bayesian A-optimal
designs are motivated by the eigenfunction representation of the process.  However,
they can be generated indirectly, avoiding the K-L decomposition, as stated in the following Proposition.

\begin{proposition}
\begin{align}\label{exact_A-opt_1}
\mathcal{Q}\left(\mathcal{D},\widehat{y}\right) = \mathrm{vol}\left(\mathcal{X}\right)-
\mathrm{tr}
\left\{
\left[
\begin{array}{ccc}
0 & &\boldsymbol{1}_n^{\mathsf{T}}\\[.5em]
\boldsymbol{1}_n & &\boldsymbol{R}
\end{array}
\right]^{-1}\int_{\mathcal{X}}
\left[
\begin{array}{ccc}
0 & &\boldsymbol{0}_n^{\mathsf{T}}\\[.5em]
\boldsymbol{0}_n & &\boldsymbol{r}\ofx\boldsymbol{r}^{\mathsf{T}}\ofx
\end{array}
\right]
\di \boldsymbol{x}
\right\}\spc.
\end{align}
\end{proposition}
\begin{proof}
By (\ref{IMSE3}) and (\ref{advanced2}),
\begin{align*}
\mathcal{Q}\left(\mathcal{D},\widehat{y}\right) &= \mathcal{J}_0\left(\mathcal{D},\widehat{y}\right) + \frac{1}{\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n}\sum_{k=1}^{\infty}\lambda_k^2\boldsymbol{\phi}_k^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{\phi}_k\\[1em]
&= \int_\mathcal{X}\left[1-\boldsymbol{r}^{\mathsf{T}}(\boldsymbol{x})\boldsymbol{R}^{-1}\boldsymbol{r}(\boldsymbol{x})+\frac{\left\{\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{r}(\boldsymbol{x})\right\}^2}{\boldsymbol{1}_n^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{1}_n}\right]\di\boldsymbol{x}\\[1em]
&= \mathrm{vol}\left(\mathcal{X}\right) - \int_\mathcal{X}\left\{\left[0\hspace{.7em}\boldsymbol{r}^{\mathsf{T}}\ofx\right]
\left[
\begin{array}{ccc}
0 & &\boldsymbol{1}_n^{\mathsf{T}}\\[.5em]
\boldsymbol{1}_n & &\boldsymbol{R}
\end{array}
\right]^{-1}
\left[
\begin{array}{c}
0\\[.1em]
\boldsymbol{r}\ofx
\end{array}
\right]\right\}\di\boldsymbol{x}\\[1em]
& = \mathrm{vol}\left(\mathcal{X}\right)-
\mathrm{tr}
\left\{
\left[
\begin{array}{ccc}
0 & &\boldsymbol{1}_n^{\mathsf{T}}\\[.5em]
\boldsymbol{1}_n & &\boldsymbol{R}
\end{array}
\right]^{-1}\int_{\mathcal{X}}
\left[
\begin{array}{ccc}
0 & &\boldsymbol{0}_n^{\mathsf{T}}\\[.5em]
\boldsymbol{0}_n & &\boldsymbol{r}\ofx\boldsymbol{r}^{\mathsf{T}}\ofx
\end{array}
\right]
\di \boldsymbol{x}
\right\}\spc.
\end{align*}
\end{proof}

\begin{rembold}
\fontfamily{phv}\selectfont{
Criterion (\ref{exact_A-opt_1}) can be easily generalized to
\begin{align}\label{exact_A-opt_2}
\mathcal{J}^{A}\left(\mathcal{D},\widehat{y}\right) = \mathrm{vol}\left(\mathcal{X}\right)-
\mathrm{tr}
\left\{
\left[
\begin{array}{ccc}
\boldsymbol{0} & &\boldsymbol{F}^{\mathsf{T}}\\[.5em]
\boldsymbol{F} & &\boldsymbol{R}
\end{array}
\right]^{-1}\int_{\mathcal{X}}
\left[
\begin{array}{ccc}
\boldsymbol{0} & &\boldsymbol{0}\\[.5em]
\boldsymbol{0} & &\boldsymbol{r}\ofx\boldsymbol{r}^{\mathsf{T}}\ofx
\end{array}
\right]
\di \boldsymbol{x}
\right\}
\end{align}
for the universal Kriging model (\ref{univer_krig}). Note the striking resemblance of criteria (\ref{exact_A-opt_2}) and (\ref{IMSPE_original}).
Interestingly, the indifference of the A-criterion to the terms related to the posterior covariances between the $\alpha_k$'s and $\beta_0$ (as well as the posterior variance of $\beta_0$) reflects in the $\boldsymbol{0}$-blocks on the secondary diagonal of the integrand in (\ref{exact_A-opt_2}).
}
\end{rembold}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Bayesian D-optimal Designs}\label{D-opt}
Having already exploited the Karhunen-Lo\`eve decomposition of the
Gaussian process $Z\ofx$ to generate IMSPE-optimal and Bayesian A-optimal
designs, other `alphabetical' optimal designs may be considered. For example,
assuming model (\ref{univer_krig}) with $\boldsymbol{\beta}\sim\mathcal{N}\left(\boldsymbol{0},\tau^2\boldsymbol{I}\right)$, we have
\begin{align*}
\left[
\alpha_1\hspace{.15em}
\cdots\hspace{.15em}
\alpha_M\hspace{.15em}
\boldsymbol{y}
\right]^{\mathsf{T}}
\sim
\mathcal{N}\left\{\boldsymbol{0}\spc,\spc
\left[
\begin{array}{cc}
\boldsymbol{\Lambda} &\boldsymbol{\Phi}\boldsymbol{\Lambda}\\[1em]
\boldsymbol{\Lambda}\boldsymbol{\Phi}^{\mathsf{T}} &\boldsymbol{R}+\tau^2\boldsymbol{F}\boldsymbol{F}^{\mathsf{T}}
\end{array}
\right]
\right\}\spc,
\end{align*}
and using similar techniques
to the one used to derive (\ref{post_var_alpha_2}), by assigning
a vague prior $\pi\left(\boldsymbol{\beta}\right)\propto1$ (i.e. by taking the limit as $\tau\to\infty$), the posterior covariance
matrix of the first $M$ coefficients in (\ref{model}) is given by
\begin{align}\label{covar_Matrix}
\Sigma_M=\var\left\{\alpha_1,\ldots,\alpha_M\big|\boldsymbol{y}\right\}=\boldsymbol{\Lambda}-\boldsymbol{\Lambda}\boldsymbol{\Phi}^{\mathsf{T}}\left[\boldsymbol{R}^{-1}-\boldsymbol{R}^{-1}\boldsymbol{F}\left(\boldsymbol{F}^{\mathsf{T}}\boldsymbol{R}^{-1}\boldsymbol{F}\right)^{-1}\boldsymbol{F}^{\mathsf{T}}\boldsymbol{R}^{-1}\right]\boldsymbol{\Phi}\boldsymbol{\Lambda}\spc.
\end{align}
An approximate Bayesian D-optimal design for the model (\ref{univer_krig}) would then be
\begin{align*}
\mathcal{D}^* = \displaystyle\argmin_{\mathcal{D}}\det\left(\Sigma_M\right)\spc.
\end{align*}
Figure \ref{all_3} shows size $8$ A, D and IMSPE-optimal designs, using $\lambda=0.1$ for the nugget term and $M=11$ terms.

\begin{figure}[ht]
\centering
\includegraphics[width=1\textwidth]{All_3.pdf}
\caption{Different optimal designs for the Gaussian process model.}
  \label{all_3}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Comparison of Several Designs}\label{sec:comparison}
We would now like to compare the performance of the designs discussed in this chapter by
their respective criteria. Designs of several sizes were generated for the ordinary Kriging model with measurement error
(and unknown intercept) (\ref{eq:nugget}), assuming the nugget parameter is $\lambda=0.1$ and the correlation function is (\ref{gaussian_cor}). For reference, we add maximin Latin hypercube designs (see \citealt[chapter~5]{santner}), the most popular experimental designs in the field of computer experiments. The results are shown in Table \ref{tab:comparison}.

\begin{table}[ht!]
\caption{Design comparison for several sample sizes and optimality criteria.}
\label{tab:comparison}
\centering
\begin{threeparttable}
{\footnotesize
\begin{tabular}{cp{1.5cm}|.|.|.|.|}
\cline{3-6}
& & \multicolumn{4}{ c| }{Design}\\
\hline
\multicolumn{1}{|c|}{Size} &\multicolumn{1}{c|}{Criterion} &\multicolumn{1}{c|}{IMSPE-optimal} &\multicolumn{1}{c|}{A-optimal} &\multicolumn{1}{c|}{D-optimal} &\multicolumn{1}{c|}{Maximin LHD}\\
\hline
%\multicolumn{1}{|c|}{\multirow{3}{*}{$10$}}
%&\multicolumn{1}{c|}{IMSPE} &0.990 &1.027  &1.142 &1.021 \\
%\cline{2-6}
%\multicolumn{1}{|c}{}
%&\multicolumn{1}{|c|}{  A  } &1.498 &1.465  &1.542 &1.506 \\
%\cline{2-6}
%\multicolumn{1}{|c}{}
%&\multicolumn{1}{|c|}{  D  } &-94.809 &-95.107 &-95.547 &-95.005 \\
%\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{$15$}}
&\multicolumn{1}{c|}{IMSPE}&0.813 &0.840  &0.850 &0.857 \\
\cline{2-6}
\multicolumn{1}{|c}{}
&\multicolumn{1}{|c|}{  A  }&1.219 &1.152  &1.196 &1.289 \\
\cline{2-6}
\multicolumn{1}{|c}{}
&\multicolumn{1}{|c|}{  D  }&-97.745 &-98.457  &-98.559 &-97.151 \\
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{$20$}}
&\multicolumn{1}{c|}{IMSPE} &0.737 &0.739  &0.754 &0.756 \\
\cline{2-6}
\multicolumn{1}{|c}{}
&\multicolumn{1}{|c|}{  A  }&1.103 &1.045  &1.085 &1.177 \\
\cline{2-6}
\multicolumn{1}{|c}{}
&\multicolumn{1}{|c|}{  D  }&-99.844 &-100.372  &-100.865 &-98.893 \\
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{$25$}}
&\multicolumn{1}{c|}{IMSPE} &0.690 &0.694  &0.699 &0.714 \\
\cline{2-6}
\multicolumn{1}{|c}{}
&\multicolumn{1}{|c|}{  A  }&1.027 &0.995  &1.025 &1.125 \\
\cline{2-6}
\multicolumn{1}{|c}{}
&\multicolumn{1}{|c|}{  D  }&-101.507 &-101.585  &-102.177 &-100.100 \\
\hline
\end{tabular}
    \begin{tablenotes}
      \footnotesize
      \item D criterion here is $\log_{10}\left|\Sigma_M\right|$ for $M=37$.
    \end{tablenotes}
}
\end{threeparttable}
\end{table}

\noindent Clearly, the reader would be mostly interested in the lines of Table \ref{tab:comparison} refering to the IMSPE criterion.
Indeed, the IMSPE-optimal designs show a steady improvement of $3\%-5\%$ over the maximin LHD designs. However, the reader
should keep in mind that the maximin LHD designs were generated independently of the model assumptions and the model parameters in particular.\\

\noindent Another, perhaps more interesting comparison is presented in Table \ref{tab:comparison2}, where the same size $20$ designs from Table \ref{tab:comparison}, designated specifically for correlation parameters $\boldsymbol{\theta} = (1,2)$, are compared to the Maximin LHD design, this time for correlation parameters different from the true ones. The choice of $n=20$ is based on a rule of thumb generally accepted in the computer experiments community which states that the recommended sample size for $\mathcal{X}\subset\mathbb{R}^d$ is $10d$. See \cite{Welch} for details. It is interesting to note that the different criteria show reasonable robustness with respect to the actual parameters.

\begin{table}[ht!]
\caption{Robustness study for the efficiency of the optimal designs with respect to the correlation parameters $\boldsymbol{\theta}$. All designs are of size $n=20$.}
\label{tab:comparison2}
\centering
\begin{threeparttable}
{\footnotesize
\begin{tabular}{>{\centering}p{1cm}>{\centering}p{2cm}|.|.|.|.|}
\cline{3-6}
& & \multicolumn{4}{ c| }{Design}\\
\hline
\multicolumn{1}{|c|}{$\boldsymbol{\theta}$} &\multicolumn{1}{c|}{Criterion} &\multicolumn{1}{c|}{IMSPE-optimal} &\multicolumn{1}{c|}{A-optimal} &\multicolumn{1}{c|}{D-optimal} &\multicolumn{1}{c|}{Maximin LHD}\\
\hline
%\multicolumn{1}{|c|}{\multirow{3}{*}{$10$}}
%&\multicolumn{1}{c|}{IMSPE} &0.990 &1.027  &1.142 &1.021 \\
%\cline{2-6}
%\multicolumn{1}{|c}{}
%&\multicolumn{1}{|c|}{  A  } &1.498 &1.465  &1.542 &1.506 \\
%\cline{2-6}
%\multicolumn{1}{|c}{}
%&\multicolumn{1}{|c|}{  D  } &-94.809 &-95.107 &-95.547 &-95.005 \\
%\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{(1,1)}}
&\multicolumn{1}{c|}{IMSPE}&0.704 &0.703  &0.714 &0.726 \\
\cline{2-6}
\multicolumn{1}{|c}{}
&\multicolumn{1}{|c|}{A}&1.241 &1.178  & 1.217 &1.345 \\
\cline{2-6}
\multicolumn{1}{|c}{}
&\multicolumn{1}{|c|}{  D  }&-81.128 &-81.596  &-81.952 &-80.224 \\
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{(1,3)}}
&\multicolumn{1}{c|}{IMSPE} &0.772 &0.779  &0.815 & 0.791 \\
\cline{2-6}
\multicolumn{1}{|c}{}
&\multicolumn{1}{|c|}{  A  }&1.046 &0.997 &1.057 & 1.104 \\
\cline{2-6}
\multicolumn{1}{|c}{}
&\multicolumn{1}{|c|}{  D  }&-117.348 &-117.915  &-118.326 &-116.408 \\
\hline
\multicolumn{1}{|c|}{\multirow{3}{*}{(2,3)}}
&\multicolumn{1}{c|}{IMSPE} &0.857 &0.893  &0.940 &0.872 \\
\cline{2-6}
\multicolumn{1}{|c}{}
&\multicolumn{1}{|c|}{  A  }&1.003 &0.994  &1.065 &1.067 \\
\cline{2-6}
\multicolumn{1}{|c}{}
&\multicolumn{1}{|c|}{  D  }&-148.781 &-149.132  &-149.644 &-147.770 \\
\hline
\end{tabular}
}
\end{threeparttable}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion}\label{discussion}
\noindent In this Chapter we took advantage of Mercer's expansion of
covariance kernels
to analyze IMSPE-optimal designs and extend the class of optimal designs for Gaussian process models.\\

\noindent Throughout this chapter we assumed the data were observations from a
Gaussian process, which guarantees that the Kriging predictor
(\ref{kriging}) is the minimizer of the mean squared prediction error
at any site $\boldsymbol{x}$. However, if we drop the Gaussianity
assumptions, while retaining the same second order statistics, i.e.
the mean $\boldsymbol{f}^{\mathsf{T}}\ofx\boldsymbol{\beta}$ and correlation structure $R\left(\boldsymbol{x},\boldsymbol{w}\right)$,
the Kriging predictor will still be the linear unbiased predictor
with minimum variance at any site $\boldsymbol{x}$, making it a
legitimate choice; see \citet[chapter~3]{santner}. The results of
this chapter thus hold for any weakly stationary random process whose first two moments
coincide with those of process (\ref{gauss_proc}), as long as the
predictor $\widehat{y}\ofx$ is (\ref{kriging}).\\


\noindent One major drawback of the designs discussed in this
chapter is the need to provide the assumed known correlation
parameters. When performing a sequential experiment, this could be
mitigated somewhat by estimating the parameters from initial data
and generating a second stage design as in Section \ref{batch}.
Otherwise, \cite{IMSE} suggested a robustness study to choose the
parameters from a finite set of reasonable values. Alternatively, a
Bayesian approach could be applied, assigning prior distributions
based on expert opinion or past studies, as in \cite{Bingham}. The
robustness study, whose results appear in Table
\ref{tab:comparison2}, suggests that when there is a reasonable
(even if not accurate) assessment of the said parameters, using
optimal designs could still be beneficial in terms of the IMSPE.
Whether or not the improvement is significant enough to employ a
design strategy that makes strong structural assumptions over a
model-independent approach such as the maximin LHD, depends on those
carrying out the experiment and their acquaintance with the data
that are to be collected.


==> Chapters/loo_trees.tex <==

\section{Introduction}
The use of trees in predictive modeling has a long history, dating
back to early versions like CHAID \citep{kass1980exploratory}, and gaining importance in the 80s and 90s through the introduction of approaches like CART \citep{breiman1984classification} and C4.5/C5.0 \citep{quinlan2014c4, quinlan2004data}. A tree describes a recursive
partitioning of a feature space into rectangular regions intended to
capture the relationships between a collection of explanatory
variables (or features) and a response variable, as illustrated in
Figure \ref{fig:tree}. The advantages of trees that made them attractive include
natural handling of different types of features
(categorical/ordinal/numerical); a variety of approaches for dealing
with missing feature values; a natural ability to capture non-linear
and non-additive relationships; and a perceived interpretability and
intuitive appeal. Over the years it has become widely understood
that these advantages are sometimes overstated, and that tree models
suffer from a significant drawback in the form of inferior
predictive performance compared to modern alternatives (which is not
surprising, given the greedy nature of their model building
approaches). However the last 15 years have seen a resurgence in the
interest in trees as ``sub-learners'' in ensemble learning
approaches like Boosting \citep{friedman2001} and Random Forest \citep{breiman2001random}. These approaches take advantage of the favorable properties described above, and mitigate the low accuracy
by averaging or adaptively adding together many trees. They are
widely considered to be among the state of the art tools for
predictive modeling \citep{hastie2009elements}.

\begin{figure}[!ht]
\begin{center}
%\centering
\includegraphics[width = 0.5\textwidth,bb= 90 95 705 600,clip]{tree.pdf}
\caption{A tree-based model example. $x_1, x_2$ are numerical/ordinal features and $x_3$ is a categorical feature}

\label{fig:tree}
\end{center}
%\vspace{-1.5em}
\end{figure}
\noindent As mentioned, popular tree building algorithms like CART can handle
both numerical and categorical features and build models for
regression, two-class classification and multi-class classification.
The splitting decisions in these algorithms are based on optimizing
a splitting criterion over all possible splits on all variables. The
split selection problems that arise present both computational and
statistical challenges, in particular for categorical features with
a large number of categories. Assume $K$ categories overall, then
the space of possible binary splits includes $O(2^K)$ candidates,
and a naive enumeration may not be feasible. However, as
demonstrated in CART \citep{breiman1984classification}, there is no need to enumerate over all of them in order to find the optimal one for regression or two-class
classification, because it is enough to sort the categories by their
mean response value and consider only splits along this sequence.
The complexity of splitting is therefore $O(\max(K \log(K), n))$,
where $n$ is the number of observations being split. However, if $K$
is large, the splitting still presents a major statistical
(overfitting) concern. At the extreme, if $K=n$ (for example, if the
categorical variable is in fact a unique identifier for each
observation), then it is easy to see that a single split on this
variable can perfectly separate a two-class classification training
set into its two classes. Even if $K$ is smaller than $n$ but large,
it is intuitively clear (and demonstrated below) that splitting on
such a categorical variable can result in severe overfitting. This
is exacerbated by the fact that this overfitting in fact causes
common tree building splitting criteria like Gini to preferably
select such categorical variables and ``enjoy'' their overfitting.\\

\noindent Some popular tree building software packages recognize this problem
and limit the number of categories that can be used in model
building. In {\sf R}, many tree-based models limit the number of categories to $32$ (as {\sf randomForest}, for example), while Matlab's regression-tree and classification-tree routines ({\sf fitrtree, fitctree}) leave this parameter for the users to define. In what follows we denote implementations which discard categorical features with a number of categories larger than $K$ as \textit{limited-$K$} while versions which do not apply this mechanism will be denoted as \textit{unlimited-$K$}. 
The ad-hoc limited-$K$ approach is of course far from satisfactory, because the chosen number can be too small or too large, depending on the nature of the specific
dataset and the categorical features it contains. It also fails to
address the conceptual/theoretical problem: since features that
are numerical or ordinal or have a small number of categories present
a smaller number of unique splits than categorical features with
many categories, there is a lack of uniformity in split criteria
selection. Finally, some large datasets may well have categorical
features with many categories that are still important for good
prediction, and discarding them is counterproductive.\\

\noindent In this work we address these concerns through a simple modification:
We propose to select the variable for splitting based on LOO scores
rather than on training sample performance, an approach we term 
Adaptive LOO Feature selection (ALOOF). The concept of using LOO estimates for variable selection in tree-based mehods was first introduced by \cite{Frank1,Frank2}. Later, \cite{sabato2008ranking} suggested a specific LOO-based variable selection mehodology for ranking categorical features according to their generalization error. However, their approach is limited to considering (categorical) K-way splits (i.e., a leaf for every categorical value), which mainly applies for C4.5 trees. In this work we take a further step and consider a LOO-based varaible selection method for two-way splits, both for numerical and categorical features. This splitting rule is of high interest to the CART family, which together with C4.5 trees, are among the most popular (and accurate) tree methods \citep{king1995statlog, lim2000comparison, caruana2006empirical}.\\

\noindent A naive implementation of ALOOF approach would call for building $n$ different best splits on each feature, each time leaving one observation out, and select the
feature that scores best in LOO. As we demonstrate below, this
implementation can be avoided in most cases. The result of our
amendment is a ``fair'' comparison between features in selection,
and consequently the ability to accommodate all categorical features
in splitting, regardless of their number of categories, with no
concern of substantial overfitting. Importantly, this means that truly
useful categorical variables can always be taken advantage of.\\

\noindent The preceding concepts are demonstrated in Figure \ref{fig:sim3}. The simulation setting includes $n=300$ observations and an interaction between a numerical variable $x_1$ and a categorical variable $x_2$ with $K=50$ categories denoted $c_1,...,c_{50}$, with a parameter $\alpha$ controlling the strength of the interaction:
\begin{align}
\label{intro_model}
 y =& \alpha \cdot \left( {\mathbb I}\left[x_1>0\right] {\mathbb I}\left[ x_2 \in \{c_1,...,c_{25}\} \right]\right. +\left. {\mathbb I}\left[x_1 \leq 0\right] {\mathbb I}\left[ x_2 \in \{c_{26},...,c_{50}\} \right] \right) + \epsilon, 
\end{align}
where $\epsilon \sim N(0,1)$ i.i.d. At small $\alpha$ the signal from the categorical variable is weak and less informative. In this case, the limited-$K$ approach is preferable (here, as in all subsequent analyses, we use a CART limited-$K$ Matlab implementation that eliminates categorical variables with $K>32$ values). As $\alpha$ increases, the categorical variable becomes more informative and unlimited-$K$ (which refers to a CART implementation on Matlab that does not discard any categorical variable) outperforms the limited-$K$ approach for the same $n$ and $K$. ALOOF (which is also implemented on a Matlab platform) successfully tracks the preferred approach in all situations, even improving slightly on the unlimited-$K$ approach for large $\alpha$ by selecting the categorical variable less often in the tree.


\begin{figure}[!ht]
\centering
\includegraphics[width = 0.6\textwidth,bb= 40 185 580 590,clip]{simulation3_3.pdf}
\caption{Predictive performance of the two CART versions and ALOOF for the model with one categorical and one numerical feature described in the text. As can be seen, ALOOF successfully identifies the better approach throughout the range of $\alpha$ (which determines the strength of the signal from the categorical variable).}
\label{fig:sim3}
%\vspace{-1.5em}
\end{figure}

\noindent The rest of this chapter is organized as follows: In Section \ref{Sec2} we
formalize the LOO splitting approach in ALOOF and discuss its statistical
properties, we then describe our algorithmic modifications for
implementing it in Section \ref{Sec3} and demonstrate that for two-class
classification they lead to an approach whose computational
complexity is comparable to CART splitting under reasonable
assumptions. In Section \ref{Sec4} we demonstrate via some toy simulations
the striking effect that ALOOF can have on improving the
performance of tree methods. We begin Section \ref{Sec5} with a comprehensive case study, where large-K categorical variables are prevalent and important. We demonstrate the significant improvement in both interpretability and prediction from using ALOOF vs regular CART splitting. We then present an extensive real data study in both regression and classification, using both single CART trees and ensemble methods, where ALOOF offers across-the-board improvement.

\section{Related Work} We focus here on two threads of related
work, which relates to our approach from two different aspects.
The Conditional Inference Trees (CIT) framework \citep{hothorn2006unbiased} proposes a method for unbiased variable selection through conditional permutation tests. At each node, the CIT procedure tests the global null hypothesis of complete independence between the response and each feature, and selects the feature with the most significant association (smallest p-value). It terminates once the global null can no longer be rejected. The advantage of this approach is that it proposes a unified framework for recursive partitioning which embeds tree-structured models into a well defined statistical theory of conditional inference procedures. However, practically it requires the computation of p-values under permutations tests, either by exact calculation, Monte Carlo simulation, or asymptotic approximation. These permutation tests are typically computationally expensive and necessitate impractical run-time as the number of observations grows (as demonstrated in our experiments). More critically, despite its well established theory, the statistical significance criterion the CIT procedure uses is not the relevant criterion for variable selection in tree-based modeling. Notice that in each node, the feature that should be most ``informative" is the one that splits the observations so that the (test-set) generalization error is minimal. This criterion does not typically select the same variable that results with the smallest p-value under the null assumption on the train-set. As our experiments in Section \ref{Sec5}  show, our ALOOF method, based on the generalization error criterion, is superior the the CIT approach, where the CIT is computationally feasible.\\

\noindent In a second line of work, \cite{sabato2008ranking} suggest ranking categorical features according to their generalization error. However, their approach is limited to considering K-way splits (i.e., a leaf for every categorical value), as opposed to binary splits which group categories,  which characterize CART and other tree methods commonly used in statistics. Their appraoch, which is also solely applicable for classification trees, offers strong theoretical results and low computational complexity (as it does not perform actual splitting), albeit in the K-way scenario which is significantly simpler theoretically than the binary split case we are considering, which requires optimizing over $O(2^K)$ possible splits. Thus our goals are similar to theirs, but since we are dealing with a more complex problem we cannot adopt either their computational approach or their theoretical results. In our classification examples we compare our approach to theirs, demonstrating the advantage of binary splitting for attaining better predictive performance in practice.  The approach of \cite{sabato2008ranking} subsumes and improves on various previous lines of work in the machine learning literature on using cross validation to select variable in K-way splitting scenarios \citep{Frank1,Frank2}. 




\section{Formulation of ALOOF} \label{Sec2}
We present here the standard CART splitting approach \citep{breiman1984classification} based on least squares for regression and Gini index (closely related to least
squares) for classification, and then describe our modifications to
adapt them to LOO splitting variable selection. We choose to
concentrate on CART as one of the most widely used tree
implementation, but our LOO approach can be adapted to other
algorithms as well. 

\subsection{CART Splitting Rules}

Assume we have $n$ observations denoted by their indexes $\{1,...,n\}$. Each observation $i$ is comprised of the pair $(x_i,y_i)$, where  $x_i$ is a $p$ dimensional vector containing $p$ candidate variables to split on. We assume, without loss of generality (WLOG), that the variables $x_{\cdot 1}...x_{\cdot q}$ are categorical with number of categories $K_1,...,K_q$ respectively, and the features $x_{\cdot q+1},...,x_{\cdot p}$ are numerical or ordinal (treated identically by CART).  
A split $s$ is a partition of the $n$ observations into two subsets $R(s),L(s)$ such that $R(s)\cap L(s)=\emptyset$ and $R(s)\cup L(s) = \{1,...,n\}$. 
For each variable $j$, denote the set of possible splits by $S_j$ and their number by $s_j = |S_j|$. 
Categorical variable $j$ has $s_j = 2^{K_j-1}-1$ possible binary splits, and each numerical/ordinal variable has $s_j \leq n$ possible splits between its unique sorted values. \\

\noindent A specific split comprises a  selection of a splitting variable $j$ and a specific split $s \in S_j$, and is evaluated by the minimizer of an ``impurity'' splitting criterion given the split $s$, denoted by ${\cal L}(s)$. \\

\noindent In regression, CART uses the squared error loss impurity criterion:
$$ {\cal L}(s) = \sum_{i \in L(s)} (y_i - \bar{y}_L)^2 +  \sum_{i \in R(s)} (y_i - \bar{y}_R)^2,$$
where $\bar{y}_L, \bar{y}_R$ are the means of the response $y$ over the sets $L(s), R(s)$ resepectively. \\

\noindent In two-class classification, it uses the Gini index of impurity:
$$ {\cal L}(s) = n_L \hat{p}_L (1-\hat{p}_L) +  n_R  \hat{p}_R (1-\hat{p}_R), $$
where $n_L,n_R$ are the numbers of observations in $L(s),R(S)$ respectively and $\hat{p}_L,\hat{p}_R$ are the observed proportions of ``class 1'' in $L(s),R(S)$. 
The Gini index is easily seen to be closely related to the squared error loss criterion, as it can be viewed as the cross-term of a squared error loss criterion with 0-1 coding for the classes. The Gini criterion for multi-class classification is a straight forward generalization of this formula, but we omit it since we do not consider the multi-class case in the remainder of this chapter. \\

\noindent Given this notation, we can now formulate the CART splitting rule as: 
$$ (j^*, s^*) = \argmin_{\substack{j \in \{1, \dots, p \}\\ s\in S_j}} {\cal L}(s),$$
and the chosen pair $ (j^*, s^*)$ is the split that will be carried out in practice. \\

\noindent A naive implementation of this approach would require considering $\sum_j s_j$ possible splits, and performing $O(n)$ work for each one. In practice, the best split for each numerical/ordinal variable can be found in $O(n \log(n))$ operations, and for each categorical variable in $O(\max(n,  K_j  \log(K_j)))$ operations, for both regression and classification problems \cite{breiman1984classification,hastie2009elements}. Given these $p$ best splits, all that is left is to find their optimum. 

\subsection{LOO Splitting Rules}

For LOO splitting, our goal is to find the best variable to split on based on LOO scores for each variable under the given impurity criterion. The actual split performed is then the best regular CART split on the  selected variable. The resulting LOO splitting algorithm is presented in Algorithm \ref{alg:high-level LOO approach}.

\begin{algorithm}[H] 
\caption{High level ALOOF approach}
\begin{algorithmic} [1]
\FORALL{$j=1$ to $p$}
\STATE  $L(j)=0$
\FORALL{$i=1$ to $n$}
\STATE $s_{ij} = \arg\min_{s \in S_j} {\cal L}^{(-i)}(s)$
\STATE  $L(j) = L(j) + R(s_{ij},i)$
\ENDFOR
\ENDFOR
\STATE  $j* = \arg\min_{j \in \{1...,p\}} L(j)$
\STATE  $s* = \arg\min_{s \in S_{j*}} {\cal L} (s)$

\end{algorithmic}
\label{alg:high-level LOO approach}
\end{algorithm}

\noindent The result of Algorithm \ref{alg:high-level LOO approach} is again a pair $(j^*,s^*)$ describing the chosen split. 
The additional notations used in this description are: 
\begin{enumerate}
\item ${\cal L}^{(-i)}(s)$: the impurity criterion for candidate split $s$, when excluding the observation $i$. For example, if we assume WLOG that $i\in L(s)$ and the impurity criterion is the suaqred loss, we get 
$${\cal L}^{(-i)}(s) = \sum_{l \in L(s), l\neq i} \left(y_l - \bar{y}^{(-i)}_L\right)^2 +  \sum_{l \in R(s)} \left(y_l - \bar{y}_R\right)^2,$$
where $\bar{y}^{(-i)}_L$ is the average calculated without the $i$th observation. If the criterion is Gini or the observation falls on the right side, the obvious modifications apply. Consequently, $s_{ij}$ is the best split for variable $j$ when excluding observation $i$.  
\item $R(s,i)$: the LOO loss of the $i$th observation for the split $s$. In the above case (squared loss, left side) we would have: 
$$ R(s,i) = \left(y_i - \bar{y}^{(-i)}_L\right)^2,$$
with obvious modifications for the other cases. $L(j)$ is simply the sum of $R(s_{ij},i)$ over $i$, i.e., the total LOO loss for the $j$th variable when the best LOO split $s_{ij}$ is chosen for each $i$. 
\end{enumerate}
\noindent A naive implementation of this algorithm as described here would require performing $n$ times the work of regular CART splitting, limiting the usefulness of the LOO approach for large data sets. As we show below, for two-class classification we can almost completely eliminate the additional computational burden compared to regular CART splitting, by appropriately enumerating the LOO splits. For regression, the worst case performance of our approach is unfortunately close to being $n$ times worse than regular CART splitting. In practice, the added burden is much smaller. 


\subsection{What is ALOOF Estimating?} \label{unbias}

The quantity $L(j)$ in our LOO approach directly estimates the generalization error of splitting on variable $j$ using a CART impurity criterion: for each observation $i$, the best split is chosen based on the other $n-1$ observations, and judged on the (left out) $i^{th}$ observation. Hence $L(j)$ is an unbiased estimate of generalization impurity error for a split on variable $j$ based on a random sample of $n-1$ observations. The selected splitting variable $j^*$ is the one that gives the lowest unbiased estimate. Hence our goal of judging all variables in a fair manner,  that identifies the variables that are truly useful for reducing impurity and not just over-fitting is attained. \\

\noindent Since we eventually perform the best split on our complete data at the current node ($n$ observations), there is still a small gap remaining between the ``$n-1$ observations splits'' being judged and the ``$n$ observations split'' ultimately performed, but this difference is negligible in most practical situations (specifically, when $n$ is large). 

\subsection{ALOOF Stopping Rules} \label{stop}

Tree methods like CART usually adopt a grow-then-prune approach, where a large tree is first grown, then pruned (cut down) to ``optimal'' size based on cross-validation or other criteria \citep{breiman1984classification}. 
Because cross-validation is built-in to the ALOOF splitting variable selection approach, it obviates the need to take this approach. For every variable, ALOOF generates an almost unbiased estimate of the generalization error (in Gini/squared loss) of splitting on this variable. If an additional split on any variable would be detrimental to generalization error performance, this would manifest in the ALOOF estimates (in expectation, at least) and the splitting would stop. This approach is not perfect, because ALOOF generates an almost-unbiased estimate for every variable, then takes the best variable, meaning it may still be over-optimistic and continue splitting when it is in fact slightly overfitting. However in our experiments below it is demonstrated that the combination of ALOOF's variable selection with ALOOF's stopping rules is superior to the CART approach. \\

\noindent It should be noted that in Boosting or Random Forest approaches utilizing trees as a sub-routine, it is usually customary to avoid pruning and determine in advance the desirable tree size (smaller in Boosting, larger in Random Forest). Similarly, when we implement ALOOF within these methods, we also build the tree to the same desirable size, rather than utilize ALOOF stopping rules. 

\section{Efficient Implementation} \label{Sec3}
As described above, the ALOOF algorithm utilizes a seemingly computationally expensive LOO cross-validation approach. However, we show that with a careful design, and under reasonable assumptions, we  are able to maintain the same computational complexity of the CART algorithm for two-class classification modeling. In addition, we show that for regression tasks ALOOF carries some increase of the computational burden, replacing a $O(log(n))$ factor in CART splitting rules with an $O(n)$ term.
We present our suggested implementation for both categorical and numerical/ordinal variables, in both two-class classification and regression settings. 

\subsection{Two-class Classification --- Categorical Variables}

Assume a categorical variable with $K$ different categories. As described above, the CART algorithm performs a split selection by sorting the $K$ categories by their
mean response value and consider only splits along this sequence. Therefore, the complexity of finding the best split for this variable is $O(\max(K \log(K), n))$, where $n$ is the number of observations being split.\\

\noindent We now present our suggested implementation and compare its computational complexity with CART. 
First, we sort the observations according to the mean response value of the $K$ categories, just like CART does. Then, for each pair $(x_i,y_i)$ we leave out, we recalculate its category's mean response (an $O(1)$ operation), and re-sort the categories by their new means. Notice that since only a single category changes its mean ($x_i$'s category), re-sorting the sequence takes only $O(\log(K))$. Once the sequence is sorted again we simply go over the $K$ splits along the sequence. Therefore, for each pair $(x_i,y_i)$ ALOOF necessitates $O(K)$ operations. 
It is important to notice that despite the fact we have $n$ observations, there are only two possible pairs for each category, as $y_i$ takes only two possible values in the classification setting. This means we practically need to repeat the LOO procedure only for $2K$ pairs. Hence, our total computational complexity is $O(\max(K^2, n))$.\\

\noindent We further show that under different reasonable assumptions, our computational complexity may even be equal to the complexity of CART splitting. 
First, assuming the number of categories grows no faster than the square root of $n$, $K^2=O(n)$, it is immediate that both algorithms result with a complexity of $O(n)$. This setting is quite common for the majority of categorical variables in real-world datasets. \\

\noindent Second, under the assumption that a single observation cannot dramatically change the order of the categories in the sorted categories sequence, then the worst case complexity is lower than $O(\max(K^2, n))$. More specifically, assuming a single observation can move the position of its category by at most $B$ positions in the sorted categories sequence, then the complexity we achieve is $O(\max(K\log(K), KB, n))$. This assumption is valid, for example, when all categories have about the same number of observations. To emphasize this point, consider the case where the number of observations in each category is exactly the same, so that each category consist of $\sfrac{n}{K}$ observations. In this case the effect of changing the value of a single observation (on the category's mean) is proportional to ($\sfrac{K}{n}$). In other words, $\sfrac{K}{n}$ corresponds to the smallest possible difference between categories' means. Moreover, when leaving out a single observation, the change in this category's mean is bounded by this value. Hence, re-sorting the categories (following the LOO operation) is not more than an exchange of positions of consecutive categories in the sorted categories sequence ($B=1$). This leads to an overall complexity equal to CART's.

\subsection{Two-class Classification --- Numerical Variables}
For numerical variables, CART performs a split selection by first sorting the $n$ pairs of observations according to their $x_i$ values, and then choosing a cut (from at most $n-1$ possible cuts) that minimizes the Gini criterion along both sides of the cut. By scanning along the list with sufficient statistics this takes $O(n)$ operations, leading to overall complexity $O(n\log(n))$ due to the sorting.\\

\noindent Our suggested implementation again utilizes the fact that $y_i$ takes only two possible values to achieve a complexity identical to CART's. Here we denote the values as $y_i \in \{-1,1\}$, we initialize our algorithm by sorting the observations in the same manner CART does. We then take out the observation $y_i=1$ with the lowest value of $x_i$, and find its best cut (by going over all $n-2$ possible cuts). We then place this observation back and take out the observations for which $y_i=1$, with the second lowest value of $x_i$. Notice that the only cuts whose Gini index values are affected by these operations are the cuts between the two pairs we replaced. Denote this group of cuts by $N_2$. This means that when exchanging the two observations we need to update the Gini values of at most $|N_2|$ cuts to find the best LOO cut. Continuing in the same manner leads to a total complexity of $O(\sum{|N_j|})=O(n)$ for finding the best cut of all observations with $y_i=1$. This process is then repeated with observations for which $y_i=-1$. Therefore, the overall complexity of our suggested implementation is $O(2n+n\log(n))=O(n\log(n))$, just like CART. We present pseudo-code of our suggested approach in Algorithm \ref{alg:algorithm}. To avoid an overload of notation we only present the case of observations for which $y_i=1$. The key idea is presented in steps 20-21 of the algorithm, where it is emphasized that only the splits in $N_j$ have to be considered in every step.  

\begin{algorithm}\label{alg1}
\caption{LOO best split selection for numerical variables in two-class classification modeling}
\begin{algorithmic} [1]
\REQUIRE Observations $(x_1,y_1),\ldots,(x_n,y_n)$.
\REQUIRE $j=1$, $n_1=$number of observations for which $y_i=1$,  $optimal${\_}$cut=$ array of size $n_1$ holding the best LOO cut for each of the $y_i=1$ observations.
\STATE Sort observations according to $x_i$ values.

\STATE Set $A=\{(x_1,y_1),\ldots,(x_n,y_n)$ such that $y_i=1\}$.
\STATE Set $A=$sort $A$ according to its $x_i$ values in ascending order.

\STATE $A=A\setminus (x_1,y_1)$.
\STATE $optimal${\_}$cut_j=\infty$.
\STATE $optimal${\_}$cut${\_}$Gini=\infty$.

\FORALL{$(x_i, y_i)\in A $}
\STATE Set $cut_i=\frac{x_i+x_{i+1}}{2}$.
\STATE Set $Gini_i=$ Gini index value with respect to the cut $cut_i$.
\IF {$Gini_i<optimal${\_}$cut${\_}$Gini$}
\STATE $optimal${\_}$cut_j=cut_i$.
\STATE $optimal${\_}$cut${\_}$Gini=Gini_i$.
\ENDIF
\ENDFOR
\STATE $j=j+1$


\FORALL{$j\in\{2, \ldots, n_1\}$}
\STATE Set $A=A\cup (x_{j-1},y_{j-1})$.
\STATE Set $A=A\setminus(x_j,y_j)$.
\STATE $optimal${\_}$cut_j=optimal${\_}$cut_{j-1}$.
\STATE $N_j=\{(x_i,y_i) \in A$ such that $x_{j-1} <x_i<x_{j} \}$ .
\FORALL{$(x_i, y_i)\in N_j $}
\STATE Set $cut_i=\frac{x_i+x_{i+1}}{2}$.
\STATE Set $Gini_i=$ Gini index value with respect to the cut $cut_i$.
\IF {$Gini_i<optimal${\_}$cut${\_}$Gini$}
\STATE $optimal${\_}$cut_j=cut_i$.
\STATE $optimal${\_}$cut${\_}$Gini=Gini_i$.
\ENDIF
\ENDFOR
\STATE $j=j+1$.
\ENDFOR

\RETURN $optimal${\_}$cut$
\end{algorithmic}
\label{alg:algorithm}
\end{algorithm}

\subsection{Regression --- Categorical Variables}
The regression modeling analysis case is similar to the two-class classification in the presence of categorical variable, with a simple modification of the loss impurity criterion. 
Both CART and our suggested ALOOF method replace the Gini index with the squared error loss impurity criterion and follow the exact same procedures mentioned above. This leads to a overall complexity of $O(\max(K\log(K),n)$ for the CART algorithm and $O(\max(n,K^2))$ for our ALOOF method. As before, the computational complexity gap between the two methods may reduce under some reasonable assumptions. One simple example is when $K^2=O(n)$. Another example is in cases where we can assume that the effect of a single observation on the mean response value of each category is bounded. This happens, for instance, when the the range of the response values is bounded and there is approximately the same number of observations in each category.    

\subsection{Regression --- Numerical Variables}
In this setting as well, we compare both algorithms' implementation to those of the classification problem. 
The CART algorithm first sorts the $n$ observation pairs according to their $x_i$ values, and then chooses a cut that minimizes the squared error loss along both sides of the cut. As in the classification case, scanning along the list with sufficient statistics this takes $O(n)$ operations, leading to overall complexity $O(n\log(n))$ due to the sorting.\\

\noindent As we examine the LOO method in this regression setting, we notice that unlike CART, it fails to simply generalize the two-class classification problem. Specifically, it is easy to show that for each observation pair $(x_i, y_i)$ that is left out, the best cut may move in a non-monotonic manner (along the values of the numerical variable $x$), depending on the specific values of the observations that were drawn. This unfortunate non-monotonic behavior leads to a straight-forward implementation, where we first sort the observations by their $x_i$ values and then find the best cut for each observation that is taken-out by exhaustive search. The overall complexity is therefore $O(n^2)$, which compared with the CART implementation, replaces the $O(\log(n))$ factor with $O(n)$. 


\section{Illustrative Simulations} \label{Sec4}

We start with two synthetic data experiments which demonstrate the behavior of ALOOF compared with CART in the presence of a categorical variable with varying number of categories. 
In the first experiment we examine our ability to detect a categorical variable which is not informative with respect to the response variable. Our goal is to model and predict the response variable from two different explanatory variables, where the first is numerical and informative while the other is categorical with $K$ different categories, and independent of the response variable.  We draw $1000$ observations which are split into $900$ observations for the train-set and $100$ for the test-set. We repeat this process multiple times and present averaged results. 
Figure \ref{fig:sim1_1} shows the test-set's average mean square error (MSE) for different number of categories $K$, using three different methods. The upper curve corresponds to the classic CART model, which is extremely vulnerable to categorical variables with large number of categories, as discussed above. The full line is our suggested ALOOF method, which manages to identify the uselessness of the categorical variable and discards it. The line with the {\sf x} symbols at the bottom is the CART model without the categorical variable at all, which constitutes a lower bound on the MSE we can achieve, using a tree-based model.   

\begin{figure}[!ht]
\centering
\includegraphics[width = 0.7\textwidth,bb= 30 100 750 490,clip]{simulation1_4.pdf}
\caption{Tree-based modeling in the presence of an uninformative categorical feature}
\label{fig:sim1_1}
%\vspace{-1.5em}
\end{figure}
\noindent In the second synthetic data experiment we revisit the model presented in the Introduction (\ref{intro_model}) as an example of a model with an informative categorical variable. We fix the strength of the interaction between the numerical and the categorical variables ($\alpha=15$) and repeat the experiment for different values of $K$. Figure \ref{fig:sim1_2} presents the results we achieve. As in the previous example ALOOF demonstrates superior performance to both its competitors as $K$ increases. This exemplifies the advantage of using ALOOF both when the categorical variable is informative or uninformative, for any number of categories $K$.  \\

\begin{figure}[!ht]
\centering
\includegraphics[width = 0.7\textwidth,bb= -10 100 710 490,clip]{simulation4.pdf}
\caption{Tree-based modeling in the presence of an informative categorical feature, (according to the model described in (\ref{intro_model}) with $\alpha=15$)}
\label{fig:sim1_2}
%\vspace{-1.5em}
\end{figure}
\noindent We now turn to compare the modeling complexity of the ALOOF approach with that of CART. Since CART has a tree-depth parameter it may provide a variety of models which differ in their model complexity and the corresponding MSE they achieve. ALOOF, on the other hand, results in a single model, using the stopping policy described in Section \ref{stop}, with its corresponding MSE. Therefore, to have a fair comparison between the two methods we use degrees of freedom ($df$). We start with a brief review of the main ideas behind this concept. \\

\noindent Following \cite{efron1986biased} and \cite{hastie2009elements}, assume 
the values of the feature vectors $X=(x_1,...,x_n)$  are fixed (the fixed-x assumption), and that the model gets one vector of response variable $Y=(y_1,...,y_n)$
for training, drawn according to the conditional probability model $p(Y|X)$ at the n data points. Denote by $Y^{new}$
another independent vector drawn according to the same distribution. $Y$ is
used for training a model $\hat{f}(x)$ and generating predictions $\hat{y_i}=\hat{f}(x_i)$ at the $n$ data points.
We define the training mean squared error as
\begin{equation}
MRSS=\frac{1}{n}\|Y-\hat{Y}\|^2_2
\end{equation}
and compare it to the expected error the same model incurs on the new, independent
copy, denoted by \cite{hastie2009elements} as $ERR_{in}$,
 \begin{equation}
ERR_{in}=\frac{1}{n}\mathbb{E}_{Y^{new}}\|Y^{new}-\hat{Y}\|^2_2
\end{equation}
The difference between the two is the \textit{optimism} of the prediction.
As \cite{efron1986biased} and others have shown, the expected optimism in MRSS is
 \begin{equation}
\mathbb{E}_{Y,Y^{new}}(ERR_{in}-MRSS)=\frac{2}{n}\sum_{i}cov(y_i,\hat{y_i})\label{eq:ERR-MRSS}
\end{equation}
For linear regression with homoskedastic errors with variance $\sigma^2$, it is easy
to show that (\ref{eq:ERR-MRSS}) is equal to $\frac{2}{n}d\sigma^2$ where $d$ is the number of regressors,
hence the degrees of freedom. 
In nonparametric models (such as tree-based models), one usually cannot calculate the actual degrees of freedom of a modeling approach. However, in simulated examples it is possible to generate good estimates $\hat{df}$ of $df$ through repeated generation of $Y, Y^{new}$ samples to empirically evaluate (\ref{eq:ERR-MRSS}). \\

\noindent In the following experiment we compare the models' degrees of freedom for CART and ALOOF. As explained above, CART generates a curve of values where the $df$ increases with the size of the tree (hence, the complexity of the model) and the MSE is the error it achieves on the test-set. Our ALOOF method provides a single value of MSE for the model we train. We draw $n=200$ observations from the same setup as in Figure \ref{fig:sim1_1} and achieve the results shown in Figure \ref{fig:sim2} for three different values of $K$. The straight line at the bottom of each figure is simply to emphasize that the MSE ALOOF achieves is uniformly lower than CART's curve, although it imposes more $df$ compared to the optimum of the CART curve. It is important to notice that this ``CART optimum" is based on Oracle knowledge; in practice, the pruned CART model is selected by cross-validation. Typically, it fails to find the model which minimizes the MSE on the test-set. As we look at the results we achieve for different values of $K$ we notice that ALOOF's superiority grows as the number of uninformative categories increases, as we expect. 


\begin{figure}[!ht]
\centering
\includegraphics[width = 0.7\textwidth,bb= 40 100 765 520,clip]{simulation2_5.pdf}
\caption{Modeling complexity (represented in $df$) and its corresponding MSE in the presence of uninformative categorical feature with $K$ different categories. The curve corresponds to CART model, the asterisk is our ALOOF approach and the straight line is to emphasize that the MSE we achieve is uniformly lower than CART's curve}
\label{fig:sim2}
%\vspace{-1.5em}
\end{figure}

\section{Real Data Study} \label{Sec5}

We now apply our ALOOF approach to real-world datasets and compare it with different commonly used tree-based methods. For obvious reasons, the data-sets we focus on are ones that include categorical features with a relatively large number of categories. All these dataset are collected from UCI repository \citep{Lichman:2013}, CMU Statlib \footnote{\url{http://lib.stat.cmu.edu/}} and Kaggle\footnote{\url{http://www.kaggle.com/competitions}} and are publicly available. \\

\noindent Throughout this section we use ten-fold cross validation to achieve an averaged validation error on each dataset. In addition, we would like to statistically test the difference between ALOOF and its competitors and assert its statistical significance. However, the use of $K$-fold cross validation for model evaluation makes this task problematic, as the variance of cross validation scores cannot be estimated well \citep{bengio}. Some mitigations have been proposed to this problem in the literature, but we are not aware of a satisfactory solution.
Therefore we limit our significance testing to policies that circumvent this problem: 
\begin{itemize}
\item For larger datasets ($>1000$ observations) we use a single 90-10 training-test division to test for significance separately from the cross validation scheme. 
\item Combining the results of all datasets, we perform a sign test to verify the ``overall'' superiority of ALOOF.  
\end{itemize}

\noindent We begin our demonstration with a comprehensive case study of the Melbourne grants dataset\footnote{\url{https://www.kaggle.com/c/unimelb}}

\subsection{Case Study: Melbourne Grants} 
The Melbourne Grants dataset was featured in a competition on the Kaggle website. The goal was to predict the success of grant applications based on a large number of variables, characterizing the applicant and the application. The full training dataset, on which we concentrate, included $8708$ observations and $252$ variables, with a binary response (success/failure). We only kept $26$  variables (the first ones, excluding some identifiers), and eliminated  observations that had missing values in these variables, leaving us with a dataset of $n=3650$ observations and $p=26$ variables. 
This dataset is interesting because some of the clearly relevant variables are categorical with many values, including: 
\begin{itemize}
\item The Field/Academic classification of the proposal ($510$ categories, encoded as codes from the Australian Standard Research Classification (ASRC)).
\item The Sponsor of the proposal ($225$ categories, an anonymized identifier).
\item The Department of the proposer ($90$ categories).
\item The Socio-economic code describing the potential impact of the proposed research ($318$ categories, encoded as codes from the Australian and New Zealand Standard Research Classification (ANZSRC)). 
\end{itemize}
Other clearly relevant variables include the history of success of failure by the current proposer, academic level, etc. \\

\noindent In Figure \ref{fig:melb} we present the top three level of three trees built on the entire dataset, using unlimited-K CART, limited-K CART and ALOOF. As expected, the unlimited-K version uses exclusively the largest-K categorical variables, the limited-K version is not exposed to them, so identifies the history of success as the most relevant non-categorical information, while ALOOF combines the use of one categorical variable (Sponsor), with the history of success. The ten-fold cross-validation errors of the three complete trees, as shown in Table \ref{table:melb}, is $0.245, 0.260, 0.218$, respectively. As discussed above, the ability to accurately infer significance from $K$-fold cross validation is limited. Therefore, in addition to the cross validation experiments, we arbitrarily partition the dataset into $90\%$  train-set and $10\%$ test-set, and apply a $t$-test on results we achieve on the test-set. 
This way we conclude that the advantage of ALOOF is statistically significant at level $0.05$ on a single random fold of the ten-fold CV.\\



\begin{figure}[htbp]
\centering
\includegraphics[width =0.8\textwidth,bb= 90 40 520 770,clip]{mel_trees_2.pdf}
\caption{Top three levels of trees built on the Melbourne Grants data using unlimited-K (standard) CART, limited-K CART (which eliminates categorical variables with $K>32$), and ALOOF.}
\label{fig:melb}
%\vspace{-1.5em}
\end{figure}
\noindent The advantage of ALOOF over CART is preserved when they are used as sub-learners in Gradient Boosting (GB) and Random Forest (RF), also shown in Table \ref{table:melb}. For GB we use $50$ trees and limit their complexity by defining the minimum number of observations in the trees' terminal nodes to be $0.05\cdot n$. We train the model with a learning parameter of $\nu=0.1$ (see \citep{friedman2001} for further details). For the RF method we use {\sf Matlab}'s procedure {\sf treeBagger} with $500$ trees, where the rest of the parameters are maintained in their default values. Although the number of trees we utilize in both ensemble methods may seem relatively small, our experiments show that additional trees are not necessary as they do not significantly change the results we achieve.  \\

\begin{table}[htbp]
\caption{Misclassification results of two CART versions and ALOOF on the Melbourne Grant dataset. Results reported are from ten-fold CV. Results are shown for a single tree, Gradient Boosting trees and Random Forest (see text for details). The stars denote that the performance of ALOOF is statisticially significantly superior for all three versions.}
\centering
\renewcommand{\baselinestretch}{1}\footnotesize
\label{table:melb} 
\centering
\begin{tabular}{cccc}  
\hline
Approach & Unlimited-K & Limited-K & ALOOF\\
\hline
Single tree & $0.245$&$0.260$&$0.218^*$ \\
Gradient Boosting  &$0.186$ & $0.192$ &${0.165^*}$ \\
Random Forest &$0.172$ & $0.185$ &${0.153^*}$ \\
\hline
\end{tabular}
\end{table}

\noindent To gain further insight we can examine the variable importance measure commonly used in RF \citep{breiman2001random}, which judges the performance based on permutation tests on out-of-bag (OOB) samples. In Table \ref{tab:RFimp} we show the top five variables for each RF version. We can see that the lists of unlimited-K and limited-K CART have only one variable in common (Grant category code), while the ALOOF list combines the top three variables from the unlimited-K list and the top two from the limited-K list. This reiterates ALOOF's ability to take advantage of both categorical and numerical variables in a balanced manner.  \\

\begin{table}[htbp]
\caption{Top variables according to Random Forest's variable importance measure for each of the three tree-building approaches. As can be seen, ALOOF successfully identifies and combines the categorical and numeric variables that are most useful.}
\centering
\renewcommand{\baselinestretch}{1}\footnotesize
\label{tab:RFimp} 
\centering
\begin{tabular}{cccc}  
\hline

Rank & Unlimited-K & Limited-K & ALOOF\\

\hline
$1$ &  Sponsor&\begin{tabular}{@{}c@{}} Successful grants \end{tabular} & Sponsor \\
$2$  &Field &\begin{tabular}{@{}c@{}} Unsuccessful grants \end{tabular} &\begin{tabular}{@{}c@{}} Successful grants \end{tabular}  \\
$3$  &\begin{tabular}{@{}c@{}} Socio-economic code \end{tabular}  & \begin{tabular}{@{}c@{}}  Grant category code \end{tabular}  &\begin{tabular}{@{}c@{}} Unsuccessful grants \end{tabular}   \\
$4$ &\begin{tabular}{@{}c@{}} Department \\  \end{tabular} & \begin{tabular}{@{}c@{}} Faculty member \end{tabular}  & Field \\
$5$ & \begin{tabular}{@{}c@{}}  Grant category code \end{tabular}  & Grant's value & \begin{tabular}{@{}c@{}} Socio-economic code \end{tabular} \\ 
\hline
\end{tabular}
\end{table}

\subsection{Regression Problems} 
We now turn to real-world regression problems. We first demonstrate our suggested approach with three classical small-size datasets.
In the Automobile dataset, we model the price of a car given a set of relevant features. This set of features include the car's brand which consists of $32$ categories. As previously discussed, the presence of such a categorical feature may cause overfitting as there are only $192$ observations. 
The Baseball experiment provides two designated datasets for hitters and catchers, where the goal is to predict the salary of each player in the preceding year. Here, the ``problematic" categorical feature is the player's team, consisting of $24$ different categories.   \\

\noindent Table \ref{table:real-world-small} summarizes the results we achieve applying three different method. The CART column corresponds to a standard unlimited-K CART algorithm. CIT is the {\sf R} implementation of the Conditional Inference Tree ({\sf ctree}) using its default parameters of $10000$ Monte-Carlo replications to attain the distribution of the test statistic and a corresponding p-value threshold of $0.05$. ALOOF is our suggested algorithm.
As our datasets are relatively small, we use ten-fold cross validation to estimate an averaged $MSE$. Ours results demonstrate the advantage that ALOOF's LOO selection scheme has over both the overfitting approach of CART and significance-based approach of CIT in generating good prediction models. 

\begin{table}[ht]
\caption{Regression real-world data experiments on small datasets. For each dataset we introduce its categorical variables whose number of categories $K_j$ is relatively large. CART is a standard CART implementation, CIT corresponds to the Conditional Inference Trees \cite{hothorn2006unbiased} and ALOOF is our suggested method. The performance of each method is measured by averaged $MSE$, via ten-fold cross validation}
\centering
\renewcommand{\baselinestretch}{1}\footnotesize
\label{table:real-world-small} 
\centering
\begin{tabular}{ M{3cm} M{1.7cm} M{0.65cm} M{0.65cm} M{1.0cm} N}  

\hline

Dataset (size)
&\begin{tabular}{@{}c@{}} Categorical \\ variables ($K_j$) \end{tabular}
&CART
&CIT
&ALOOF&\\[15pt]

\hline

\begin{tabular}{@{}c@{}} Auto  $(192)$ \end{tabular}   
&\begin{tabular}{@{}c@{}} Car brand $(32)$ \end{tabular}  
&$9.48$
&$13.24$ 
&${8.22}$&\\[15pt]  


\begin{tabular}{@{}c@{}} Baseball hitters $(264)$ \end{tabular}   
& Team $(24)$  
&$0.140$
&$0.136$ 
&$0.131$&\\[15pt]  



\begin{tabular}{@{}c@{}} Baseball  catchers  $(176)$ \end{tabular}   
& Team $(24)$  
&$0.076$
&$0.075$ 
&$0.062$&\\[15pt]  

\hline

\end{tabular}
\end{table}
\vspace{1em}
\noindent In addition to these illustrative small-size datasets we apply our suggested method to more modern and large-scale regression problems. Table \ref{table:real-world-large-reg} presents the results we achieve in five different regression experiments. In Boston Housing we predict the value of each house, where the town's name is the categorical variable which may cause overfitting. In the Strikes experiment we model volume of large strikes (days lost due to industrial disputes) over a total of more than $30$ years. The name of the country in which the strike took place is the categorical variable with relatively many categories. The Donations dataset is from \textit{KDD} Cup of $1998$ (excluding missing values) where participants were asked to model the amount of donations raised, given a list of variables. These included several categorical variables, each with a large number of categories, as described in Table \ref{table:real-world-large-reg}. The Internet usage dataset consists of two modeling problems. The first models the number of years a household is connected to an Internet provider while the second models the household's income. The variables used for modeling include multiple socio-economical variables where the problematic categorical ones are the occupation, language and the residence country of each household.\\

\noindent In all of these experiment we apply our ALOOF algorithm and compare it with a limited-$K$ and an unlimited-$K$ CART algorithms (as described above). Notice that in these large-scale experiments we cannot apply the CIT  method \citep{hothorn2006unbiased} as it is computationally infeasible.
In addition to these single tree models we also apply the ensemble methods Gradient Boosting (GB) and Random Forest (RF). We apply both of these methods using either unlimited-K CART trees or our suggested ALOOF method as sub-learners (limited-K is not competitive in relevant problems, where important categorical predictors are present, as demonstrated in the detailed Melbourne Grants case study). 
We apply GB and RF with the same set of parameters mentioned above. As in previous experiments we use ten-fold cross validation to achieve an averaged validation $MSE$. In addition, in order to attain statistically significant results we infer on a single random fold of the ten-fold CV for sufficiently large datasets (above $1000$ observations: the last three datasets in Table  \ref{table:real-world-large-reg}). A star indicates that the difference between ALOOF and its best competitor is statistically significant according to this $t$-test.\\

\noindent The results we achieve demonstrate the advantage of using ALOOF  both as a single tree and as a sub-learner in ensemble methods. Note that while the MSE ALOOF achieves in a single tree setting is consistently significantly lower than its competitors, it is not always the case with ensemble methods. This emphasizes the well-known advantage of using ensemble methods over a single tree, which can sometime mitigate the shortcomings of a single tree. However, it is still evident that ALOOF based ensemble methods are preferable (or at least equal) to the CART based methods. Moreover, it is notable that in some cases a single ALOOF tree achieves competitive results to ensemble based methods, such as in the Internet dataset.  



\subsection{Classification Problems} 


In addition to the real-world regression experiments we also examine our suggested approach on a varity two-class classification problems. For each examined dataset we provide its number of observations and the portion of positive response values, as reference to the misclassification rate of the methods we apply. 
The Online Sales dataset describes the yearly online sales of different products. It is originally a regression problem which we converted to a two-class classification by comparing each response value to the mean of the response vector. Its variables' names are confidential but there exist several categorical variables with relatively large number of categories, as described in Table \ref{table:real-world-large-class}.  The Melbourne Grants dataset is described in detail above. The Price Up dataset provides a list of products and specifies whether the prices were raised at different stores in different time slots. It provides a set of variables which consist of two ``problematic" categorical variables: The name of the product and its brand. In the Salary Posting experiment our task is to determine the salary of a job posting given a set of relevant variables. As in the Online Sales, this dataset too is originally a regression problem which we converted to a two-class classification by comparing each response value with the mean of the response vector. Its ``large-$K$" categorical variables are the location of the job, the company and the title of the offered position. Lastly, the Cabs Cancellations dataset provides a list of cab calls and specifies which ones were eventually canceled.  The area code is the categorical variable which contains a large number of categories. \\

\noindent As in the regression experiments, we apply different tree-based modeling methods to these datasets and compare the misclassification rate we achieve. In addition to the methods used in the regression problems we also apply the  method of \cite{sabato2008ranking}, which is designed for classification problems. We again perform a ten-fold cross validation to estimate the misclassification rate. As before, we also arbitrarily partition large datasets (the last four in Table \ref{table:real-world-large-reg}) into $90\%$  train-set and $10\%$ test-set, and apply a paired test on the difference between the results we achieve using ALOOF and each of its competitors. A star indicates that the difference between ALOOF and its best competitor is statistically significant.\\

\noindent As in the regression experiments, it is evident that our suggested ALOOF method is preferable both as a single tree and as sub-learner in ensemble methods. Note that in several experiments (such as Salary Postings) our advantage is even more remarkable compared with a limited-$K$ CART, which simply discards useful categorical variables only because they have too many categories. It is also notable that the single ALOOF tree is competitive with CART-based ensemble methods for several of the datasets. In particular, for the last three datasets the gain from replacing a single ALOOF tree with either GB or RF using CART is not statistically significant (whereas GB/RF + ALOOF does significantly improve on the CART ensemble counterparts).  \\

\noindent In addition to the misclassification rate, we also evaluated the performance of our suggested algorithm under the Area Under the Curve (AUC) criterion. The results we achieved were very simialr with those in Table \ref{table:real-world-large-reg} and are omitted from this chapter for brevity. \\

\noindent In order to obtain a valid overall statistical inference on the results we achieve, we examined the null hypothesis that ALOOF performs equally well to each of its competitors, based on all the datasets together, using a one-sided sign test as suggested by \cite{demvsar2006statistical}. 
For every competitor, we count the number of datasets (out of ten in Tables \ref{table:real-world-large-reg} and \ref{table:real-world-large-class} combined) in which ALOOF wins and apply a one-sided sign test. ALOOF outperforms both versions of CART on all datasets examined, performs better in GB for nine of ten, and for RF in eight of ten, with corresponding one-sided p-values of $0.001$, $0.01$ and $0.05$, respectively, after continuity correction. 




\section{Discussion}
In this chapter we have demonstrated that the simple cross-validation scheme underlying ALOOF can alleviate a major problems of tree-based methods that are not able to properly utilize categorical features with large number of categories in predictive modeling. By adopting a LOO framework for selecting the splitting variable we allow ALOOF to eliminate categorical features that do not improve prediction, and select the useful ones even if they have many categories.\\

\noindent As our simulations and real data examples demonstrate, the effect of using the ALOOF approach for splitting feature selection can be dramatic in improving predictive performance, specifically when categorical features with many values are present and carry real information (i.e., cannot simply be discarded). \\

\noindent A key aspect of our approach is the design of efficient algorithms for implementing ALOOF that minimize the extra computational work compared to simple CART splitting rules. As our results in Section \ref{Sec3} indicate, ALOOF is more efficient in two-class classification than in regression. In practice, in our biggest regression examples in Section \ref{Sec5} (about $10,000$ observations), building an ALOOF tree takes up to $15$ times longer than building a similar size CART tree (the exact ratio obviously depends on other parameters as well). This means that at this data size, regression tree with ALOOF is still a practical approach even with GB or RF.  \\

\noindent For larger data sizes, an obvious mitigating approach to the inefficiency of ALOOF in regression is to avoid using LOO in this case, instead using L-fold cross validation with $L<<n$. This would guarantee the computational complexity is no larger than $L$ times that of CART splitting even with a naive implementation. The price would be a potential reduction in accuracy, as the {\em almost unbiasedness} discussed in Section \ref{unbias} relies on the LOO scheme. \\

\noindent Despite the LOO estimate being (almost) unbiased, there are well known results on the high variance of LOO estimates of prediction error \citep{elisseeff2003leave} which make them  unreliable for  model selection \citep{cawley2010over}. This argument is mainly based on synthetic \citep{cawley2010over} and real-world \citep{kohavi1995study} experimental studies. However, it is clear that reducing the number of folds does not mitigate this problem, as \cite{burman1989comparative} and  \cite{arlot2010survey} argue that in typical cases, the variance decreases with the number of folds. Since our application is not a simple model selection one, we rely on the extensive empirical evidence we present to argue that the high variance of LOO model selection does not negatively impact its utility within our framework of splitting variable selection in trees. \\


\onecolumn
\begin{landscape}
\begin{table*}[htbp]
\caption{Regression real-world data experiments. For each dataset we introduce its categorical variables whose number of categories $K_j$ is relatively large. limited-$K$ CART is a CART implementation which discards categorical variables with $K_j>32$ while the unlimited-$K$ CART is an implementation which does not discard any variable. Gradient Boosting (GB) modeling with $50$ trees and Random Forest (RF) with $500$ are also provided, both with either CART or ALOOF as a sub-learner. The performance of each method is measured by averaged $MSE$, via ten-fold cross validation. In addition, a star indicates that the difference between ALOOF its best competitor in the same category (single tree, GB, RF) is statistically significant on a single arbitrary partitioning to train and test sets (this test was only applied to the last three datasets, with more than 1000 observations). }

\centering
\renewcommand{\baselinestretch}{1}\footnotesize
\label{table:real-world-large-reg} 
\centering
\begin{tabular}{M{3.5cm} M{5cm} M{1.5cm} M{1.75cm} M{1.1cm} M{1.2cm} M{1.2cm} M{1.2cm} M{1.2cm} N}  

\hline

Dataset (size)
&\begin{tabular}{@{}c@{}} Categorical \\ variables ($K_j$) \end{tabular}
&\begin{tabular}{@{}c@{}} Limited-$K$ \\  CART \end{tabular}
&\begin{tabular}{@{}c@{}} Unlimited-$K$ \\ CART \end{tabular}
&ALOOF
&\begin{tabular}{@{}c@{}} GB via \\ CART \end{tabular}
&\begin{tabular}{@{}c@{}} GB via \\  ALOOF \end{tabular}
&\begin{tabular}{@{}c@{}} RF via\\ CART \end{tabular}
&\begin{tabular}{@{}c@{}} RF via\\ ALOOF \end{tabular}&\\[20pt]

\hline

\begin{tabular}{@{}c@{}} Boston Housing \\ $(506)$ \end{tabular}   
&Town name $(88)$ 
&$24.35$
&$24.07$ 
&${20.83}$
&$9.24$
&${7.88}$
&$9.08$
&${8.99}$& \\[20pt]  



\begin{tabular}{@{}c@{}} Strikes \\ $(626)$ \end{tabular}   
&Country $(18)$ 
&$315.95$
&$315.95$ 
&${280.23}$
&$256.31$
&$257.12$
&$255.59$
&$256.06$& \\[20pt]  



\begin{tabular}{@{}c@{}} Donations \\ $(6521)$ \end{tabular}   
&Socio-cluster $(62)$,  ADI code $(180)$, DMA code $(180)$,  MSA code $(245)$,  Mailing list $(348)$,   Zip code $(3824)$ 
&$30.99$
&$39.30$ 
&${22.92^*}$
&$23.34$
&${18.89^*}$
&$21.39$
&${16.28^*}$& \\[20pt]  



\begin{tabular}{@{}c@{}} Internet - years online \\ $(10108)$ \end{tabular}   
& Occupation $(46)$,  Language $(99)$,  Country $(129)$  
&$0.727$
&$0.754$ 
&${0.703^*}$
&$0.699$
&$0.698$
&$0.698$
&$0.698$& \\[20pt]  



\begin{tabular}{@{}c@{}} Internet - household  income \\ $(10108)$ \end{tabular}   
&Occupation $(46)$,  Language $(99)$,  Country $(129)$ 
&$4.144$
&$4.308$ 
&${4.103^*}$
&$4.099$
&${4.005^*}$
&$3.991$
&$3.989$& \\[20pt]  


\hline

\end{tabular}
\end{table*}
\vspace{1em}

\end{landscape}



\begin{landscape}
\begin{table*}[htbp]
\caption{Classification real-world data experiments. The columns correspond to the same models as in the regression experiment, with the additional \cite{sabato2008ranking} (S\&S) algorithm which is only applicable for classification problems. The performance of each method is measured by averaged misclassification rate, using ten-fold cross validation. In addition, a star indicates that the difference between ALOOF its best competitor in the same category (single tree, GB, RF) is statistically significant on a single arbitrary partitioning to train and test sets (this test was only applied to the last four datasets with more than $1000$ observations).}
\centering
\renewcommand{\baselinestretch}{1}\footnotesize
\label{table:real-world-large-class} 
\centering
\begin{tabular}{ M{2.2cm} M{6.3cm} M{1.45cm} M{1.75cm} M{0.7cm} M{1.1cm} M{0.95cm} M{1.1cm} M{0.9cm} M{1.1cm} N}  

\hline

Dataset (size, portion of positives)
&\begin{tabular}{@{}c@{}} Categorical \\ variables ($K_j$) \end{tabular}
&\begin{tabular}{@{}c@{}} Limited-$K$ \\  CART \end{tabular}
&\begin{tabular}{@{}c@{}} Unlimited-$K$ \\ CART \end{tabular}
&S\&S
&ALOOF
&\begin{tabular}{@{}c@{}} GB via \\ CART \end{tabular}
&\begin{tabular}{@{}c@{}} GB via \\  ALOOF \end{tabular}
&\begin{tabular}{@{}c@{}} RF via\\ CART \end{tabular}
&\begin{tabular}{@{}c@{}} RF via\\ ALOOF \end{tabular}&\\[35pt]

\hline

\begin{tabular}{@{}c@{}} Online Sales \\ $(725, 0.29)$ \end{tabular}   
& Confidential $(70)$, Confidential $(273)$, Confidential $(406)$ 
&$0.198$
&$0.1903$ 
&$0.153$
&${0.151}$
&$0.145$
&${0.135}$
&$0.134$
&${0.121}$& \\[20pt]  



\begin{tabular}{@{}c@{}} Melbourne Grants \\ $(3650, 0.29)$ \end{tabular}   
&Department $(99)$, Sponsor $(234)$, Field $(519)$ 
&$0.260$
&$0.245$ 
&$0.240$
&${0.218^*}$
&$0.186$
&${0.165^*}$
&$0.172$
&${0.153^*}$& \\[20pt]  



\begin{tabular}{@{}c@{}} Price Up  \\ $(3980, 0.045)$ \end{tabular}   
&Brand $(27)$ , Product $(216)$ 
&$0.035$
&$0.047$ 
&$0.036$
&${0.033^*}$
&$0.039$
&${0.034^*}$
&$0.034$
&$0.034$& \\[20pt]  




\begin{tabular}{@{}c@{}} Salary Posting  \\ $(10000, 0.31)$ \end{tabular}   
&Location $(390)$, Company $(390)$, Title $(8324)$ 
&$0.330$
&$0.149$ 
&$0.148$
&${0.142^*}$
&$0.142$
&$0.142$
&$0.140$
&${0.138^*}$& \\[20pt]  




\begin{tabular}{@{}c@{}} CabsCancellations  \\ $(34293, 0.096)$ \end{tabular}   
&Area code $(586)$
&$0.093$
&$0.095$ 
&$0.088$
&${0.083^*}$
&$0.088$
&${0.083^*}$
&$0.083$
&$0.083$& \\[20pt]  



\hline

\end{tabular}
\end{table*}
\vspace{1em}

\end{landscape}


==> Chapters/trees_comp.tex <==

bla bla
